A Unified Calibration Framework for High-Accuracy Articulated Robot Kinematics

Researchers have identified various sources of tool positioning errors for articulated industrial robots and have proposed dedicated compensation strategies. However, these typically require individual, specialized experiments with separate models and identification procedures. This article presents a unified approach to the static calibration of industrial robots that identifies a robot model, including geometric and non-geometric effects (compliant bending, thermal deformation, gear transmission errors), using only a single, straightforward experiment for data collection. The model augments the kinematic chain with virtual joints for each modeled effect and realizes the identification using Gauss-Newton optimization with analytic gradients. Fisher information spectra show that the estimation is well-conditioned and the parameterization near-minimal, whereas systematic temporal cross-validation and model ablations demonstrate robustness of the model identification. The resulting model is very accurate and its identification robust, achieving a mean position error of 26.8 $\mu m$ on a KUKA KR30 industrial robot compared to 102.3 $\mu m$ for purely geometric calibration.

==> data_SyntheticData_singular_value_spectra_T_10_to_50.tex <==
SV_index,TC_2e-05,TC_2e-04,TC_2e-03,TC_2e-02,TC_2e-01,TC_2e+00,TC_2e+01,TC_2e+02
1,114.97651317060361,115.02557754113423,114.98607303126172,115.0317348687459,114.98076641871154,115.79364514760145,720.3980013077277,168.89494198498983
2,114.04347430039104,114.04673223215237,113.9531559879636,113.95678542842963,114.08661146620638,112.72866761717289,708.3383463211605,118.53386063195289
3,112.33555443772865,112.43381300044811,112.29098925179754,112.33370204019228,112.59309290401758,111.48107050506154,576.0250917084719,112.86842140426906
4,73.55755407626975,73.64166237000923,73.56783534926386,73.57461336797053,73.7496031420206,72.71999402130857,232.74295646046426,95.34931255448652
5,68.23400056804799,68.2027428471846,68.15921124812343,68.18326101033165,68.3015990100088,67.01527219434396,160.0888180038808,87.10708550588856
6,61.30668672240821,61.38437720006848,61.309245629770444,61.34044324793503,61.24386211991222,62.80500984311229,139.79488374005737,71.7176892072401
7,27.315268741527614,27.219013453896082,27.621228825718934,27.677584299217607,26.53148195911136,30.933518304567432,138.4551294998655,68.53403644899898
8,25.940506171010135,25.92542584495059,26.527650201040455,26.6086604645614,25.29530788692749,30.169553687786607,120.3238391398453,59.57365265007044
9,21.63305648690512,21.427664305707438,21.62686705222708,21.50752418027739,21.25136082857137,21.26298878366016,104.78099984112421,57.9301192249996
10,19.297392097249944,19.208129044488967,19.49464073555354,19.541715779160487,18.783290393951315,20.362272033847347,86.85519390573,54.58792236536959
11,18.175738885217772,17.951168871603656,18.05542928889432,17.68462635024167,18.482663456679706,17.694028910494836,78.93893658014014,50.57940433463938
12,15.443703643777226,15.51726216517542,15.55019963498685,15.56431981042225,15.781667975232203,17.415401674122407,69.03525810507558,45.372788694484306
13,15.324157601277378,15.086468203344007,15.229634241829151,15.206537124528275,14.741659119075923,15.234512323871085,54.87482891379746,44.73655470714791
14,14.090709347100002,13.54966589094617,13.919907091399851,13.363486116188454,14.259861257560303,13.00680726405065,52.19027850333174,44.450685419363985
15,13.182338801003349,13.356041942490032,13.424485220153866,13.331102828966708,13.379856185881584,12.847659721941206,48.293776200504276,41.4404270372794
16,12.38787967368506,12.08690833663051,12.234508473679524,12.095831118429762,12.285978031079736,12.337139012647583,44.352756478038124,38.43922194431306
17,11.701800680674241,11.563748939679648,11.616615682407796,11.453897205595398,11.91367273861088,11.320551567342559,42.72875375157871,36.198260574189014
18,10.390180686572517,10.397991649334637,10.654195157028715,10.343879449569878,10.466267996045351,10.797078021953858,37.372509078343356,35.790982045143416
19,9.924771343752619,9.861123757509185,9.659708110798023,10.001216636466095,9.564449667039792,10.13093473674359,35.93800423662495,34.12482328631348
20,9.295278267687827,9.28938295246054,9.198468931777942,9.103010797285354,9.406823414089368,9.774429276317237,27.728598433442833,32.18087606244925
21,8.823710586293538,8.584524867336773,8.705312627220257,8.609926443275693,8.681030879236236,9.019993367464188,23.916036072070177,31.753131963152978
22,8.20808700808286,8.255448344185163,8.139984684658069,8.221232318728614,8.3571638888602,7.241409047280594,20.843155496618813,29.22319363870897
23,7.994539766889928,7.986666767082132,7.908827123364758,7.819385664656374,7.979516173758733,6.750843815947894,15.127929007113517,27.868180278529902
24,6.879788448790076,6.968233938361992,6.717437614563197,6.925578970129766,6.949700609465163,6.51119686276153,11.884145768993413,25.840541001193007
25,6.470807838872087,6.5935388186489865,6.463619812782235,6.58022077155385,6.446337069575226,6.17623046083485,10.860097944918856,20.76955895832508
26,6.327630316402281,6.2868312953160155,6.378329679781367,6.223184011369194,6.3590877787709665,6.052410437258902,9.248951721717859,19.7746687864202
27,5.325885926766246,5.3806437481178815,5.248516588235503,5.4504172965454645,5.245616583767021,4.918363775226138,7.3690773799131515,18.364577118781558
28,4.882182742769204,4.945614150504469,4.7880514647173795,4.9508450452449795,4.825009107376216,4.312773472067104,6.502312121312833,16.879409775623206
29,4.720384375381986,4.817850120421859,4.662511557597157,4.807411559962515,4.64356011104802,4.284326499147705,5.962991098431108,14.114701742976978
30,4.461923597496157,4.550419453905419,4.43049607185787,4.545142610292449,4.465059392617512,3.948264150332671,4.134344204191261,13.07413675125169
31,0.00011184149712809149,0.00012524473914379497,0.0005172105812839123,0.004911072743999003,0.15442942909241678,1.1938387859565893,3.7402291756986963,11.830472301749332
32,8.101915517400638e-05,8.46976011403466e-05,0.00033025390141379774,0.0042854603309563895,0.0881273221822111,0.8780530490105537,3.117571086472286,10.788437924916899
33,1.9910732340520106e-05,2.3491268528493504e-05,6.566449334289555e-05,0.0016989238980736167,0.028394253870621937,0.7923507600384045,2.0538362674766963,6.989564542067448
34,1.749402466083154e-05,1.9574194052558377e-05,5.506496594419345e-05,0.0009840211180473955,0.014525579768867057,0.3271847935341152,1.4546303374089917,6.490815237642752
35,5.111205098758738e-07,2.9786876510931757e-07,3.782438199356487e-06,8.678493854606027e-05,0.00962437669945598,0.12849149983872343,1.202408683792035,1.8301526755966127
36,3.603539333530213e-07,2.421863544038591e-07,1.1450572227004339e-06,1.942362871352991e-05,0.007210093821005816,0.08996127147582028,0.1469466186398652,0.2633176279080919


==> data_full_Temp_only.tex <==
index,timestamp,T9
0,0.0,26.875
1,24.930000066757202,26.875
2,48.049999952316284,26.875
3,71.00999999046326,26.875
4,94.07999992370605,26.875
5,118.44000005722046,26.875
6,141.53999996185303,26.875
7,164.79999995231628,26.875
8,187.6399998664856,26.875
9,210.74000000953674,26.9375
10,235.29999995231628,26.9375
11,346.8599998950958,26.9375
12,370.4500000476837,26.9375
13,393.4800000190735,26.9375
14,417.47000002861023,26.9375
15,440.59999990463257,26.9375
16,464.22000002861023,26.9375
17,488.4500000476837,26.9375
18,511.59999990463257,26.9375
19,535.829999923706,26.9375
20,559.9400000572205,26.9375
21,583.9700000286102,26.9375
22,607.0999999046326,26.9375
23,630.6600000858307,26.9375
24,654.5,26.9375
25,678.1600000858307,26.9375
26,790.25,26.9375
27,813.0999999046326,27.0
28,836.5499999523163,26.9375
29,859.7300000190735,27.0
30,883.329999923706,27.0
31,955.8999998569489,27.0
32,980.0499999523163,26.9375
33,1004.0599999427795,27.0
34,1028.2699999809265,27.0
35,1051.7000000476837,27.0
36,1075.6800000667572,27.0
37,1099.2000000476837,27.0
38,1122.5199999809265,27.0
39,1293.869999885559,27.0
40,1316.960000038147,27.0625
41,1340.3799998760223,27.0
42,1364.2200000286102,27.0625
43,1411.5699999332428,27.0
44,1435.5099999904633,27.0
45,1459.670000076294,27.0625
46,1483.8799998760223,27.0625
47,1507.0499999523163,27.0625
48,1530.9500000476837,27.0625
49,1554.0999999046326,27.0625
50,1577.6600000858307,27.0625
51,1600.5,27.0625
52,1625.289999961853,27.0625
53,1765.9300000667572,27.0625
54,1790.119999885559,27.125
55,1814.1800000667572,27.0625
56,1837.6099998950958,27.0625
57,1860.539999961853,27.0625
58,1884.2699999809265,27.0625
59,1908.1900000572205,27.0625
60,1954.7699999809265,27.0625
61,1978.5299999713898,27.0625
62,2001.3799998760223,27.0625
63,2025.5999999046326,27.0625
64,2048.789999961853,27.125
65,2071.869999885559,27.0625
66,2094.819999933243,27.125
67,2319.9700000286102,27.125
68,2344.4400000572205,27.125
69,2367.399999856949,27.125
70,2438.3799998760223,27.125
71,2461.4500000476837,27.125
72,2484.8799998760223,27.125
73,2508.670000076294,27.125
74,2533.4400000572205,27.125
75,2557.0099999904633,27.125
76,2580.109999895096,27.1875
77,2604.75,27.1875
78,2627.5999999046326,27.125
79,2651.649999856949,27.125
80,2766.069999933243,27.1875
81,2789.149999856949,27.125
82,2811.869999885559,27.1875
83,2835.2599999904633,27.1875
84,2858.3899998664856,27.1875
85,2882.3399999141693,27.1875
86,2905.539999961853,27.1875
87,2928.569999933243,27.1875
88,2951.569999933243,27.1875
89,2975.3399999141693,27.1875
90,2998.7300000190735,27.1875
91,3169.319999933243,27.1875
92,3193.5499999523163,27.1875
93,3217.4700000286102,27.25
94,3289.670000076294,27.25
95,3313.899999856949,27.1875
96,3360.7999999523163,27.1875
97,3384.289999961853,27.25
98,3407.039999961853,27.25
99,3429.8899998664856,27.25
100,3454.920000076294,27.25
101,3478.1399998664856,27.25
102,3502.4900000095367,27.25
103,3675.869999885559,27.25
104,3700.149999856949,27.25
105,3723.5,27.25
106,3747.619999885559,27.25
107,3771.7400000095367,27.25
108,3795.5899999141693,27.25
109,3839.6900000572205,27.25
110,3863.4400000572205,27.25
111,3886.539999961853,27.25
112,3910.5099999904633,27.3125
113,3934.0299999713898,27.25
114,3956.7300000190735,27.25
115,3980.9700000286102,27.25
116,4004.1399998664856,27.25
117,4116.849999904633,27.25
118,4139.47000002861,27.25
119,4163.180000066757,27.3125
120,4186.509999990463,27.3125
121,4209.129999876022,27.3125
122,4233.299999952316,27.3125
123,4257.25,27.3125
124,4281.200000047684,27.3125
125,4328.930000066757,27.3125
126,4353.069999933243,27.3125
127,4376.129999876022,27.3125
128,4399.27999997139,27.3125
129,4423.319999933243,27.3125
130,4447.4800000190735,27.3125
131,4470.579999923706,27.3125
132,4494.2699999809265,27.3125
133,4609.2300000190735,27.3125
134,4632.680000066757,27.3125
135,4656.369999885559,27.3125
136,4679.539999961853,27.3125
137,4725.97000002861,27.3125
138,4749.6900000572205,27.375
139,4772.920000076294,27.375
140,4796.5599999427795,27.3125
141,4819.9800000190735,27.3125
142,4843.420000076294,27.375
143,4866.609999895096,27.375
144,4890.539999961853,27.375
145,4913.629999876022,27.375
146,5024.859999895096,27.375
147,5048.619999885559,27.375
148,5072.379999876022,27.375
149,5095.839999914169,27.375
150,5120.210000038147,27.375
151,5144.339999914169,27.375
152,5168.450000047684,27.375
153,5191.819999933243,27.375
154,5214.910000085831,27.375
155,5237.950000047684,27.375
156,5261.589999914169,27.375
157,5286.139999866486,27.375
158,5309.410000085831,27.375
159,5333.660000085831,27.375
160,5357.379999876022,27.375
161,5380.47000002861,27.375
162,5403.740000009537,27.375
163,5426.490000009537,27.375
164,5450.3099999427795,27.375
165,5591.75,27.375
166,5614.599999904633,27.4375
167,5637.349999904633,27.375
168,5660.910000085831,27.4375
169,5684.609999895096,27.4375
170,5708.119999885559,27.4375
171,5731.180000066757,27.4375
172,5754.599999904633,27.4375
173,5777.700000047684,27.4375
174,5800.740000009537,27.4375
175,5823.649999856949,27.4375
176,5847.170000076294,27.4375
177,5870.420000076294,27.4375
178,5893.129999876022,27.4375
179,6064.700000047684,27.4375
180,6088.75,27.4375
181,6112.210000038147,27.4375
182,6135.899999856949,27.4375
183,6160.579999923706,27.4375
184,6184.609999895096,27.4375
185,6207.97000002861,27.5
186,6232.22000002861,27.4375
187,6255.829999923706,27.4375
188,6279.569999933243,27.4375
189,6303.180000066757,27.5
190,6326.369999885559,27.4375
191,6350.799999952316,27.5
192,6375.069999933243,27.5
193,6589.2300000190735,27.5
194,6612.139999866486,27.5
195,6635.819999933243,27.5
196,6659.47000002861,27.5
197,6683.0599999427795,27.5
198,6707.170000076294,27.5
199,6730.97000002861,27.5
200,6753.680000066757,27.5
201,6776.680000066757,27.5
202,6800.920000076294,27.5
203,6823.950000047684,27.5
204,6847.680000066757,27.5
205,6872.240000009537,27.5
206,6896.119999885559,27.5
207,6919.22000002861,27.5
208,7059.829999923706,27.5
209,7083.369999885559,27.5
210,7106.430000066757,27.5
211,7130.579999923706,27.5
212,7153.740000009537,27.5
213,7177.609999895096,27.5
214,7201.009999990463,27.5
215,7224.329999923706,27.5
216,7247.7699999809265,27.5
217,7271.5199999809265,27.5
218,7295.710000038147,27.5
219,7319.369999885559,27.5
220,7342.799999952316,27.5
221,7365.9800000190735,27.5
222,7389.599999904633,27.5625
223,7591.160000085831,27.5625
224,7614.139999866486,27.5625
225,7637.619999885559,27.5625
226,7660.789999961853,27.5625
227,7684.339999914169,27.5625
228,7707.680000066757,27.5625
229,7731.950000047684,27.5625
230,7755.369999885559,27.5625
231,7779.8099999427795,27.5625
232,7849.879999876022,27.5625
233,7873.399999856949,27.5625
234,7897.259999990463,27.5625
235,8122.589999914169,27.5625
236,8146.349999904633,27.5625
237,8170.329999923706,27.5625
238,8194.369999885559,27.5625
239,8218.119999885559,27.5625
240,8242.259999990463,27.625
241,8266.109999895096,27.625
242,8290.269999980927,27.5625
243,8313.990000009537,27.625
244,8337.33999991417,27.5625
245,8360.210000038147,27.625
246,8384.490000009537,27.5625
247,8407.519999980927,27.5625
248,8432.210000038147,27.625
249,8455.670000076294,27.5625
250,8567.75,27.625
251,8590.899999856949,27.5625
252,8614.47000002861,27.5625
253,8638.450000047684,27.625
254,8661.19000005722,27.625
255,8684.97000002861,27.5625
256,8708.519999980927,27.625
257,8731.519999980927,27.5625
258,8754.930000066757,27.5625
259,8778.829999923706,27.625
260,8802.379999876022,27.625
261,8825.609999895096,27.625
262,8849.129999876022,27.625
263,8873.569999933243,27.625
264,8985.180000066757,27.625
265,9009.83999991417,27.625
266,9032.670000076294,27.625
267,9056.710000038147,27.625
268,9079.91000008583,27.625
269,9103.05999994278,27.625
270,9125.859999895096,27.625
271,9148.819999933243,27.625
272,9172.91000008583,27.625
273,9196.129999876022,27.625
274,9219.680000066757,27.625
275,9242.930000066757,27.625
276,9265.829999923706,27.625
277,9288.789999961853,27.625
278,9312.289999961853,27.625
279,9335.980000019073,27.625
280,9359.319999933243,27.625
281,9470.759999990463,27.625
282,9493.619999885559,27.625
283,9517.789999961853,27.6875
284,9541.379999876022,27.625
285,9565.230000019073,27.625
286,9589.41000008583,27.625
287,9612.579999923706,27.625
288,9636.269999980927,27.625
289,9659.08999991417,27.625
290,9682.730000019073,27.625
291,9706.269999980927,27.625
292,9729.41000008583,27.625
293,9800.05999994278,27.625
294,9823.710000038147,27.6875
295,9985.5,27.6875
296,10009.349999904633,27.6875
297,10033.180000066757,27.6875
298,10056.52999997139,27.6875
299,10079.369999885559,27.6875
300,10102.210000038147,27.6875
301,10125.329999923706,27.6875
302,10149.52999997139,27.6875
303,10196.430000066757,27.6875
304,10220.519999980927,27.6875
305,10244.25,27.6875
306,10267.33999991417,27.6875
307,10290.710000038147,27.6875
308,10461.450000047684,27.6875
309,10484.420000076294,27.6875
310,10508.069999933243,27.6875
311,10532.299999952316,27.6875
312,10556.490000009537,27.6875
313,10581.299999952316,27.6875
314,10603.91000008583,27.6875
315,10627.039999961853,27.6875
316,10651.039999961853,27.6875
317,10674.109999895096,27.6875
318,10698.02999997139,27.6875
319,10721.75,27.6875
320,10745.990000009537,27.6875
321,10887.869999885559,27.6875
322,10911.099999904633,27.75
323,10934.91000008583,27.6875
324,10957.950000047684,27.75
325,10982.649999856949,27.6875
326,11006.91000008583,27.75
327,11029.950000047684,27.6875
328,11054.0,27.6875
329,11076.899999856949,27.6875
330,11100.619999885559,27.6875
331,11124.369999885559,27.6875
332,11149.240000009537,27.6875
333,11173.609999895096,27.6875
334,11198.210000038147,27.6875
335,11220.990000009537,27.6875
336,11244.97000002861,27.6875
337,11267.930000066757,27.6875
338,11469.539999961853,27.75
339,11493.450000047684,27.6875
340,11517.44000005722,27.75
341,11541.109999895096,27.6875
342,11564.349999904633,27.75
343,11588.670000076294,27.75
344,11612.109999895096,27.75
345,11636.049999952316,27.6875
346,11660.170000076294,27.75
347,11683.769999980927,27.6875
348,11706.950000047684,27.75
349,11730.079999923706,27.6875
350,11753.990000009537,27.75
351,11776.97000002861,27.75
352,11801.670000076294,27.75
353,11824.450000047684,27.75
354,11978.19000005722,27.75
355,12002.619999885559,27.75
356,12025.549999952316,27.75
357,12049.129999876022,27.75
358,12073.58999991417,27.75
359,12096.97000002861,27.75
360,12120.02999997139,27.75
361,12143.299999952316,27.75
362,12214.80999994278,27.75
363,12385.450000047684,27.75
364,12454.960000038147,27.75
365,12478.819999933243,27.75
366,12502.22000002861,27.75
367,12526.349999904633,27.75
368,12550.369999885559,27.75
369,12575.02999997139,27.75
370,12598.210000038147,27.75
371,12622.230000019073,27.75
372,12645.579999923706,27.75
373,12668.700000047684,27.75
374,12692.25,27.75
375,12715.299999952316,27.75
376,12738.599999904633,27.75
377,12762.33999991417,27.75
378,12873.170000076294,27.75
379,12896.16000008583,27.75
380,12919.149999856949,27.75
381,12942.149999856949,27.75
382,12965.899999856949,27.75
383,12989.430000066757,27.75
384,13012.769999980927,27.75
385,13035.899999856949,27.75
386,13058.849999904633,27.75
387,13082.619999885559,27.75
388,13106.170000076294,27.75
389,13129.740000009537,27.75
390,13152.950000047684,27.75
391,13175.930000066757,27.75
392,13286.359999895096,27.8125
393,13309.19000005722,27.75
394,13332.990000009537,27.8125
395,13356.990000009537,27.75
396,13380.97000002861,27.75
397,13404.480000019073,27.75
398,13427.69000005722,27.8125
399,13452.389999866486,27.8125
400,13475.77999997139,27.8125
401,13498.629999876022,27.75
402,13523.25,27.75
403,13546.710000038147,27.75
404,13570.149999856949,27.75
405,13593.680000066757,27.75
406,13705.829999923706,27.75
407,13729.47000002861,27.75
408,13753.480000019073,27.75
409,13777.41000008583,27.75
410,13801.369999885559,27.8125
411,13825.019999980927,27.8125
412,13847.710000038147,27.75
413,13871.91000008583,27.8125
414,13894.700000047684,27.8125
415,13917.889999866486,27.75
416,13941.399999856949,27.8125
417,13964.930000066757,27.75
418,13988.700000047684,27.8125
419,14013.289999961853,27.8125
420,14036.930000066757,27.8125
421,14149.509999990463,27.8125
422,14172.609999895096,27.8125
423,14299.289999961853,27.8125
424,14322.97000002861,27.8125
425,14346.200000047684,27.8125
426,14369.139999866486,27.8125
427,14391.72000002861,27.8125
428,14415.569999933243,27.8125
429,14439.30999994278,27.8125
430,14463.33999991417,27.8125
431,14486.670000076294,27.8125
432,14510.769999980927,27.8125
433,14534.149999856949,27.8125
434,14557.319999933243,27.8125
435,14580.269999980927,27.8125
436,14604.700000047684,27.8125
437,14775.399999856949,27.8125
438,14798.75,27.8125
439,14822.47000002861,27.8125
440,14846.519999980927,27.8125
441,14869.25,27.8125
442,14892.19000005722,27.8125
443,14916.539999961853,27.8125
444,14963.569999933243,27.8125
445,14987.399999856949,27.8125
446,15010.329999923706,27.8125
447,15035.0,27.8125
448,15058.259999990463,27.8125
449,15081.700000047684,27.8125
450,15105.069999933243,27.8125
451,15246.19000005722,27.8125
452,15270.049999952316,27.8125
453,15294.049999952316,27.8125
454,15318.049999952316,27.8125
455,15341.230000019073,27.8125
456,15366.069999933243,27.8125
457,15389.980000019073,27.8125
458,15413.420000076294,27.8125
459,15438.139999866486,27.8125
460,15461.77999997139,27.8125
461,15484.72000002861,27.8125
462,15508.210000038147,27.8125
463,15531.539999961853,27.8125
464,15554.759999990463,27.8125
465,15578.0,27.8125
466,15601.259999990463,27.8125
467,15742.240000009537,27.8125
468,15766.509999990463,27.8125
469,15790.149999856949,27.8125
470,15814.44000005722,27.8125
471,15862.47000002861,27.8125
472,15886.230000019073,27.8125
473,15910.55999994278,27.8125
474,15934.799999952316,27.8125
475,15957.670000076294,27.8125
476,15981.83999991417,27.8125
477,16004.569999933243,27.8125
478,16028.27999997139,27.8125
479,16051.91000008583,27.8125
480,16193.740000009537,27.8125
481,16216.80999994278,27.8125
482,16240.019999980927,27.8125
483,16265.269999980927,27.8125
484,16288.75,27.8125
485,16311.69000005722,27.8125
486,16334.889999866486,27.8125
487,16359.02999997139,27.875
488,16382.75,27.8125
489,16406.879999876022,27.8125
490,16430.25,27.8125
491,16453.460000038147,27.8125
492,16476.55999994278,27.8125
493,16500.579999923706,27.8125
494,16672.39999985695,27.8125
495,16696.009999990463,27.8125
496,16719.44000005722,27.8125
497,16743.019999980927,27.8125
498,16766.25,27.8125
499,16790.05999994278,27.8125
500,16813.329999923706,27.8125
501,16836.430000066757,27.8125
502,16860.980000019073,27.8125
503,16885.41000008583,27.875
504,16908.450000047684,27.875
505,16931.539999961853,27.8125
506,16954.61999988556,27.8125
507,16978.30999994278,27.8125
508,17001.730000019073,27.8125
509,17025.25,27.8125
510,17136.680000066757,27.875
511,17159.829999923706,27.875
512,17182.91000008583,27.8125
513,17206.769999980927,27.8125
514,17229.769999980927,27.8125
515,17253.009999990463,27.8125
516,17277.269999980927,27.8125
517,17301.319999933243,27.8125
518,17325.009999990463,27.8125
519,17349.240000009537,27.8125
520,17372.539999961853,27.8125
521,17394.980000019073,27.8125
522,17418.730000019073,27.8125
523,17442.789999961853,27.8125
524,17466.549999952316,27.875
525,17489.930000066757,27.8125
526,17661.83999991417,27.8125
527,17685.299999952316,27.875
528,17708.200000047684,27.8125
529,17732.299999952316,27.8125
530,17756.049999952316,27.875
531,17779.61999988556,27.875
532,17803.430000066757,27.875
533,17826.89999985695,27.875
534,17851.769999980927,27.875
535,17875.58999991417,27.8125
536,17898.299999952316,27.8125
537,17922.230000019073,27.875
538,17945.269999980927,27.875
539,17970.230000019073,27.875
540,17994.509999990463,27.8125
541,18036.769999980927,27.875
542,18060.549999952316,27.8125
543,18231.289999961853,27.8125
544,18255.109999895096,27.8125
545,18279.77999997139,27.8125
546,18302.89999985695,27.8125
547,18326.180000066757,27.8125
548,18350.039999961853,27.875
549,18374.210000038147,27.875
550,18398.039999961853,27.8125
551,18422.14999985695,27.875
552,18445.069999933243,27.8125
553,18469.0,27.8125
554,18491.66000008583,27.8125
555,18514.539999961853,27.8125
556,18538.670000076294,27.8125
557,18561.91000008583,27.8125
558,18584.700000047684,27.8125
559,18761.25,27.8125
560,18785.180000066757,27.8125
561,18808.33999991417,27.8125
562,18831.97000002861,27.8125
563,18881.450000047684,27.8125
564,18905.200000047684,27.8125
565,18928.30999994278,27.8125
566,18951.69000005722,27.8125
567,18975.859999895096,27.8125
568,18999.639999866486,27.8125
569,19023.319999933243,27.8125
570,19046.19000005722,27.8125
571,19157.129999876022,27.8125
572,19179.80999994278,27.8125
573,19204.039999961853,27.8125
574,19227.930000066757,27.8125
575,19251.990000009537,27.8125
576,19275.55999994278,27.8125
577,19299.77999997139,27.8125
578,19323.72000002861,27.8125
579,19346.69000005722,27.8125
580,19370.819999933243,27.8125
581,19393.86999988556,27.8125
582,19416.980000019073,27.8125
583,19440.569999933243,27.8125
584,19581.19000005722,27.8125
585,19604.829999923706,27.8125
586,19628.019999980927,27.8125
587,19650.930000066757,27.8125
588,19675.05999994278,27.8125
589,19698.670000076294,27.8125
590,19721.609999895096,27.8125
591,19745.950000047684,27.8125
592,19769.14999985695,27.8125
593,19792.109999895096,27.8125
594,19815.519999980927,27.8125
595,19839.700000047684,27.8125
596,19863.259999990463,27.8125
597,20064.960000038147,27.8125
598,20088.329999923706,27.8125
599,20110.950000047684,27.8125
600,20134.480000019073,27.8125
601,20158.710000038147,27.8125
602,20183.11999988556,27.8125
603,20207.710000038147,27.8125
604,20231.490000009537,27.8125
605,20255.759999990463,27.8125
606,20278.58999991417,27.8125
607,20303.450000047684,27.8125
608,20326.799999952316,27.8125
609,20349.819999933243,27.8125
610,20372.740000009537,27.8125
611,20395.670000076294,27.8125
612,20420.41000008583,27.8125
613,20443.61999988556,27.8125
614,20467.700000047684,27.8125
615,20490.379999876022,27.8125
616,20654.450000047684,27.8125
617,20678.039999961853,27.8125
618,20701.86999988556,27.8125
619,20725.27999997139,27.8125
620,20748.109999895096,27.8125
621,20771.19000005722,27.75
622,20795.389999866486,27.75
623,20818.52999997139,27.8125
624,20841.47000002861,27.8125
625,20865.759999990463,27.8125
626,20889.14999985695,27.8125
627,20913.64999985695,27.8125
628,20937.730000019073,27.8125
629,20962.05999994278,27.75
630,21073.700000047684,27.75
631,21096.77999997139,27.8125
632,21143.609999895096,27.75
633,21166.519999980927,27.75
634,21190.16000008583,27.75
635,21236.769999980927,27.75
636,21259.80999994278,27.75
637,21283.11999988556,27.75
638,21305.710000038147,27.75
639,21328.52999997139,27.75
640,21352.86999988556,27.8125
641,21493.61999988556,27.75
642,21517.420000076294,27.8125
643,21541.569999933243,27.75
644,21565.039999961853,27.8125
645,21588.170000076294,27.75
646,21612.950000047684,27.75
647,21636.700000047684,27.75
648,21660.079999923706,27.75
649,21683.299999952316,27.75
650,21707.849999904633,27.75
651,21731.180000066757,27.75
652,21754.420000076294,27.75
653,21779.83999991417,27.75
654,21802.960000038147,27.75
655,21826.86999988556,27.75
656,21850.64999985695,27.75
657,21874.879999876022,27.75
658,22015.66000008583,27.75
659,22039.72000002861,27.75
660,22063.609999895096,27.75
661,22086.139999866486,27.75
662,22110.05999994278,27.75
663,22133.66000008583,27.75
664,22156.569999933243,27.75
665,22179.329999923706,27.75
666,22202.389999866486,27.75
667,22225.490000009537,27.75
668,22249.319999933243,27.75
669,22272.379999876022,27.75
670,22295.700000047684,27.75
671,22497.009999990463,27.75
672,22520.89999985695,27.75
673,22545.139999866486,27.75
674,22569.329999923706,27.6875
675,22592.950000047684,27.75
676,22616.799999952316,27.6875
677,22639.97000002861,27.75
678,22664.700000047684,27.75
679,22688.480000019073,27.6875
680,22711.210000038147,27.75
681,22734.69000005722,27.6875
682,22757.539999961853,27.6875
683,22781.41000008583,27.75
684,22805.33999991417,27.6875
685,23005.91000008583,27.6875
686,23030.14999985695,27.75
687,23053.859999895096,27.75
688,23077.200000047684,27.6875
689,23101.490000009537,27.6875
690,23125.58999991417,27.6875
691,23148.97000002861,27.6875
692,23171.889999866486,27.6875
693,23196.129999876022,27.6875
694,23219.269999980927,27.6875
695,23242.83999991417,27.6875
696,23266.259999990463,27.6875
697,23289.77999997139,27.625
698,23314.0,27.625
699,23454.920000076294,27.6875
700,23478.639999866486,27.6875
701,23502.05999994278,27.6875
702,23525.990000009537,27.6875
703,23549.27999997139,27.6875
704,23573.39999985695,27.6875
705,23600.170000076294,27.625
706,23624.77999997139,27.6875
707,23648.5,27.625
708,23671.480000019073,27.625
709,23694.89999985695,27.625
710,23717.77999997139,27.625
711,23740.97000002861,27.625
712,23971.960000038147,27.625
713,23996.19000005722,27.625
714,24018.920000076294,27.625
715,24042.36999988556,27.625
716,24065.39999985695,27.625
717,24088.819999933243,27.625
718,24112.490000009537,27.625
719,24136.289999961853,27.625
720,24159.97000002861,27.625
721,24183.769999980927,27.5625
722,24207.920000076294,27.625
723,24231.990000009537,27.625
724,24256.329999923706,27.625
725,24279.629999876022,27.625
726,24302.789999961853,27.625
727,24444.879999876022,27.625
728,24468.319999933243,27.625
729,24491.539999961853,27.625
730,24515.139999866486,27.625
731,24539.210000038147,27.5625
732,24563.240000009537,27.625
733,24586.33999991417,27.625
734,24610.789999961853,27.625
735,24635.230000019073,27.5625
736,24658.64999985695,27.5625
737,24681.629999876022,27.5625
738,24705.77999997139,27.5625
739,24729.039999961853,27.5625
740,24751.990000009537,27.5625
741,24922.89999985695,27.625
742,24946.47000002861,27.5625
743,24969.549999952316,27.5625
744,24993.379999876022,27.5625
745,25017.02999997139,27.5625
746,25040.97000002861,27.5625
747,25064.83999991417,27.5625
748,25088.83999991417,27.5625
749,25112.97000002861,27.5625
750,25159.77999997139,27.5625
751,25184.019999980927,27.5625
752,25208.129999876022,27.5625
753,25231.450000047684,27.5625
754,25254.30999994278,27.5625
755,25364.66000008583,27.5625
756,25388.129999876022,27.5625
757,25413.58999991417,27.5625
758,25437.549999952316,27.5625
759,25460.710000038147,27.5625
760,25483.920000076294,27.5625
761,25508.129999876022,27.5
762,25531.86999988556,27.5
763,25554.829999923706,27.5
764,25577.61999988556,27.5
765,25600.789999961853,27.5
766,25742.509999990463,27.5
767,25766.109999895096,27.5
768,25789.170000076294,27.5625
769,25812.47000002861,27.5
770,25835.289999961853,27.5
771,25859.27999997139,27.5
772,25882.450000047684,27.5
773,25905.41000008583,27.5
774,25929.61999988556,27.5
775,25952.97000002861,27.5
776,25975.599999904633,27.5
777,25998.299999952316,27.4375
778,26021.389999866486,27.5
779,26044.950000047684,27.4375
780,26068.079999923706,27.5
781,26092.099999904633,27.4375
782,26233.259999990463,27.4375
783,26257.289999961853,27.4375
784,26281.009999990463,27.4375
785,26304.480000019073,27.4375
786,26329.109999895096,27.4375
787,26353.509999990463,27.4375
788,26376.889999866486,27.4375
789,26399.80999994278,27.4375
790,26424.109999895096,27.4375
791,26448.269999980927,27.4375
792,26517.879999876022,27.4375
793,26541.200000047684,27.4375
794,26565.25,27.4375
795,26589.039999961853,27.4375
796,26699.980000019073,27.4375
797,26724.569999933243,27.4375
798,26748.83999991417,27.4375
799,26772.019999980927,27.4375
800,26795.889999866486,27.375
801,26819.430000066757,27.375
802,26843.009999990463,27.375
803,26866.950000047684,27.375
804,26891.039999961853,27.375
805,26915.490000009537,27.375
806,26939.599999904633,27.375
807,26962.799999952316,27.375
808,26986.14999985695,27.4375
809,27098.450000047684,27.375
810,27121.460000038147,27.375
811,27145.769999980927,27.375
812,27169.44000005722,27.375
813,27193.5,27.375
814,27218.319999933243,27.375
815,27241.069999933243,27.375
816,27264.180000066757,27.375
817,27288.349999904633,27.375
818,27311.52999997139,27.375
819,27335.47000002861,27.375
820,27447.180000066757,27.375
821,27470.430000066757,27.375
822,27493.139999866486,27.375
823,27516.389999866486,27.375
824,27540.36999988556,27.3125
825,27563.47000002861,27.375
826,27611.049999952316,27.3125
827,27634.47000002861,27.3125
828,27657.69000005722,27.3125
829,27680.55999994278,27.3125
830,27703.379999876022,27.3125
831,27726.519999980927,27.3125
832,27750.420000076294,27.3125
833,27773.980000019073,27.3125
834,27946.230000019073,27.3125
835,27969.41000008583,27.3125
836,27992.670000076294,27.3125
837,28016.299999952316,27.3125
838,28040.5,27.3125
839,28064.44000005722,27.3125
840,28088.349999904633,27.3125
841,28112.44000005722,27.3125
842,28136.109999895096,27.3125
843,28160.079999923706,27.3125
844,28183.44000005722,27.3125
845,28371.879999876022,27.25
846,28395.799999952316,27.3125
847,28418.930000066757,27.25
848,28441.64999985695,27.3125
849,28465.730000019073,27.3125
850,28488.670000076294,27.25
851,28512.700000047684,27.3125
852,28535.97000002861,27.25
853,28558.829999923706,27.25
854,28582.819999933243,27.25
855,28606.47000002861,27.25
856,28630.680000066757,27.25
857,28653.289999961853,27.25
858,28824.83999991417,27.25
859,28848.379999876022,27.25
860,28895.27999997139,27.25
861,28918.44000005722,27.25
862,28941.950000047684,27.25
863,28965.97000002861,27.25
864,28988.740000009537,27.25
865,29012.25,27.25
866,29036.769999980927,27.25
867,29060.66000008583,27.1875
868,29085.450000047684,27.25
869,29108.730000019073,27.25
870,29131.769999980927,27.1875
871,29154.700000047684,27.1875
872,29295.14999985695,27.25
873,29319.240000009537,27.1875
874,29342.329999923706,27.1875
875,29366.47000002861,27.1875
876,29390.009999990463,27.1875
877,29412.700000047684,27.1875
878,29436.769999980927,27.25
879,29459.629999876022,27.1875
880,29482.849999904633,27.1875
881,29507.170000076294,27.1875
882,29530.960000038147,27.1875
883,29554.789999961853,27.1875
884,29577.879999876022,27.1875
885,29601.170000076294,27.1875
886,29624.049999952316,27.1875
887,29647.109999895096,27.1875
888,29787.52999997139,27.1875
889,29811.64999985695,27.1875
890,29834.950000047684,27.1875
891,29859.170000076294,27.1875
892,29883.349999904633,27.125
893,29906.61999988556,27.125
894,29929.799999952316,27.125
895,29953.730000019073,27.125
896,29977.52999997139,27.125
897,30224.75,27.125
898,30248.170000076294,27.125
899,30271.5,27.125
900,30312.680000066757,27.125
901,30336.289999961853,27.125
902,30359.950000047684,27.0625
903,30383.670000076294,27.0625
904,30406.47000002861,27.125
905,30429.289999961853,27.125
906,30452.33999991417,27.125
907,30623.460000038147,27.0625
908,30647.490000009537,27.0625
909,30671.509999990463,27.0625
910,30696.099999904633,27.125
911,30720.5,27.0625
912,30743.519999980927,27.0625
913,30767.11999988556,27.0625
914,30791.08999991417,27.0625
915,30815.210000038147,27.0625
916,30838.86999988556,27.0625
917,30864.930000066757,27.0625
918,30887.80999994278,27.0625
919,31072.170000076294,27.0625
920,31095.049999952316,27.0625
921,31119.019999980927,27.0625
922,31142.61999988556,27.0625
923,31166.039999961853,27.0625
924,31190.25,27.0625
925,31213.30999994278,27.0625
926,31236.509999990463,27.0625
927,31259.180000066757,27.0625
928,31282.83999991417,27.0625
929,31305.730000019073,27.0
930,31328.710000038147,27.0
931,31351.769999980927,27.0
932,31376.289999961853,27.0
933,31400.170000076294,27.0
934,31424.58999991417,27.0
935,31448.180000066757,27.0
936,31471.599999904633,27.0
937,31582.950000047684,27.0
938,31607.379999876022,27.0
939,31632.519999980927,27.0
940,31655.14999985695,27.0
941,31678.22000002861,27.0
942,31702.25,27.0
943,31726.389999866486,27.0
944,31749.879999876022,26.9375
945,31773.099999904633,26.9375
946,31796.420000076294,26.9375
947,31843.14999985695,26.9375
948,31867.25,26.9375
949,31890.36999988556,26.9375
950,31914.569999933243,26.9375
951,31938.14999985695,26.9375
952,32048.889999866486,26.9375
953,32072.91000008583,26.9375
954,32096.97000002861,26.9375
955,32120.389999866486,26.9375
956,32144.139999866486,26.9375
957,32167.319999933243,26.9375
958,32190.430000066757,26.875
959,32213.539999961853,26.875
960,32237.269999980927,26.875
961,32260.879999876022,26.875
962,32284.670000076294,26.875
963,32309.36999988556,26.875
964,32333.19000005722,26.875
965,32357.769999980927,26.875
966,32470.099999904633,26.875
967,32494.069999933243,26.875
968,32517.569999933243,26.875
969,32541.30999994278,26.875
970,32564.69000005722,26.875
971,32587.329999923706,26.875
972,32610.61999988556,26.875
973,32634.670000076294,26.875
974,32657.349999904633,26.8125
975,32680.480000019073,26.875
976,32704.210000038147,26.875
977,32727.5,26.875
978,32751.69000005722,26.875
979,32775.11999988556,26.8125
980,32798.80999994278,26.875
981,32939.799999952316,26.875
982,32962.609999895096,26.875
983,32986.76999998093,26.875
984,33010.00999999046,26.875
985,33032.99000000954,26.875
986,33056.31999993324,26.875
987,33079.00999999046,26.8125
988,33101.76999998093,26.875
989,33125.89999985695,26.875
990,33150.420000076294,26.875
991,33175.200000047684,26.875
992,33199.26999998093,26.875
993,33223.829999923706,26.875
994,33247.08999991417,26.875
995,33270.079999923706,26.8125
996,33292.75999999046,26.8125
997,33434.859999895096,26.875
998,33459.01999998093,26.875
999,33483.049999952316,26.875
1000,33554.09999990463,26.875
1001,33578.49000000954,26.875
1002,33601.37999987602,26.875
1003,33625.34999990463,26.8125
1004,33648.27999997139,26.875
1005,33671.36999988556,26.875
1006,33694.37999987602,26.875
1007,33717.26999998093,26.8125
1008,33741.21000003815,26.8125
1009,33764.84999990463,26.8125
1010,33787.56999993324,26.8125
1011,33811.18000006676,26.8125
1012,33952.43000006676,26.875
1013,33976.33999991417,26.875
1014,34000.27999997139,26.875
1015,34023.84999990463,26.8125
1016,34047.02999997139,26.8125
1017,34071.06999993324,26.8125
1018,34095.19000005722,26.8125
1019,34118.74000000954,26.8125
1020,34142.94000005722,26.8125
1021,34165.889999866486,26.8125
1022,34189.420000076294,26.8125
1023,34213.81999993324,26.8125
1024,34238.30999994278,26.8125
1025,34348.75999999046,26.8125
1026,34373.06999993324,26.8125
1027,34396.33999991417,26.8125
1028,34419.36999988556,26.8125
1029,34444.079999923706,26.8125
1030,34468.26999998093,26.8125
1031,34492.0,26.8125
1032,34515.56999993324,26.8125
1033,34538.950000047684,26.8125
1034,34561.98000001907,26.8125
1035,34585.49000000954,26.8125
1036,34609.25999999046,26.8125
1037,34633.12999987602,26.8125
1038,34656.079999923706,26.8125
1039,34679.22000002861,26.8125
1040,34702.47000002861,26.8125
1041,34812.75,26.8125
1042,34837.56999993324,26.8125
1043,34860.73000001907,26.8125
1044,34884.39999985695,26.8125
1045,34908.11999988556,26.8125
1046,34931.80999994278,26.8125
1047,34955.50999999046,26.8125
1048,34979.06999993324,26.8125
1049,35002.33999991417,26.8125
1050,35026.389999866486,26.75
1051,35051.26999998093,26.8125
1052,35073.84999990463,26.8125
1053,35098.079999923706,26.8125
1054,35121.11999988556,26.8125
1055,35292.049999952316,26.8125
1056,35316.12999987602,26.8125
1057,35339.75,26.8125
1058,35364.59999990463,26.8125
1059,35387.78999996185,26.8125
1060,35411.80999994278,26.8125
1061,35435.21000003815,26.8125
1062,35458.21000003815,26.75
1063,35482.47000002861,26.75
1064,35506.27999997139,26.75
1065,35617.75999999046,26.75
1066,35642.200000047684,26.75
1067,35665.579999923706,26.75
1068,35688.94000005722,26.75
1069,35711.64999985695,26.75
1070,35734.52999997139,26.75
1071,35757.83999991417,26.75
1072,35782.81999993324,26.75
1073,35806.84999990463,26.75
1074,35830.74000000954,26.75
1075,35855.420000076294,26.75
1076,35879.08999991417,26.75
1077,36050.299999952316,26.8125
1078,36073.33999991417,26.75
1079,36096.920000076294,26.8125
1080,36120.23000001907,26.75
1081,36143.74000000954,26.8125
1082,36167.64999985695,26.8125
1083,36191.03999996185,26.75
1084,36215.03999996185,26.75
1085,36259.86999988556,26.75
1086,36284.01999998093,26.75
1087,36306.84999990463,26.75
1088,36329.950000047684,26.75
1089,36353.170000076294,26.75
1090,36464.03999996185,26.75
1091,36487.76999998093,26.75
1092,36511.34999990463,26.6875
1093,36535.06999993324,26.75
1094,36558.03999996185,26.75
1095,36581.41000008583,26.75
1096,36604.94000005722,26.6875
1097,36628.23000001907,26.6875
1098,36651.44000005722,26.6875
1099,36675.549999952316,26.75
1100,36698.37999987602,26.6875
1101,36722.52999997139,26.75
1102,36893.00999999046,26.75
1103,36916.80999994278,26.75
1104,36940.78999996185,26.75
1105,36964.5,26.75
1106,36987.26999998093,26.6875
1107,37011.549999952316,26.6875
1108,37034.86999988556,26.6875
1109,37058.71000003815,26.6875
1110,37082.37999987602,26.6875
1111,37106.27999997139,26.6875
1112,37130.47000002861,26.6875
1113,37153.72000002861,26.6875
1114,37178.30999994278,26.75
1115,37202.09999990463,26.6875
1116,37225.56999993324,26.6875
1117,37367.359999895096,26.6875
1118,37390.56999993324,26.6875
1119,37415.299999952316,26.6875
1120,37438.53999996185,26.6875
1121,37462.28999996185,26.6875
1122,37486.26999998093,26.6875
1123,37509.87999987602,26.6875
1124,37534.28999996185,26.6875
1125,37558.21000003815,26.6875
1126,37581.46000003815,26.6875
1127,37604.389999866486,26.6875
1128,37627.549999952316,26.6875
1129,37650.50999999046,26.6875
1130,37673.43000006676,26.6875
1131,37697.609999895096,26.6875
1132,37721.670000076294,26.6875
1133,37863.41000008583,26.6875
1134,37887.609999895096,26.6875
1135,37910.920000076294,26.6875
1136,37933.77999997139,26.625
1137,37957.109999895096,26.6875
1138,37980.64999985695,26.6875
1139,38003.66000008583,26.625
1140,38073.55999994278,26.625
1141,38096.55999994278,26.625
1142,38122.109999895096,26.625
1143,38144.80999994278,26.625
1144,38169.359999895096,26.625
1145,38281.49000000954,26.625
1146,38305.609999895096,26.6875
1147,38348.47000002861,26.625
1148,38372.56999993324,26.625
1149,38396.05999994278,26.625
1150,38419.86999988556,26.625
1151,38442.69000005722,26.625
1152,38465.609999895096,26.625
1153,38488.700000047684,26.625
1154,38512.34999990463,26.625
1155,38535.450000047684,26.625
1156,38560.049999952316,26.625
1157,38583.68000006676,26.625
1158,38725.41000008583,26.625
1159,38748.94000005722,26.625
1160,38771.859999895096,26.625
1161,38795.920000076294,26.625
1162,38819.33999991417,26.625
1163,38843.670000076294,26.625
1164,38867.609999895096,26.625
1165,38890.86999988556,26.625
1166,38915.05999994278,26.625
1167,38939.09999990463,26.625
1168,38963.69000005722,26.625
1169,38987.34999990463,26.5625
1170,39010.86999988556,26.625
1171,39153.43000006676,26.625
1172,39176.37999987602,26.625
1173,39201.06999993324,26.625
1174,39224.25,26.625
1175,39247.72000002861,26.625
1176,39270.829999923706,26.625
1177,39294.93000006676,26.625
1178,39318.48000001907,26.5625
1179,39342.109999895096,26.5625
1180,39366.18000006676,26.5625
1181,39414.24000000954,26.5625
1182,39439.06999993324,26.625
1183,39462.31999993324,26.5625
1184,39573.81999993324,26.625
1185,39597.76999998093,26.5625
1186,39621.30999994278,26.5625
1187,39645.23000001907,26.5625
1188,39668.80999994278,26.5625
1189,39692.56999993324,26.5625
1190,39716.12999987602,26.5625
1191,39740.89999985695,26.5625
1192,39765.139999866486,26.5625
1193,39789.75,26.5625
1194,39813.02999997139,26.5625
1195,39836.26999998093,26.5625
1196,39859.36999988556,26.5625
1197,39883.93000006676,26.5625
1198,39908.22000002861,26.5625
1199,39933.950000047684,26.5625
1200,39956.66000008583,26.5625
1201,40151.299999952316,26.5625
1202,40174.359999895096,26.5625
1203,40197.389999866486,26.5625
1204,40220.80999994278,26.5625
1205,40244.01999998093,26.5625
1206,40268.87999987602,26.5625
1207,40292.47000002861,26.5625
1208,40315.670000076294,26.5625
1209,40339.670000076294,26.5625
1210,40363.50999999046,26.5625
1211,40386.80999994278,26.5625
1212,40429.97000002861,26.5
1213,40453.50999999046,26.5625
1214,40477.62999987602,26.5625
1215,40619.25,26.5625
1216,40643.89999985695,26.5
1217,40667.14999985695,26.5
1218,40690.36999988556,26.5
1219,40713.670000076294,26.5
1220,40736.30999994278,26.5
1221,40760.609999895096,26.5
1222,40784.329999923706,26.5
1223,40808.36999988556,26.5
1224,40832.47000002861,26.5
1225,40856.829999923706,26.5
1226,40880.23000001907,26.5
1227,40903.829999923706,26.5
1228,40928.24000000954,26.5
1229,41040.18000006676,26.5
1230,41063.25,26.5
1231,41086.25999999046,26.5
1232,41109.48000001907,26.5
1233,41133.0,26.5
1234,41157.06999993324,26.5
1235,41180.39999985695,26.5
1236,41204.0,26.4375
1237,41227.08999991417,26.4375
1238,41250.00999999046,26.4375
1239,41274.200000047684,26.5
1240,41297.47000002861,26.5
1241,41320.420000076294,26.5
1242,41344.74000000954,26.4375
1243,41368.59999990463,26.5
1244,41392.52999997139,26.4375
1245,41504.5,26.4375
1246,41526.96000003815,26.5
1247,41551.5,26.4375
1248,41575.48000001907,26.4375
1249,41599.46000003815,26.4375
1250,41623.670000076294,26.4375
1251,41647.73000001907,26.4375
1252,41672.08999991417,26.4375
1253,41695.170000076294,26.4375
1254,41718.299999952316,26.4375
1255,41742.889999866486,26.4375
1256,41766.05999994278,26.4375
1257,41789.670000076294,26.4375
1258,41900.920000076294,26.4375
1259,41924.64999985695,26.4375
1260,41947.87999987602,26.4375
1261,41971.14999985695,26.4375
1262,41994.24000000954,26.4375
1263,42017.36999988556,26.4375
1264,42040.69000005722,26.4375
1265,42064.109999895096,26.4375
1266,42088.450000047684,26.4375
1267,42112.76999998093,26.4375
1268,42136.0,26.4375
1269,42160.12999987602,26.4375
1270,42183.89999985695,26.4375
1271,42208.049999952316,26.4375
1272,42231.33999991417,26.4375
1273,42432.049999952316,26.4375
1274,42455.12999987602,26.4375
1275,42478.24000000954,26.4375
1276,42501.30999994278,26.4375
1277,42525.27999997139,26.4375
1278,42548.47000002861,26.375
1279,42572.670000076294,26.4375
1280,42596.75999999046,26.4375
1281,42620.170000076294,26.4375
1282,42643.51999998093,26.4375
1283,42666.58999991417,26.4375
1284,42690.43000006676,26.375
1285,42760.359999895096,26.375
1286,42783.170000076294,26.375
1287,42807.24000000954,26.375
1288,42948.66000008583,26.4375
1289,42972.639999866486,26.4375
1290,42995.84999990463,26.375
1291,43019.91000008583,26.4375
1292,43044.12999987602,26.375
1293,43067.98000001907,26.375
1294,43091.49000000954,26.4375
1295,43115.50999999046,26.375
1296,43140.01999998093,26.375
1297,43163.74000000954,26.375
1298,43187.81999993324,26.375
1299,43211.049999952316,26.375
1300,43235.049999952316,26.375
1301,43259.19000005722,26.375
1302,43371.78999996185,26.375
1303,43395.5,26.375
1304,43418.26999998093,26.375
1305,43442.049999952316,26.375
1306,43465.299999952316,26.375
1307,43489.47000002861,26.375
1308,43513.62999987602,26.375
1309,43537.71000003815,26.375
1310,43561.61999988556,26.3125
1311,43584.700000047684,26.3125
1312,43609.06999993324,26.375
1313,43678.450000047684,26.3125
1314,43701.97000002861,26.375
1315,43813.91000008583,26.375
1316,43836.64999985695,26.375
1317,43861.76999998093,26.375
1318,43884.84999990463,26.3125
1319,43907.98000001907,26.375
1320,43932.23000001907,26.3125
1321,43956.450000047684,26.3125
1322,43981.12999987602,26.3125
1323,44004.34999990463,26.3125
1324,44027.48000001907,26.3125
1325,44050.86999988556,26.3125
1326,44073.609999895096,26.3125
1327,44097.549999952316,26.3125
1328,44120.48000001907,26.3125
1329,44143.23000001907,26.3125
1330,44166.389999866486,26.3125
1331,44190.139999866486,26.3125
1332,44391.36999988556,26.375
1333,44414.99000000954,26.375
1334,44438.86999988556,26.375
1335,44483.18000006676,26.3125
1336,44507.02999997139,26.3125
1337,44529.89999985695,26.375
1338,44553.99000000954,26.3125
1339,44577.549999952316,26.3125
1340,44601.55999994278,26.3125
1341,44625.83999991417,26.3125
1342,44669.48000001907,26.3125
1343,44693.56999993324,26.3125
1344,44716.859999895096,26.3125
1345,44740.22000002861,26.3125
1346,44764.450000047684,26.3125
1347,44935.73000001907,26.3125
1348,44958.96000003815,26.3125
1349,44982.84999990463,26.3125
1350,45052.00999999046,26.3125
1351,45075.80999994278,26.3125
1352,45099.579999923706,26.25
1353,45146.76999998093,26.3125
1354,45170.829999923706,26.3125
1355,45193.64999985695,26.3125
1356,45242.109999895096,26.3125
1357,45312.48000001907,26.25
1358,45514.420000076294,26.3125
1359,45538.16000008583,26.25
1360,45561.549999952316,26.25
1361,45585.24000000954,26.25
1362,45608.73000001907,26.25
1363,45631.72000002861,26.25
1364,45655.97000002861,26.25
1365,45679.62999987602,26.25
1366,45702.829999923706,26.25
1367,45727.80999994278,26.25
1368,45750.450000047684,26.25
1369,45774.53999996185,26.25
1370,45797.56999993324,26.25
1371,45821.34999990463,26.25
1372,45845.00999999046,26.25
1373,45868.96000003815,26.25
1374,46009.74000000954,26.25
1375,46033.859999895096,26.25
1376,46057.08999991417,26.25
1377,46080.609999895096,26.25
1378,46104.80999994278,26.25
1379,46153.329999923706,26.25
1380,46176.89999985695,26.25
1381,46200.80999994278,26.25
1382,46224.66000008583,26.1875
1383,46271.670000076294,26.25
1384,46464.200000047684,26.25
1385,46488.14999985695,26.25
1386,46511.43000006676,26.25
1387,46534.61999988556,26.25
1388,46557.609999895096,26.25
1389,46581.0,26.25
1390,46604.23000001907,26.25
1391,46627.37999987602,26.25
1392,46651.09999990463,26.25
1393,46674.639999866486,26.1875
1394,46698.139999866486,26.25
1395,46721.03999996185,26.1875
1396,46744.11999988556,26.25
1397,46768.170000076294,26.25
1398,46791.80999994278,26.25
1399,46934.11999988556,26.25
1400,46957.21000003815,26.1875
1401,46980.12999987602,26.25
1402,47004.08999991417,26.1875
1403,47026.829999923706,26.25
1404,47049.80999994278,26.1875
1405,47072.80999994278,26.1875
1406,47097.0,26.1875
1407,47119.98000001907,26.1875
1408,47144.14999985695,26.1875
1409,47167.28999996185,26.1875
1410,47192.27999997139,26.1875
1411,47216.18000006676,26.1875
1412,47239.99000000954,26.1875
1413,47263.72000002861,26.1875
1414,47375.46000003815,26.1875
1415,47398.53999996185,26.1875
1416,47421.44000005722,26.1875
1417,47445.26999998093,26.1875
1418,47468.93000006676,26.1875
1419,47492.25,26.1875
1420,47515.97000002861,26.1875
1421,47584.58999991417,26.1875
1422,47726.34999990463,26.1875
1423,47773.59999990463,26.1875
1424,47796.44000005722,26.1875
1425,47819.549999952316,26.1875
1426,47842.58999991417,26.1875
1427,47865.58999991417,26.1875
1428,47889.76999998093,26.1875
1429,47913.049999952316,26.1875
1430,47936.47000002861,26.1875
1431,47961.200000047684,26.125
1432,47984.25,26.125
1433,48008.55999994278,26.1875
1434,48032.670000076294,26.125
1435,48056.52999997139,26.1875
1436,48228.14999985695,26.1875
1437,48251.950000047684,26.1875
1438,48275.609999895096,26.1875
1439,48298.36999988556,26.1875
1440,48322.34999990463,26.1875
1441,48346.549999952316,26.1875
1442,48370.25,26.1875
1443,48393.579999923706,26.1875
1444,48417.200000047684,26.125
1445,48441.11999988556,26.1875
1446,48465.39999985695,26.1875
1447,48489.25,26.125
1448,48512.299999952316,26.125
1449,48536.22000002861,26.125
1450,48560.450000047684,26.125
1451,48584.31999993324,26.125
1452,48695.579999923706,26.125
1453,48719.950000047684,26.1875
1454,48742.59999990463,26.125
1455,48766.06999993324,26.1875
1456,48789.02999997139,26.125
1457,48813.30999994278,26.125
1458,48836.03999996185,26.125
1459,48860.50999999046,26.125
1460,48883.76999998093,26.125
1461,48906.28999996185,26.125
1462,48929.24000000954,26.125
1463,48953.98000001907,26.125
1464,48976.639999866486,26.125
1465,48999.51999998093,26.125
1466,49170.799999952316,26.125
1467,49194.68000006676,26.125
1468,49218.41000008583,26.125
1469,49243.049999952316,26.125
1470,49266.579999923706,26.125
1471,49290.53999996185,26.0625
1472,49314.5,26.125
1473,49338.59999990463,26.125
1474,49361.78999996185,26.0625
1475,49385.31999993324,26.125
1476,49409.39999985695,26.125
1477,49432.24000000954,26.125
1478,49456.21000003815,26.0625
1479,49479.27999997139,26.0625
1480,49502.87999987602,26.0625
1481,49735.139999866486,26.0625
1482,49759.61999988556,26.0625
1483,49782.62999987602,26.0625
1484,49806.170000076294,26.125
1485,49828.86999988556,26.0625
1486,49851.64999985695,26.0625
1487,49874.64999985695,26.0625
1488,49922.109999895096,26.0625
1489,49946.670000076294,26.0625
1490,49970.0,26.0625
1491,49994.049999952316,26.0625
1492,50017.71000003815,26.0625
1493,50041.81999993324,26.0625
1494,50064.64999985695,26.0625
1495,50296.19000005722,26.0625
1496,50319.00999999046,26.0625
1497,50342.98000001907,26.0625
1498,50366.84999990463,26.0625
1499,50389.76999998093,26.0625
1500,50413.08999991417,26.0625
1501,50437.37999987602,26.0625
1502,50460.76999998093,26.0625
1503,50484.56999993324,26.0625
1504,50509.299999952316,26.0625
1505,50532.80999994278,26.0625
1506,50556.77999997139,26.0
1507,50580.359999895096,26.0625
1508,50603.64999985695,26.0
1509,50626.87999987602,26.0
1510,50650.30999994278,26.0
1511,50792.64999985695,26.0625
1512,50817.079999923706,26.0
1513,50842.01999998093,26.0
1514,50867.18000006676,26.0
1515,50891.69000005722,26.0
1516,50914.77999997139,26.0
1517,50938.53999996185,26.0
1518,50962.99000000954,26.0
1519,50985.670000076294,26.0
1520,51008.670000076294,26.0
1521,51031.97000002861,26.0
1522,51144.549999952316,26.0
1523,51168.89999985695,26.0
1524,51191.99000000954,26.0
1525,51216.049999952316,26.0
1526,51238.72000002861,26.0
1527,51261.55999994278,26.0
1528,51284.33999991417,26.0
1529,51307.41000008583,26.0
1530,51330.299999952316,26.0
1531,51354.64999985695,26.0
1532,51378.299999952316,25.9375
1533,51402.139999866486,25.9375
1534,51426.24000000954,26.0
1535,51449.84999990463,26.0
1536,51473.700000047684,26.0
1537,51496.47000002861,25.9375
1538,51697.80999994278,26.0
1539,51720.91000008583,26.0
1540,51744.53999996185,25.9375
1541,51768.549999952316,25.9375
1542,51791.71000003815,25.9375
1543,51815.26999998093,25.9375
1544,51838.24000000954,25.9375
1545,51861.58999991417,25.9375
1546,51885.170000076294,25.9375
1547,51908.049999952316,25.9375
1548,51932.25,25.9375
1549,51955.36999988556,25.9375
1550,51979.450000047684,25.9375
1551,52003.61999988556,25.9375
1552,52026.99000000954,25.9375
1553,52138.72000002861,25.9375
1554,52161.68000006676,25.9375
1555,52185.52999997139,25.9375
1556,52208.359999895096,25.9375
1557,52231.41000008583,25.9375
1558,52254.420000076294,25.9375
1559,52277.49000000954,25.9375
1560,52300.76999998093,25.9375
1561,52323.98000001907,25.9375
1562,52347.25,25.9375
1563,52369.86999988556,25.9375
1564,52393.0,25.9375
1565,52416.28999996185,25.9375
1566,52588.31999993324,25.9375
1567,52611.91000008583,25.9375
1568,52635.549999952316,25.9375
1569,52658.36999988556,25.9375
1570,52682.21000003815,25.9375
1571,52706.609999895096,25.9375
1572,52729.47000002861,25.9375
1573,52752.01999998093,25.875
1574,52775.670000076294,25.875
1575,52798.75,25.875
1576,52821.78999996185,25.875
1577,52845.62999987602,25.875
1578,52869.21000003815,25.875
1579,52892.69000005722,25.875
1580,52916.329999923706,25.875
1581,53088.02999997139,25.9375
1582,53158.75,25.875
1583,53181.97000002861,25.875
1584,53205.78999996185,25.875
1585,53229.77999997139,25.9375
1586,53254.079999923706,25.875
1587,53277.73000001907,25.875
1588,53300.91000008583,25.875
1589,53324.05999994278,25.875
1590,53346.889999866486,25.875
1591,53458.89999985695,25.875
1592,53482.64999985695,25.875
1593,53506.28999996185,25.875
1594,53529.579999923706,25.875
1595,53578.59999990463,25.875
1596,53601.72000002861,25.875
1597,53625.99000000954,25.875
1598,53648.950000047684,25.875
1599,53672.89999985695,25.875
1600,53696.74000000954,25.875
1601,53720.01999998093,25.875
1602,53742.72000002861,25.875
1603,53766.299999952316,25.875
1604,53789.26999998093,25.875
1605,53812.21000003815,25.875
1606,53922.94000005722,25.875
1607,53945.86999988556,25.875
1608,53968.83999991417,25.8125
1609,53993.389999866486,25.875
1610,54017.96000003815,25.875
1611,54041.06999993324,25.875
1612,54064.75,25.8125
1613,54088.03999996185,25.875
1614,54112.139999866486,25.8125
1615,54136.049999952316,25.8125
1616,54159.22000002861,25.8125
1617,54300.5,25.8125
1618,54324.26999998093,25.8125
1619,54348.049999952316,25.8125
1620,54371.93000006676,25.8125
1621,54394.81999993324,25.8125
1622,54417.76999998093,25.8125
1623,54442.56999993324,25.8125
1624,54466.39999985695,25.8125
1625,54537.09999990463,25.8125
1626,54560.18000006676,25.8125
1627,54583.200000047684,25.8125
1628,54695.00999999046,25.8125
1629,54718.33999991417,25.8125
1630,54742.52999997139,25.8125
1631,54765.77999997139,25.8125
1632,54789.96000003815,25.8125
1633,54812.97000002861,25.8125
1634,54836.670000076294,25.8125
1635,54860.31999993324,25.8125
1636,54883.81999993324,25.8125
1637,54907.670000076294,25.8125
1638,54931.0,25.8125
1639,54954.0,25.8125
1640,54977.00999999046,25.75
1641,55088.950000047684,25.8125
1642,55113.24000000954,25.8125
1643,55135.77999997139,25.8125
1644,55159.68000006676,25.8125
1645,55183.53999996185,25.75
1646,55207.170000076294,25.8125
1647,55230.68000006676,25.75
1648,55254.950000047684,25.8125
1649,55279.11999988556,25.75
1650,55301.86999988556,25.8125
1651,55325.84999990463,25.75
1652,55350.46000003815,25.75
1653,55375.079999923706,25.75
1654,55398.26999998093,25.8125
1655,55540.58999991417,25.8125
1656,55563.53999996185,25.75
1657,55586.36999988556,25.75
1658,55633.74000000954,25.75
1659,55657.59999990463,25.75
1660,55680.68000006676,25.75
1661,55704.609999895096,25.75
1662,55727.889999866486,25.75
1663,55751.170000076294,25.75
1664,55775.639999866486,25.75
1665,55800.25999999046,25.75
1666,55824.34999990463,25.75
1667,55848.200000047684,25.75
1668,55871.01999998093,25.75
1669,55982.079999923706,25.75
1670,56006.06999993324,25.75
1671,56029.33999991417,25.75
1672,56053.049999952316,25.75
1673,56075.94000005722,25.75
1674,56100.06999993324,25.75
1675,56123.170000076294,25.75
1676,56146.16000008583,25.75
1677,56169.18000006676,25.75
1678,56193.11999988556,25.75
1679,56239.799999952316,25.75
1680,56264.450000047684,25.75
1681,56287.59999990463,25.75
1682,56311.14999985695,25.75
1683,56452.89999985695,25.6875
1684,56475.93000006676,25.6875
1685,56500.049999952316,25.6875
1686,56524.33999991417,25.6875
1687,56548.18000006676,25.6875
1688,56572.5,25.75
1689,56597.08999991417,25.6875
1690,56620.44000005722,25.75
1691,56643.26999998093,25.6875
1692,56667.78999996185,25.6875
1693,56691.26999998093,25.6875
1694,56714.87999987602,25.6875
1695,56916.00999999046,25.75
1696,56939.26999998093,25.75
1697,56962.93000006676,25.75
1698,56986.53999996185,25.6875
1699,57010.61999988556,25.75
1700,57033.76999998093,25.6875
1701,57057.670000076294,25.6875
1702,57081.579999923706,25.6875
1703,57104.19000005722,25.6875
1704,57127.11999988556,25.6875
1705,57150.23000001907,25.6875
1706,57174.00999999046,25.6875
1707,57197.72000002861,25.6875
1708,57221.80999994278,25.6875
1709,57363.74000000954,25.6875
1710,57386.52999997139,25.6875
1711,57409.78999996185,25.6875
1712,57433.359999895096,25.6875
1713,57457.52999997139,25.6875
1714,57480.579999923706,25.6875
1715,57504.53999996185,25.6875
1716,57527.77999997139,25.6875
1717,57551.37999987602,25.6875
1718,57575.06999993324,25.6875
1719,57598.329999923706,25.6875
1720,57622.139999866486,25.6875
1721,57645.81999993324,25.6875
1722,57668.84999990463,25.6875
1723,57693.08999991417,25.6875
1724,57804.76999998093,25.6875
1725,57828.68000006676,25.6875
1726,57852.33999991417,25.6875
1727,57875.43000006676,25.6875
1728,57898.62999987602,25.6875
1729,57922.200000047684,25.625
1730,57945.41000008583,25.625
1731,57968.48000001907,25.6875
1732,57992.5,25.6875
1733,58016.75,25.6875
1734,58040.389999866486,25.6875
1735,58063.78999996185,25.6875
1736,58091.22000002861,25.6875
1737,58113.71000003815,25.6875
1738,58136.75,25.625
1739,58160.69000005722,25.6875
1740,58184.72000002861,25.625
1741,58326.16000008583,25.6875
1742,58349.889999866486,25.6875
1743,58372.72000002861,25.625
1744,58395.71000003815,25.625
1745,58419.44000005722,25.625
1746,58442.47000002861,25.625
1747,58466.43000006676,25.625
1748,58490.420000076294,25.625
1749,58514.18000006676,25.625
1750,58537.049999952316,25.625
1751,58560.18000006676,25.625
1752,58583.31999993324,25.625
1753,58694.25999999046,25.625
1754,58717.05999994278,25.625
1755,58764.049999952316,25.625
1756,58787.81999993324,25.625
1757,58811.389999866486,25.625
1758,58835.41000008583,25.625
1759,58858.799999952316,25.625
1760,58882.47000002861,25.625
1761,58905.64999985695,25.625
1762,58929.700000047684,25.625
1763,58953.73000001907,25.625
1764,58977.56999993324,25.625
1765,59003.889999866486,25.625
1766,59234.21000003815,25.625
1767,59256.83999991417,25.625
1768,59280.97000002861,25.625
1769,59303.91000008583,25.625
1770,59327.71000003815,25.625
1771,59350.73000001907,25.625
1772,59373.99000000954,25.625
1773,59397.639999866486,25.5625
1774,59420.69000005722,25.5625
1775,59445.06999993324,25.625
1776,59469.109999895096,25.625
1777,59492.14999985695,25.625
1778,59627.18000006676,25.625
1779,59650.450000047684,25.625
1780,59698.0,25.625
1781,59721.22000002861,25.5625
1782,59743.93000006676,25.625
1783,59767.86999988556,25.625
1784,59791.579999923706,25.625
1785,59815.06999993324,25.5625
1786,59838.98000001907,25.625
1787,59862.18000006676,25.5625
1788,59886.84999990463,25.625
1789,59912.78999996185,25.5625
1790,59936.670000076294,25.5625
1791,59959.920000076294,25.625
1792,59983.36999988556,25.625
1793,60103.889999866486,25.625
1794,60127.99000000954,25.5625
1795,60151.78999996185,25.5625
1796,60174.420000076294,25.5625
1797,60198.26999998093,25.5625
1798,60222.170000076294,25.5625
1799,60245.420000076294,25.5625
1800,60269.30999994278,25.5625
1801,60293.47000002861,25.5625
1802,60317.05999994278,25.5625
1803,60339.91000008583,25.5625
1804,60363.97000002861,25.5625
1805,60388.12999987602,25.5625
1806,60411.329999923706,25.5625
1807,60522.71000003815,25.5625
1808,60546.84999990463,25.5625
1809,60570.0,25.5625
1810,60593.83999991417,25.5625
1811,60616.71000003815,25.5625
1812,60640.670000076294,25.5625
1813,60664.80999994278,25.5625
1814,60687.75,25.5625
1815,60711.77999997139,25.5625
1816,60735.37999987602,25.5625
1817,60758.91000008583,25.5625
1818,60783.34999990463,25.5625
1819,60807.75,25.5625
1820,60831.69000005722,25.5625
1821,60854.859999895096,25.5625
1822,60878.11999988556,25.5625
1823,61029.76999998093,25.5625
1824,61052.87999987602,25.5625
1825,61076.77999997139,25.5625
1826,61100.99000000954,25.5625
1827,61124.72000002861,25.5625
1828,61148.34999990463,25.5625
1829,61172.30999994278,25.5625
1830,61195.48000001907,25.5625
1831,61218.75999999046,25.5625
1832,61243.450000047684,25.5625
1833,61266.56999993324,25.5625
1834,61289.37999987602,25.5625
1835,61312.84999990463,25.5625
1836,61337.36999988556,25.5625
1837,61360.0,25.5625
1838,61384.12999987602,25.5625
1839,61408.170000076294,25.5625
1840,61622.450000047684,25.5625
1841,61646.84999990463,25.5625
1842,61669.81999993324,25.5625
1843,61692.94000005722,25.5625
1844,61716.23000001907,25.5625
1845,61739.37999987602,25.5625
1846,61762.920000076294,25.5625
1847,61786.47000002861,25.5625
1848,61811.079999923706,25.5625
1849,61834.26999998093,25.5625
1850,61857.829999923706,25.5
1851,61880.920000076294,25.5
1852,61904.920000076294,25.5625
1853,61928.77999997139,25.5625
1854,61951.53999996185,25.5625
1855,62062.609999895096,25.5625
1856,62085.75999999046,25.5625
1857,62109.700000047684,25.5625
1858,62132.73000001907,25.5625
1859,62155.5,25.5625
1860,62179.01999998093,25.5625
1861,62201.71000003815,25.5625
1862,62225.139999866486,25.5625
1863,62249.24000000954,25.5625
1864,62273.01999998093,25.5625
1865,62295.86999988556,25.5625
1866,62319.89999985695,25.5625
1867,62343.06999993324,25.5625
1868,62366.670000076294,25.5625
1869,62389.83999991417,25.5625
1870,62435.359999895096,25.5625
1871,62458.139999866486,25.5625
1872,62599.609999895096,25.5625
1873,62622.80999994278,25.5625
1874,62646.01999998093,25.5625
1875,62669.889999866486,25.5625
1876,62693.639999866486,25.5625
1877,62717.39999985695,25.5625
1878,62741.46000003815,25.5625
1879,62764.77999997139,25.5
1880,62788.91000008583,25.5625
1881,62813.06999993324,25.5625
1882,62837.26999998093,25.5625
1883,62861.139999866486,25.5
1884,62884.25,25.5
1885,62908.41000008583,25.5
1886,62931.14999985695,25.5625
1887,62954.25,25.5
1888,62977.639999866486,25.5625
1889,63148.77999997139,25.5625
1890,63172.00999999046,25.5625
1891,63195.609999895096,25.5625
1892,63219.64999985695,25.5625
1893,63242.700000047684,25.5625
1894,63266.28999996185,25.5625
1895,63290.39999985695,25.5625
1896,63314.200000047684,25.5625
1897,63337.579999923706,25.5625
1898,63361.09999990463,25.5625
1899,63384.24000000954,25.5625
1900,63408.47000002861,25.5625
1901,63431.71000003815,25.5625
1902,63455.19000005722,25.5625
1903,63478.97000002861,25.5625
1904,63679.579999923706,25.5
1905,63703.03999996185,25.5625
1906,63726.80999994278,25.5625
1907,63749.609999895096,25.5625
1908,63772.700000047684,25.5625
1909,63797.28999996185,25.5625
1910,63821.049999952316,25.5625
1911,63844.609999895096,25.5625
1912,63867.670000076294,25.5625
1913,63891.93000006676,25.5625
1914,63915.06999993324,25.5625
1915,63939.21000003815,25.5625
1916,63962.93000006676,25.5625
1917,63986.93000006676,25.5625
1918,64129.14999985695,25.5625
1919,64152.81999993324,25.5625
1920,64176.93000006676,25.5625
1921,64200.36999988556,25.5625
1922,64223.670000076294,25.5625
1923,64247.829999923706,25.5625
1924,64272.06999993324,25.5625
1925,64295.12999987602,25.5625
1926,64318.139999866486,25.5625
1927,64341.06999993324,25.5625
1928,64364.829999923706,25.5625
1929,64388.01999998093,25.5625
1930,64411.22000002861,25.5625
1931,64553.33999991417,25.5625
1932,64576.34999990463,25.5625
1933,64600.11999988556,25.5625
1934,64623.78999996185,25.5625
1935,64646.609999895096,25.5625
1936,64669.83999991417,25.5625
1937,64692.69000005722,25.5625
1938,64716.12999987602,25.5625
1939,64739.25,25.5625
1940,64761.98000001907,25.5625
1941,64785.450000047684,25.5625
1942,64810.80999994278,25.5625
1943,64834.0,25.5625
1944,64857.34999990463,25.5625
1945,64881.52999997139,25.5625
1946,64993.27999997139,25.5625
1947,65016.23000001907,25.5625
1948,65039.420000076294,25.5625
1949,65063.420000076294,25.5625
1950,65087.86999988556,25.5625
1951,65111.71000003815,25.5625
1952,65134.47000002861,25.5625
1953,65157.27999997139,25.5625
1954,65181.079999923706,25.5625
1955,65204.43000006676,25.5625
1956,65227.5,25.5625
1957,65251.11999988556,25.5625
1958,65274.0,25.5625
1959,65297.72000002861,25.5625
1960,65321.200000047684,25.5625
1961,65344.81999993324,25.5625
1962,65554.29999995232,25.5625
1963,65577.34999990463,25.5625
1964,65600.26999998093,25.5625
1965,65623.21000003815,25.5625
1966,65647.3299999237,25.5625
1967,65670.94000005722,25.5625
1968,65694.62999987602,25.5625
1969,65718.73000001907,25.5625
1970,65742.13999986649,25.5625
1971,65765.23000001907,25.5625
1972,65812.8299999237,25.5
1973,65837.44000005722,25.5625
1974,66008.78999996185,25.5
1975,66031.97000002861,25.5
1976,66055.5,25.5
1977,66078.58999991417,25.5
1978,66101.79999995232,25.5
1979,66125.48000001907,25.5
1980,66148.46000003815,25.5
1981,66172.41000008583,25.5
1982,66196.08999991417,25.5
1983,66219.99000000954,25.5
1984,66243.37999987602,25.5
1985,66269.02999997139,25.5
1986,66292.13999986649,25.5
1987,66316.19000005722,25.5
1988,66427.62999987602,25.4375
1989,66451.48000001907,25.5
1990,66474.38999986649,25.5
1991,66497.62999987602,25.4375
1992,66520.31999993324,25.5
1993,66544.53999996185,25.5
1994,66567.8299999237,25.5
1995,66591.29999995232,25.5
1996,66615.26999998093,25.5
1997,66638.49000000954,25.5
1998,66662.84999990463,25.5
1999,66685.84999990463,25.5
2000,66827.66000008583,25.5
2001,66850.58999991417,25.5
2002,66874.3299999237,25.5
2003,66898.4200000763,25.5
2004,66922.47000002861,25.5
2005,66946.47000002861,25.5
2006,66969.80999994278,25.5
2007,66994.6099998951,25.5
2008,67018.97000002861,25.5
2009,67043.31999993324,25.5
2010,67067.6700000763,25.5
2011,67091.88999986649,25.5
2012,67264.43000006676,25.5
2013,67288.21000003815,25.5625
2014,67312.37999987602,25.5
2015,67337.13999986649,25.5
2016,67361.22000002861,25.5625
2017,67384.79999995232,25.5
2018,67408.87999987602,25.5
2019,67431.77999997139,25.5
2020,67455.69000005722,25.5
2021,67479.89999985695,25.5625
2022,67503.4200000763,25.5625
2023,67527.5,25.5
2024,67550.70000004768,25.5625
2025,67574.96000003815,25.5625
2026,67688.43000006676,25.5625
2027,67711.49000000954,25.5625
2028,67758.53999996185,25.5625
2029,67782.36999988556,25.5625
2030,67805.73000001907,25.5625
2031,67829.23000001907,25.5625
2032,67852.61999988556,25.5625
2033,67876.16000008583,25.5625
2034,67899.30999994278,25.5625
2035,67922.51999998093,25.5625
2036,67945.54999995232,25.5625
2037,67968.5,25.5625
2038,67991.50999999046,25.625
2039,68136.8599998951,25.625
2040,68161.25,25.625
2041,68185.14999985695,25.5625
2042,68208.9200000763,25.625
2043,68233.00999999046,25.5625
2044,68256.78999996185,25.625
2045,68280.30999994278,25.625
0,68671.45000004768,25.6875
1,68695.61999988556,25.6875
2,68720.47000002861,25.6875
3,68743.06999993324,25.6875
4,68767.4200000763,25.6875
5,68790.63999986649,25.6875
6,68814.81999993324,25.6875
7,68839.47000002861,25.625
8,68863.53999996185,25.625
9,68886.14999985695,25.6875
10,68910.00999999046,25.625
11,68933.25999999046,25.625
12,68956.01999998093,25.625
13,68980.49000000954,25.6875
14,69003.41000008583,25.6875
15,69145.69000005722,25.6875
16,69169.31999993324,25.6875
17,69193.18000006676,25.6875
18,69263.96000003815,25.6875
19,69287.81999993324,25.6875
20,69311.74000000954,25.6875
21,69334.47000002861,25.6875
22,69358.70000004768,25.6875
23,69381.96000003815,25.6875
24,69405.5799999237,25.6875
25,69430.44000005722,25.6875
26,69453.14999985695,25.6875
27,69593.75,25.6875
28,69618.11999988556,25.6875
29,69641.72000002861,25.6875
30,69665.48000001907,25.6875
31,69688.46000003815,25.6875
32,69712.16000008583,25.6875
33,69736.19000005722,25.6875
34,69759.86999988556,25.6875
35,69783.47000002861,25.6875
36,69807.50999999046,25.6875
37,69830.48000001907,25.6875
38,69853.69000005722,25.6875
39,69877.26999998093,25.6875
40,69901.72000002861,25.6875
41,70012.1099998951,25.6875
42,70035.0,25.6875
43,70059.0799999237,25.6875
44,70083.5,25.6875
45,70107.70000004768,25.6875
46,70130.81999993324,25.6875
47,70154.13999986649,25.6875
48,70176.84999990463,25.6875
49,70201.09999990463,25.6875
50,70225.59999990463,25.6875
51,70248.50999999046,25.6875
52,70272.45000004768,25.75
53,70295.33999991417,25.6875
54,70318.1099998951,25.75
55,70341.06999993324,25.75
56,70364.8299999237,25.75
57,70536.1700000763,25.75
58,70558.62999987602,25.75
59,70582.79999995232,25.75
60,70606.8599998951,25.75
61,70630.37999987602,25.75
62,70654.66000008583,25.75
63,70678.76999998093,25.75
64,70701.77999997139,25.75
65,70725.77999997139,25.75
66,70749.26999998093,25.75
67,70772.44000005722,25.75
68,70796.05999994278,25.75
69,70906.98000001907,25.75
70,70930.54999995232,25.75
71,70953.63999986649,25.75
72,70976.76999998093,25.75
73,71000.98000001907,25.75
74,71024.30999994278,25.8125
75,71047.04999995232,25.8125
76,71172.77999997139,25.75
77,71197.25999999046,25.75
78,71220.59999990463,25.8125
79,71243.23000001907,25.8125
80,71267.11999988556,25.8125
81,71437.96000003815,25.8125
82,71462.0799999237,25.8125
83,71485.98000001907,25.8125
84,71509.00999999046,25.8125
85,71532.25999999046,25.8125
86,71555.01999998093,25.8125
87,71579.37999987602,25.8125
88,71602.63999986649,25.8125
89,71626.78999996185,25.8125
90,71650.06999993324,25.8125
91,71672.98000001907,25.8125
92,71695.6700000763,25.8125
93,71720.31999993324,25.8125
94,71743.41000008583,25.8125
95,71766.44000005722,25.8125
96,71790.4200000763,25.8125
97,71814.58999991417,25.8125
98,71986.86999988556,25.875
99,72009.8299999237,25.8125
100,72032.91000008583,25.8125
101,72056.13999986649,25.875
102,72078.81999993324,25.8125
103,72102.33999991417,25.875
104,72126.27999997139,25.8125
105,72149.31999993324,25.875
106,72172.88999986649,25.875
107,72196.94000005722,25.8125
108,72220.11999988556,25.8125
109,72243.29999995232,25.8125
110,72267.20000004768,25.875
111,72290.3299999237,25.875
112,72313.99000000954,25.875
113,72455.29999995232,25.875
114,72479.31999993324,25.875
115,72502.0799999237,25.875
116,72526.25999999046,25.875
117,72549.97000002861,25.875
118,72574.31999993324,25.875
119,72598.71000003815,25.875
120,72623.58999991417,25.875
121,72646.24000000954,25.875
122,72669.5,25.875
123,72693.39999985695,25.875
124,72716.4200000763,25.875
125,72740.1700000763,25.875
126,72762.80999994278,25.875
127,72785.59999990463,25.875
128,72808.53999996185,25.875
129,72832.46000003815,25.875
130,72855.09999990463,25.875
131,73085.6700000763,25.9375
132,73109.71000003815,25.9375
133,73132.6700000763,25.9375
134,73156.5799999237,25.9375
135,73180.27999997139,25.9375
136,73204.08999991417,25.9375
137,73227.13999986649,25.9375
138,73250.50999999046,25.9375
139,73274.59999990463,25.9375
140,73298.25999999046,25.9375
141,73321.36999988556,25.9375
142,73344.68000006676,25.875
143,73367.44000005722,25.9375
144,73390.28999996185,25.9375
145,73592.28999996185,25.9375
146,73664.19000005722,25.9375
147,73688.34999990463,25.9375
148,73730.09999990463,25.9375
149,73754.28999996185,25.9375
150,73801.41000008583,25.9375
151,73824.79999995232,25.9375
152,73848.0,25.9375
153,73872.44000005722,25.9375
154,73896.53999996185,25.9375
155,73919.18000006676,25.875
156,74060.69000005722,25.9375
157,74083.96000003815,25.9375
158,74106.87999987602,25.9375
159,74131.04999995232,25.9375
160,74153.8599998951,25.9375
161,74178.39999985695,25.9375
162,74201.61999988556,26.0
163,74225.03999996185,25.9375
164,74248.20000004768,26.0
165,74271.1700000763,25.9375
166,74294.83999991417,25.9375
167,74318.93000006676,25.9375
168,74341.53999996185,25.9375
169,74453.89999985695,26.0
170,74500.75999999046,25.9375
171,74524.12999987602,25.9375
172,74546.95000004768,25.9375
173,74570.83999991417,26.0
174,74593.95000004768,26.0
175,74618.8299999237,25.9375
176,74642.76999998093,25.9375
177,74666.48000001907,25.9375
178,74689.18000006676,26.0
179,74860.18000006676,26.0
180,74883.36999988556,26.0
181,74907.14999985695,26.0
182,74931.53999996185,26.0625
183,74954.69000005722,26.0
184,74978.34999990463,26.0
185,75001.43000006676,26.0
186,75025.1099998951,26.0
187,75048.55999994278,26.0
188,75071.97000002861,26.0
189,75095.27999997139,26.0
190,75118.84999990463,26.0
191,75141.53999996185,26.0
192,75165.62999987602,26.0625
193,75188.59999990463,26.0
194,75300.25999999046,26.0625
195,75324.49000000954,26.0625
196,75348.97000002861,26.0
197,75372.04999995232,26.0625
198,75396.55999994278,26.0625
199,75420.39999985695,26.0
200,75443.45000004768,26.0625
201,75466.3599998951,26.0625
202,75490.51999998093,26.0625
203,75514.5799999237,26.0
204,75538.49000000954,26.0625
205,75562.14999985695,26.0625
206,75585.51999998093,26.0625
207,75609.81999993324,26.0625
208,75720.39999985695,26.0625
209,75743.24000000954,26.0625
210,75766.66000008583,26.0625
211,75789.56999993324,26.0625
212,75814.44000005722,26.0625
213,75837.44000005722,26.0625
214,75862.51999998093,26.0625
215,75886.22000002861,26.0625
216,75933.45000004768,26.0625
217,75956.03999996185,26.0625
218,75979.0,26.0625
219,76002.76999998093,26.0625
220,76026.54999995232,26.0625
221,76049.70000004768,26.0625
222,76250.25999999046,26.125
223,76274.39999985695,26.125
224,76297.1099998951,26.125
225,76319.80999994278,26.125
226,76344.44000005722,26.125
227,76368.37999987602,26.125
228,76392.24000000954,26.125
229,76415.48000001907,26.125
230,76438.84999990463,26.125
231,76462.9200000763,26.125
232,76486.8599998951,26.125
233,76510.98000001907,26.125
234,76534.89999985695,26.125
235,76558.44000005722,26.125
236,76729.9200000763,26.125
237,76753.89999985695,26.125
238,76776.37999987602,26.1875
239,76800.47000002861,26.125
240,76824.69000005722,26.125
241,76847.49000000954,26.125
242,76892.43000006676,26.1875
243,76916.13999986649,26.1875
244,76939.54999995232,26.1875
245,76962.94000005722,26.1875
246,77033.63999986649,26.1875
247,77057.54999995232,26.1875
248,77080.59999990463,26.1875
249,77298.22000002861,26.1875
250,77322.03999996185,26.1875
251,77344.86999988556,26.1875
252,77367.73000001907,26.1875
253,77390.56999993324,26.1875
254,77413.52999997139,26.1875
255,77438.34999990463,26.1875
256,77461.68000006676,26.1875
257,77485.00999999046,26.1875
258,77509.75999999046,26.1875
259,77681.29999995232,26.25
260,77704.99000000954,26.25
261,77728.44000005722,26.25
262,77751.89999985695,26.1875
263,77775.08999991417,26.1875
264,77797.87999987602,26.1875
265,77820.83999991417,26.25
266,77843.91000008583,26.25
267,77868.11999988556,26.25
268,77891.93000006676,26.25
269,77916.22000002861,26.25
270,77939.88999986649,26.25
271,77963.94000005722,26.25
272,77986.54999995232,26.1875
273,78097.88999986649,26.25
274,78120.70000004768,26.25
275,78143.84999990463,26.25
276,78166.48000001907,26.25
277,78190.4200000763,26.25
278,78213.59999990463,26.25
279,78237.41000008583,26.25
280,78260.24000000954,26.25
281,78283.11999988556,26.25
282,78307.28999996185,26.25
283,78330.1700000763,26.25
284,78353.99000000954,26.25
285,78378.91000008583,26.25
286,78403.04999995232,26.25
287,78427.25,26.25
288,78450.75,26.25
289,78475.72000002861,26.25
290,78616.37999987602,26.25
291,78640.63999986649,26.25
292,78664.88999986649,26.3125
293,78688.8599998951,26.25
294,78712.86999988556,26.25
295,78735.99000000954,26.25
296,78784.26999998093,26.25
297,78807.47000002861,26.3125
298,78830.29999995232,26.3125
299,78853.24000000954,26.25
300,78876.27999997139,26.25
301,78900.14999985695,26.3125
302,78923.74000000954,26.3125
303,78947.13999986649,26.25
304,78971.41000008583,26.3125
305,79112.06999993324,26.3125
306,79136.25,26.3125
307,79159.61999988556,26.3125
308,79183.68000006676,26.3125
309,79206.41000008583,26.3125
310,79229.25,26.3125
311,79253.39999985695,26.3125
312,79277.47000002861,26.3125
313,79301.20000004768,26.3125
314,79413.29999995232,26.375
315,79436.3599998951,26.375
316,79460.24000000954,26.3125
317,79483.22000002861,26.3125
318,79506.59999990463,26.3125
319,79531.4200000763,26.3125
320,79554.39999985695,26.375
321,79577.26999998093,26.375
322,79601.56999993324,26.3125
323,79624.8599998951,26.375
324,79648.1700000763,26.375
325,79671.55999994278,26.375
326,79695.3599998951,26.375
327,79719.02999997139,26.375
328,79742.11999988556,26.375
329,79853.47000002861,26.375
330,79878.24000000954,26.375
331,79902.1700000763,26.375
332,79925.91000008583,26.375
333,79949.46000003815,26.375
334,79972.36999988556,26.375
335,79995.25,26.375
336,80019.37999987602,26.375
337,80043.49000000954,26.375
338,80067.5799999237,26.375
339,80091.25999999046,26.375
340,80114.99000000954,26.375
341,80138.26999998093,26.4375
342,80162.33999991417,26.4375
343,80185.1700000763,26.4375
344,80296.47000002861,26.4375
345,80320.25999999046,26.4375
346,80343.0,26.4375
347,80366.25999999046,26.4375
348,80390.05999994278,26.4375
349,80413.63999986649,26.4375
350,80436.87999987602,26.4375
351,80460.1700000763,26.4375
352,80484.24000000954,26.4375
353,80507.24000000954,26.4375
354,80529.94000005722,26.4375
355,80552.75,26.4375
356,80576.91000008583,26.4375
357,80600.30999994278,26.4375
358,80623.96000003815,26.5
359,80735.78999996185,26.4375
360,80758.6700000763,26.5
361,80781.69000005722,26.4375
362,80805.05999994278,26.5
363,80828.98000001907,26.4375
364,80852.20000004768,26.4375
365,80875.41000008583,26.5
366,80898.95000004768,26.5
367,80923.20000004768,26.5
368,80946.87999987602,26.5
369,80969.70000004768,26.5
370,80992.50999999046,26.5
371,81015.47000002861,26.5
372,81038.94000005722,26.5
373,81149.58999991417,26.5
374,81173.21000003815,26.5
375,81197.31999993324,26.5
376,81221.44000005722,26.5
377,81245.20000004768,26.5
378,81269.5,26.5
379,81292.61999988556,26.5
380,81316.5,26.5
381,81340.13999986649,26.5
382,81363.63999986649,26.5625
383,81387.00999999046,26.5625
384,81411.83999991417,26.5
385,81523.25999999046,26.5625
386,81547.69000005722,26.5625
387,81571.39999985695,26.5625
388,81595.66000008583,26.5625
389,81619.64999985695,26.5625
390,81643.68000006676,26.5625
391,81666.93000006676,26.5625
392,81691.5799999237,26.5625
393,81735.48000001907,26.5625
394,81758.01999998093,26.5625
395,81781.29999995232,26.5625
396,81804.98000001907,26.5625
397,81828.09999990463,26.5625
398,82029.75,26.625
399,82054.12999987602,26.625
400,82077.13999986649,26.625
401,82101.09999990463,26.625
402,82124.22000002861,26.625
403,82147.53999996185,26.625
404,82170.75999999046,26.625
405,82193.5,26.625
406,82217.48000001907,26.625
407,82240.81999993324,26.625
408,82264.46000003815,26.625
409,82287.81999993324,26.625
410,82310.51999998093,26.625
411,82481.89999985695,26.625
412,82505.21000003815,26.625
413,82529.25,26.625
414,82552.83999991417,26.625
415,82575.64999985695,26.625
416,82598.89999985695,26.625
417,82622.75,26.625
418,82646.68000006676,26.6875
419,82670.58999991417,26.625
420,82694.94000005722,26.625
421,82717.98000001907,26.625
422,82741.76999998093,26.625
423,82764.75999999046,26.6875
424,82787.79999995232,26.6875
425,82811.69000005722,26.6875
426,82982.81999993324,26.6875
427,83006.44000005722,26.6875
428,83030.44000005722,26.6875
429,83053.44000005722,26.6875
430,83077.14999985695,26.6875
431,83100.23000001907,26.6875
432,83123.33999991417,26.6875
433,83146.30999994278,26.6875
434,83169.50999999046,26.6875
435,83193.50999999046,26.6875
436,83217.41000008583,26.6875
437,83240.59999990463,26.6875
438,83263.75,26.6875
439,83286.9200000763,26.6875
440,83310.91000008583,26.6875
441,83334.79999995232,26.6875
442,83358.01999998093,26.6875
443,83529.6099998951,26.6875
444,83553.49000000954,26.6875
445,83576.86999988556,26.6875
446,83599.75,26.6875
447,83622.83999991417,26.6875
448,83646.95000004768,26.6875
449,83669.71000003815,26.6875
450,83692.75999999046,26.6875
451,83763.41000008583,26.75
452,83787.5799999237,26.75
453,83810.94000005722,26.75
454,83952.62999987602,26.75
455,83976.74000000954,26.75
456,84000.56999993324,26.75
457,84024.53999996185,26.75
458,84048.24000000954,26.75
459,84072.75999999046,26.75
460,84096.45000004768,26.75
461,84120.38999986649,26.75
462,84143.26999998093,26.75
463,84167.76999998093,26.75
464,84190.83999991417,26.75
465,84213.89999985695,26.75
466,84237.83999991417,26.75
467,84261.28999996185,26.75
468,84284.1099998951,26.75
469,84307.30999994278,26.75
470,84330.6700000763,26.8125
471,84501.47000002861,26.8125
472,84524.88999986649,26.8125
473,84549.51999998093,26.8125
474,84573.55999994278,26.8125
475,84596.95000004768,26.8125
476,84619.77999997139,26.8125
477,84643.6099998951,26.8125
478,84667.25999999046,26.8125
479,84690.86999988556,26.8125
480,84713.59999990463,26.8125
481,84737.24000000954,26.8125
482,84761.68000006676,26.875
483,84785.11999988556,26.8125
484,84810.29999995232,26.875
485,84834.47000002861,26.875
486,84858.3299999237,26.875
487,84969.26999998093,26.875
488,84993.18000006676,26.875
489,85017.20000004768,26.8125
490,85041.23000001907,26.875
491,85064.47000002861,26.875
492,85087.6099998951,26.875
493,85111.6700000763,26.875
494,85134.80999994278,26.875
495,85159.3599998951,26.875
496,85183.31999993324,26.9375
497,85206.69000005722,26.875
498,85230.55999994278,26.875
499,85253.14999985695,26.875
500,85277.14999985695,26.875
501,85301.39999985695,26.875
502,85325.06999993324,26.875
503,85348.33999991417,26.875
504,85520.49000000954,26.9375
505,85543.75,26.9375
506,85568.22000002861,26.9375
507,85593.14999985695,26.9375
508,85617.48000001907,26.9375
509,85641.70000004768,26.9375
510,85689.18000006676,26.9375
511,85712.89999985695,26.9375
512,85736.84999990463,26.9375
513,85760.9200000763,26.9375
514,85784.63999986649,26.9375
515,85807.64999985695,27.0
516,85832.03999996185,26.9375
517,85856.28999996185,27.0
518,85879.59999990463,26.9375
519,85902.0799999237,27.0
520,85925.9200000763,27.0
521,85949.01999998093,27.0
522,85972.87999987602,27.0
523,85997.81999993324,27.0
524,86020.94000005722,27.0
525,86043.94000005722,27.0
526,86068.34999990463,27.0
527,86092.55999994278,27.0
528,86116.48000001907,27.0
529,86139.4200000763,27.0
530,86162.53999996185,27.0625
531,86185.25,27.0
532,86208.39999985695,27.0625
533,86380.1099998951,27.0625
534,86403.84999990463,27.0
535,86426.72000002861,27.0625
536,86450.77999997139,27.0625
537,86474.63999986649,27.0625
538,86498.58999991417,27.0625
539,86522.44000005722,27.0625
540,86546.21000003815,27.0625
541,86569.39999985695,27.0625
542,86593.91000008583,27.0625
543,86618.37999987602,27.0625
544,86641.69000005722,27.0625
545,86664.71000003815,27.0625
546,86687.78999996185,27.0625
547,86711.79999995232,27.0625
548,86822.93000006676,27.0625
549,86846.58999991417,27.0625
550,86870.97000002861,27.0625
551,86894.68000006676,27.125
552,86919.19000005722,27.125
553,86942.20000004768,27.0625
554,86966.13999986649,27.125
555,86989.53999996185,27.125
556,87013.00999999046,27.125
557,87037.18000006676,27.125
558,87060.28999996185,27.125
559,87083.96000003815,27.125
560,87106.53999996185,27.125
561,87130.31999993324,27.125
562,87302.04999995232,27.125
563,87324.97000002861,27.1875
564,87348.9200000763,27.125
565,87372.08999991417,27.125
566,87394.78999996185,27.1875
567,87418.04999995232,27.1875
568,87442.79999995232,27.1875
569,87465.86999988556,27.1875
570,87489.75,27.1875
571,87513.6099998951,27.1875
572,87537.95000004768,27.1875
573,87562.16000008583,27.1875
574,87586.1099998951,27.1875
575,87609.3299999237,27.1875
576,87633.5799999237,27.1875
577,87656.75999999046,27.1875
578,87679.8599998951,27.1875
579,87704.53999996185,27.1875
580,87728.05999994278,27.1875
581,87750.72000002861,27.1875
582,87773.39999985695,27.1875
583,87796.78999996185,27.1875
584,87820.20000004768,27.1875
585,87844.05999994278,27.1875
586,87867.95000004768,27.25
587,87891.63999986649,27.25
588,87915.13999986649,27.1875
589,87938.24000000954,27.1875
590,88079.83999991417,27.25
591,88102.80999994278,27.25
592,88126.75999999046,27.25
593,88151.06999993324,27.25
594,88175.0,27.25
595,88198.86999988556,27.25
596,88221.88999986649,27.25
597,88245.77999997139,27.25
598,88268.64999985695,27.25
599,88292.31999993324,27.25
600,88315.95000004768,27.25
601,88427.54999995232,27.3125
602,88450.0799999237,27.3125
603,88473.24000000954,27.3125
604,88495.96000003815,27.3125
605,88566.00999999046,27.3125
606,88590.00999999046,27.3125
607,88612.89999985695,27.3125
608,88636.59999990463,27.3125
609,88660.39999985695,27.3125
610,88683.53999996185,27.3125
611,88707.31999993324,27.3125
612,88730.56999993324,27.3125
613,88754.28999996185,27.3125
614,88777.97000002861,27.3125
615,88978.99000000954,27.375
616,89002.89999985695,27.3125
617,89026.28999996185,27.375
618,89050.16000008583,27.375
619,89074.48000001907,27.375
620,89098.52999997139,27.375
621,89121.74000000954,27.375
622,89144.68000006676,27.375
623,89167.53999996185,27.375
624,89191.01999998093,27.375
625,89213.75,27.375
626,89400.9200000763,27.375
627,89424.96000003815,27.375
628,89448.29999995232,27.375
629,89472.30999994278,27.4375
630,89496.48000001907,27.375
631,89519.53999996185,27.375
632,89542.50999999046,27.4375
633,89565.5,27.4375
634,89589.08999991417,27.375
635,89631.46000003815,27.4375
636,89654.25999999046,27.4375
637,89677.01999998093,27.4375
638,89818.11999988556,27.4375
639,89842.3299999237,27.4375
640,89867.24000000954,27.4375
641,89890.39999985695,27.4375
642,89914.44000005722,27.4375
643,89938.53999996185,27.4375
644,89961.63999986649,27.4375
645,89985.27999997139,27.4375
646,90009.03999996185,27.4375
647,90032.6099998951,27.4375
648,90055.24000000954,27.4375
649,90078.74000000954,27.5
650,90219.79999995232,27.5
651,90244.44000005722,27.5
652,90292.13999986649,27.5
653,90315.14999985695,27.5
654,90338.79999995232,27.5
655,90362.46000003815,27.5
656,90386.55999994278,27.5
657,90410.58999991417,27.5
658,90434.21000003815,27.5
659,90458.6099998951,27.5
660,90481.25999999046,27.5
661,90593.48000001907,27.5
662,90618.34999990463,27.5625
663,90642.34999990463,27.5625
664,90666.53999996185,27.5625
665,90689.72000002861,27.5625
666,90713.76999998093,27.5625
667,90737.61999988556,27.5625
668,90760.68000006676,27.5625
669,90787.48000001907,27.5625
670,90810.1700000763,27.5625
671,90834.30999994278,27.5625
672,90857.84999990463,27.5625
673,90881.98000001907,27.5625
674,90905.1700000763,27.5625
675,90928.28999996185,27.5625
676,90953.1099998951,27.5625
677,91094.56999993324,27.625
678,91117.51999998093,27.625
679,91140.75,27.5625
680,91164.9200000763,27.625
681,91188.94000005722,27.625
682,91212.63999986649,27.625
683,91236.51999998093,27.5625
684,91259.20000004768,27.5625
685,91283.21000003815,27.625
686,91306.54999995232,27.625
687,91329.27999997139,27.625
688,91353.97000002861,27.625
689,91378.00999999046,27.625
690,91402.05999994278,27.625
691,91542.75,27.625
692,91566.16000008583,27.625
693,91590.75999999046,27.6875
694,91615.1099998951,27.6875
695,91638.26999998093,27.625
696,91662.26999998093,27.625
697,91686.86999988556,27.6875
698,91710.53999996185,27.625
699,91734.72000002861,27.6875
700,91759.54999995232,27.6875
701,91782.9200000763,27.6875
702,91807.09999990463,27.6875
703,91831.1099998951,27.625
704,92000.02999997139,27.6875
705,92023.08999991417,27.6875
706,92046.84999990463,27.6875
707,92071.0799999237,27.6875
708,92095.50999999046,27.6875
709,92119.75,27.6875
710,92143.77999997139,27.6875
711,92167.27999997139,27.6875
712,92191.01999998093,27.6875
713,92213.93000006676,27.6875
714,92237.44000005722,27.6875
715,92261.16000008583,27.6875
716,92284.81999993324,27.6875
717,92308.81999993324,27.6875
718,92420.6700000763,27.6875
719,92444.18000006676,27.6875
720,92467.30999994278,27.75
721,92491.61999988556,27.75
722,92514.80999994278,27.75
723,92538.75,27.75
724,92561.53999996185,27.75
725,92585.48000001907,27.75
726,92608.37999987602,27.75
727,92631.48000001907,27.75
728,92655.06999993324,27.75
729,92678.88999986649,27.75
730,92701.5,27.75
731,92724.36999988556,27.75
732,92747.13999986649,27.8125
733,92910.69000005722,27.8125
734,92935.20000004768,27.8125
735,92958.95000004768,27.75
736,92982.5,27.75
737,93006.13999986649,27.8125
738,93029.36999988556,27.8125
739,93052.78999996185,27.8125
740,93076.11999988556,27.75
741,93099.74000000954,27.8125
742,93123.73000001907,27.8125
743,93147.88999986649,27.8125
744,93172.18000006676,27.8125
745,93196.13999986649,27.8125
746,93219.95000004768,27.8125
747,93243.29999995232,27.8125
748,93267.21000003815,27.8125
749,93379.04999995232,27.8125
750,93403.20000004768,27.8125
751,93427.13999986649,27.8125
752,93450.80999994278,27.8125
753,93475.0799999237,27.8125
754,93499.06999993324,27.875
755,93543.74000000954,27.8125
756,93566.91000008583,27.8125
757,93589.81999993324,27.8125
758,93731.84999990463,27.875
759,93754.9200000763,27.8125
760,93777.8599998951,27.8125
761,93801.09999990463,27.875
762,93825.6700000763,27.875
763,93848.68000006676,27.875
764,93871.47000002861,27.875
765,93895.13999986649,27.875
766,93918.25999999046,27.875
767,93942.20000004768,27.875
768,93965.62999987602,27.875
769,93988.84999990463,27.875
770,94011.95000004768,27.875
771,94035.63999986649,27.875
772,94059.00999999046,27.875
773,94082.8599998951,27.9375
774,94194.37999987602,27.875
775,94217.80999994278,27.875
776,94240.72000002861,27.875
777,94311.36999988556,27.875
778,94334.39999985695,27.875
779,94358.30999994278,27.875
780,94381.97000002861,27.875
781,94405.64999985695,27.875
782,94429.79999995232,27.9375
783,94570.53999996185,27.9375
784,94593.22000002861,27.9375
785,94617.41000008583,27.9375
786,94641.63999986649,27.9375
787,94664.94000005722,27.9375
788,94688.69000005722,27.9375
789,94712.55999994278,27.9375
790,94735.9200000763,27.9375
791,94760.49000000954,27.9375
792,94784.0,27.9375
793,94807.96000003815,27.9375
794,94831.08999991417,27.9375
795,94854.44000005722,27.9375
796,94878.6099998951,27.9375
797,94901.63999986649,27.9375
798,95102.25999999046,27.9375
799,95125.86999988556,27.9375
800,95148.50999999046,27.9375
801,95172.37999987602,27.9375
802,95196.6099998951,27.9375
803,95221.05999994278,27.9375
804,95244.25,27.9375
805,95268.75999999046,27.9375
806,95291.37999987602,27.9375
807,95315.37999987602,27.9375
808,95339.50999999046,27.9375
809,95362.18000006676,27.9375
810,95386.51999998093,27.9375
811,95410.1700000763,28.0
812,95434.29999995232,27.9375
813,95457.83999991417,27.9375
814,95481.97000002861,27.9375
815,95593.1099998951,28.0
816,95616.28999996185,27.9375
817,95639.13999986649,28.0
818,95663.0799999237,27.9375
819,95686.49000000954,28.0
820,95709.39999985695,28.0
821,95732.56999993324,28.0
822,95756.13999986649,28.0
823,95779.53999996185,28.0
824,95804.04999995232,28.0
825,95827.44000005722,28.0
826,95850.81999993324,28.0
827,95874.63999986649,28.0
828,95897.83999991417,28.0
829,95921.48000001907,28.0
830,96032.66000008583,28.0
831,96096.02999997139,28.0
832,96119.53999996185,28.0
833,96142.02999997139,28.0
834,96166.26999998093,28.0
835,96189.39999985695,28.0
836,96212.1099998951,28.0
837,96235.03999996185,28.0
838,96259.6700000763,28.0
839,96282.5,28.0
840,96305.54999995232,28.0
841,96328.9200000763,28.0
842,96470.0,28.0
843,96494.06999993324,28.0
844,96517.87999987602,28.0625
845,96542.03999996185,28.0
846,96566.16000008583,28.0625
847,96591.00999999046,28.0
848,96614.36999988556,28.0625
849,96637.61999988556,28.0
850,96661.16000008583,28.0625
851,96683.98000001907,28.0625
852,96707.44000005722,28.0625
853,96731.34999990463,28.0
854,96872.16000008583,28.0625
855,96895.25,28.0625
856,96918.24000000954,28.0625
857,96941.34999990463,28.0
858,96965.44000005722,28.0625
859,96988.75,28.0625
860,97011.68000006676,28.0625
861,97035.72000002861,28.0625
862,97058.9200000763,28.0625
863,97082.94000005722,28.0625
864,97106.30999994278,28.0625
865,97130.86999988556,28.0625
866,97154.53999996185,28.0625
867,97178.09999990463,28.0625
868,97200.75,28.0625
869,97224.45000004768,28.0625
870,97247.9200000763,28.0625
871,97270.50999999046,28.0625
872,97411.8599998951,28.0625
873,97435.87999987602,28.0625
874,97460.3599998951,28.0625
875,97483.99000000954,28.0625
876,97507.56999993324,28.0625
877,97531.29999995232,28.0625
878,97555.25,28.0625
879,97579.8299999237,28.0625
880,97603.18000006676,28.0625
881,97626.69000005722,28.0625
882,97650.0799999237,28.0625
883,97673.19000005722,28.0625
884,97697.12999987602,28.0625
885,97720.5,28.0625
886,97743.04999995232,28.0625
887,97943.61999988556,28.0625
888,97966.70000004768,28.0625
889,97989.93000006676,28.0625
890,98012.55999994278,28.125
891,98039.46000003815,28.0625
892,98062.4200000763,28.0625
893,98086.38999986649,28.125
894,98109.36999988556,28.125
895,98133.80999994278,28.125
896,98156.9200000763,28.125
897,98179.72000002861,28.0625
898,98203.48000001907,28.0625
899,98226.62999987602,28.125
900,98249.86999988556,28.125
901,98274.74000000954,28.125
902,98297.86999988556,28.0625
903,98321.29999995232,28.125
904,98344.95000004768,28.125
905,98481.53999996185,28.125
906,98504.74000000954,28.125
907,98528.94000005722,28.125
908,98553.28999996185,28.125
909,98576.44000005722,28.125
910,98599.44000005722,28.125
911,98623.05999994278,28.125
912,98646.22000002861,28.125
913,98669.09999990463,28.125
914,98692.37999987602,28.125
915,98716.6099998951,28.125
916,98739.41000008583,28.125
917,98849.75999999046,28.125
918,98872.52999997139,28.125
919,98895.79999995232,28.125
920,98918.58999991417,28.125
921,98942.93000006676,28.125
922,98966.74000000954,28.125
923,98990.48000001907,28.125
924,99014.95000004768,28.125
925,99038.25,28.125
926,99061.61999988556,28.125
927,99085.71000003815,28.125
928,99228.54999995232,28.125
929,99252.37999987602,28.125
930,99275.56999993324,28.125
931,99299.6700000763,28.1875
932,99324.11999988556,28.125
933,99348.13999986649,28.125
934,99372.18000006676,28.1875
935,99395.80999994278,28.1875
936,99419.84999990463,28.125
937,99442.96000003815,28.1875
938,99466.19000005722,28.1875
939,99490.14999985695,28.1875
940,99513.97000002861,28.125
941,99537.39999985695,28.1875
942,99582.13999986649,28.125
943,99605.4200000763,28.1875
944,99629.61999988556,28.1875
945,99771.25,28.1875
946,99795.4200000763,28.1875
947,99819.53999996185,28.1875
948,99842.99000000954,28.1875
949,99865.86999988556,28.1875
950,99889.41000008583,28.1875
951,99913.43000006676,28.1875
952,99937.49000000954,28.1875
953,99961.41000008583,28.1875
954,99984.93000006676,28.1875
955,100009.08999991417,28.1875
956,100032.97000002861,28.1875
957,100057.48000001907,28.1875
958,100080.74000000954,28.1875
959,100253.44000005722,28.1875
960,100276.55999994278,28.1875
961,100299.43000006676,28.1875
962,100322.95000004768,28.1875
963,100345.68000006676,28.1875
964,100369.21000003815,28.1875
965,100393.02999997139,28.1875
966,100415.6099998951,28.1875
967,100439.58999991417,28.1875
968,100463.50999999046,28.1875
969,100487.33999991417,28.1875
970,100511.00999999046,28.1875
971,100534.84999990463,28.1875
972,100557.96000003815,28.1875
973,100581.25999999046,28.1875
974,100783.71000003815,28.25
975,100807.74000000954,28.1875
976,100831.98000001907,28.1875
977,100855.89999985695,28.25
978,100903.75999999046,28.25
979,100926.87999987602,28.1875
980,100950.71000003815,28.1875
981,100975.80999994278,28.25
982,100998.31999993324,28.25
983,101021.87999987602,28.1875
984,101045.93000006676,28.25
985,101069.13999986649,28.25
986,101091.74000000954,28.25
987,101114.71000003815,28.1875
988,101137.81999993324,28.25
989,101280.21000003815,28.25
990,101304.55999994278,28.25
991,101327.28999996185,28.25
992,101349.84999990463,28.1875
993,101373.04999995232,28.25
994,101397.29999995232,28.25
995,101419.9200000763,28.25
996,101443.83999991417,28.25
997,101467.33999991417,28.25
998,101490.9200000763,28.25
999,101514.98000001907,28.25
1000,101538.22000002861,28.25
1001,101562.0,28.25
1002,101585.25999999046,28.25
1003,101608.75,28.25
1004,101779.75,28.25
1005,101802.99000000954,28.25
1006,101826.1099998951,28.25
1007,101850.27999997139,28.25
1008,101874.20000004768,28.25
1009,101897.83999991417,28.25
1010,101921.09999990463,28.25
1011,101945.0799999237,28.25
1012,101970.01999998093,28.25
1013,101994.09999990463,28.25
1014,102017.25,28.25
1015,102040.94000005722,28.25
1016,102064.61999988556,28.25
1017,102088.28999996185,28.25
1018,102112.51999998093,28.25
1019,102136.4200000763,28.25
1020,102160.45000004768,28.25
1021,102183.02999997139,28.25
1022,102383.88999986649,28.3125
1023,102407.06999993324,28.25
1024,102430.03999996185,28.25
1025,102454.4200000763,28.25
1026,102478.62999987602,28.25
1027,102502.26999998093,28.25
1028,102525.5,28.25
1029,102549.3599998951,28.25
1030,102573.6700000763,28.25
1031,102596.75,28.3125
1032,102620.76999998093,28.25
1033,102644.53999996185,28.25
1034,102669.14999985695,28.25
1035,102693.45000004768,28.25
1036,102716.49000000954,28.25
1037,102827.1700000763,28.25
1038,102850.75999999046,28.3125
1039,102874.97000002861,28.25
1040,102898.94000005722,28.3125
1041,102922.30999994278,28.25
1042,102945.26999998093,28.25
1043,102968.26999998093,28.25
1044,102992.36999988556,28.3125
1045,103016.3599998951,28.3125
1046,103039.24000000954,28.3125
1047,103062.12999987602,28.3125
1048,103085.21000003815,28.25
1049,103226.14999985695,28.25
1050,103250.25999999046,28.3125
1051,103273.50999999046,28.3125
1052,103297.59999990463,28.3125
1053,103321.63999986649,28.3125
1054,103344.87999987602,28.3125
1055,103368.80999994278,28.3125
1056,103391.48000001907,28.3125
1057,103414.9200000763,28.25
1058,103438.45000004768,28.25
1059,103462.41000008583,28.25
1060,103486.18000006676,28.3125
1061,103508.99000000954,28.3125
1062,103532.61999988556,28.3125
1063,103555.5799999237,28.3125
1064,103579.47000002861,28.3125
1065,103602.78999996185,28.3125
1066,103744.59999990463,28.3125
1067,103767.22000002861,28.3125
1068,103789.8599998951,28.25
1069,103813.06999993324,28.3125
1070,103835.8599998951,28.3125
1071,103860.08999991417,28.3125
1072,103883.76999998093,28.3125
1073,103907.97000002861,28.3125
1074,103932.26999998093,28.3125
1075,103955.75999999046,28.3125
1076,103978.4200000763,28.3125
1077,104021.94000005722,28.25
1078,104045.37999987602,28.3125
1079,104186.24000000954,28.3125
1080,104210.06999993324,28.3125
1081,104233.08999991417,28.3125
1082,104256.12999987602,28.3125
1083,104279.45000004768,28.3125
1084,104302.41000008583,28.3125
1085,104325.46000003815,28.3125
1086,104373.19000005722,28.3125
1087,104397.33999991417,28.3125
1088,104568.52999997139,28.3125
1089,104592.54999995232,28.3125
1090,104616.03999996185,28.3125
1091,104641.03999996185,28.3125
1092,104664.79999995232,28.3125
1093,104687.78999996185,28.3125
1094,104710.77999997139,28.3125
1095,104733.62999987602,28.3125
1096,104757.46000003815,28.3125
1097,104781.00999999046,28.3125
1098,104805.08999991417,28.3125
1099,104828.31999993324,28.3125
1100,104851.33999991417,28.3125
1101,104874.56999993324,28.3125
1102,104898.78999996185,28.3125
1103,104922.03999996185,28.3125
1104,105096.21000003815,28.3125
1105,105120.01999998093,28.3125
1106,105143.24000000954,28.3125
1107,105190.63999986649,28.3125
1108,105214.59999990463,28.3125
1109,105237.5799999237,28.3125
1110,105262.22000002861,28.3125
1111,105286.44000005722,28.3125
1112,105311.01999998093,28.375
1113,105333.83999991417,28.3125
1114,105358.00999999046,28.3125
1115,105381.75999999046,28.3125
1116,105405.39999985695,28.3125
1117,105428.83999991417,28.375
1118,105451.9200000763,28.3125
1119,105474.8599998951,28.3125
1120,105498.56999993324,28.3125
1121,105522.66000008583,28.3125
1122,105545.74000000954,28.3125
1123,105717.34999990463,28.3125
1124,105741.26999998093,28.375
1125,105764.94000005722,28.3125
1126,105788.25,28.3125
1127,105811.75,28.3125
1128,105835.16000008583,28.3125
1129,105858.34999990463,28.3125
1130,105881.22000002861,28.3125
1131,105904.3599998951,28.3125
1132,105927.43000006676,28.375
1133,105951.53999996185,28.3125
1134,105975.39999985695,28.3125
1135,105998.63999986649,28.375
1136,106022.56999993324,28.375
1137,106046.68000006676,28.375
1138,106158.0799999237,28.3125
1139,106181.13999986649,28.3125
1140,106204.9200000763,28.3125
1141,106229.27999997139,28.375
1142,106252.13999986649,28.3125
1143,106275.25999999046,28.3125
1144,106297.98000001907,28.3125
1145,106320.71000003815,28.3125
1146,106344.09999990463,28.375
1147,106368.16000008583,28.3125
1148,106391.71000003815,28.3125
1149,106415.72000002861,28.375
1150,106439.00999999046,28.3125
1151,106463.0,28.3125
1152,106486.80999994278,28.3125
1153,106510.81999993324,28.3125
1154,106621.83999991417,28.375
1155,106644.95000004768,28.3125
1156,106668.4200000763,28.375
1157,106691.5799999237,28.375
1158,106715.83999991417,28.375
1159,106740.08999991417,28.375
1160,106764.25,28.375
1161,106788.33999991417,28.375
1162,106811.08999991417,28.375
1163,106833.83999991417,28.375
1164,106857.3299999237,28.375
1165,106880.6099998951,28.3125
1166,106904.1700000763,28.375
1167,106928.00999999046,28.375
1168,106951.36999988556,28.375
1169,106975.64999985695,28.3125
1170,107086.27999997139,28.375
1171,107110.31999993324,28.375
1172,107133.06999993324,28.3125
1173,107156.93000006676,28.375
1174,107179.72000002861,28.375
1175,107202.8599998951,28.375
1176,107225.6700000763,28.375
1177,107249.59999990463,28.375
1178,107273.28999996185,28.375
1179,107296.5799999237,28.375
1180,107320.43000006676,28.375
1181,107344.23000001907,28.375
1182,107368.70000004768,28.375
1183,107570.74000000954,28.375
1184,107593.73000001907,28.375
1185,107617.5,28.375
1186,107640.51999998093,28.375
1187,107663.55999994278,28.375
1188,107687.64999985695,28.3125
1189,107711.02999997139,28.375
1190,107734.44000005722,28.3125
1191,107758.24000000954,28.375
1192,107781.97000002861,28.375
1193,107806.12999987602,28.375
1194,107829.6700000763,28.375
1195,107853.76999998093,28.375
1196,107876.73000001907,28.375
1197,107900.3299999237,28.375
1198,107923.58999991417,28.375
1199,107947.09999990463,28.375
1200,108058.00999999046,28.375
1201,108080.8299999237,28.375
1202,108104.98000001907,28.375
1203,108128.83999991417,28.375
1204,108151.66000008583,28.375
1205,108174.5799999237,28.375
1206,108197.4200000763,28.375
1207,108222.13999986649,28.375
1208,108246.0799999237,28.375
1209,108268.89999985695,28.375
1210,108291.9200000763,28.375
1211,108315.96000003815,28.375
1212,108339.23000001907,28.3125
1213,108527.13999986649,28.375
1214,108550.96000003815,28.375
1215,108573.86999988556,28.375
1216,108596.9200000763,28.375
1217,108620.77999997139,28.375
1218,108644.58999991417,28.375
1219,108667.69000005722,28.375
1220,108691.31999993324,28.375
1221,108714.41000008583,28.375
1222,108737.37999987602,28.375
1223,108760.33999991417,28.375
1224,108784.03999996185,28.375
1225,108807.59999990463,28.375
1226,108830.69000005722,28.375
1227,108855.53999996185,28.375
1228,108878.9200000763,28.375
1229,108901.78999996185,28.375
1230,109014.69000005722,28.375
1231,109038.23000001907,28.375
1232,109061.11999988556,28.375
1233,109084.94000005722,28.375
1234,109108.46000003815,28.375
1235,109132.48000001907,28.375
1236,109156.50999999046,28.375
1237,109203.04999995232,28.375
1238,109227.6099998951,28.4375
1239,109250.83999991417,28.375
1240,109273.87999987602,28.375
1241,109298.08999991417,28.375
1242,109321.88999986649,28.375
1243,109345.79999995232,28.375
1244,109368.83999991417,28.375
1245,109392.5799999237,28.375
1246,109416.53999996185,28.375
1247,109439.64999985695,28.375
1248,109580.74000000954,28.375
1249,109603.54999995232,28.375
1250,109626.72000002861,28.375
1251,109649.95000004768,28.375
1252,109673.00999999046,28.375
1253,109695.68000006676,28.375
1254,109718.73000001907,28.375
1255,109742.5799999237,28.375
1256,109766.50999999046,28.375
1257,109789.73000001907,28.375
1258,109812.89999985695,28.375
1259,109836.79999995232,28.375
1260,109859.8599998951,28.375
1261,109882.75999999046,28.375
1262,109905.75999999046,28.375
1263,109928.55999994278,28.375
1264,110162.04999995232,28.375
1265,110184.50999999046,28.375
1266,110207.64999985695,28.375
1267,110230.46000003815,28.375
1268,110253.48000001907,28.375
1269,110276.47000002861,28.375
1270,110300.66000008583,28.375
1271,110323.9200000763,28.375
1272,110347.12999987602,28.375
1273,110370.72000002861,28.375
1274,110393.80999994278,28.375
1275,110416.79999995232,28.375
1276,110441.24000000954,28.375
1277,110484.63999986649,28.375
1278,110625.41000008583,28.375
1279,110648.44000005722,28.375
1280,110671.91000008583,28.375
1281,110695.91000008583,28.375
1282,110719.0799999237,28.375
1283,110742.1099998951,28.375
1284,110765.41000008583,28.375
1285,110788.76999998093,28.375
1286,110811.89999985695,28.375
1287,110836.25,28.375
1288,110860.00999999046,28.375
1289,111001.26999998093,28.375
1290,111024.47000002861,28.375
1291,111048.6700000763,28.375
1292,111072.99000000954,28.375
1293,111096.11999988556,28.375
1294,111119.98000001907,28.375
1295,111143.5799999237,28.375
1296,111167.05999994278,28.375
1297,111190.66000008583,28.375
1298,111214.1099998951,28.375
1299,111237.25,28.375
1300,111261.37999987602,28.375
1301,111286.04999995232,28.375
1302,111310.27999997139,28.375
1303,111333.51999998093,28.375
1304,111403.00999999046,28.375
1305,111573.89999985695,28.375
1306,111598.01999998093,28.375
1307,111621.6700000763,28.375
1308,111645.63999986649,28.375
1309,111669.52999997139,28.375
1310,111693.95000004768,28.375
1311,111716.99000000954,28.375
1312,111842.88999986649,28.375
1313,111866.94000005722,28.375
1314,111889.70000004768,28.375
1315,111913.43000006676,28.375
1316,111937.53999996185,28.375
1317,112127.0799999237,28.375
1318,112149.74000000954,28.375
1319,112173.3599998951,28.375
1320,112197.43000006676,28.375
1321,112221.20000004768,28.375
1322,112244.08999991417,28.375
1323,112267.95000004768,28.375
1324,112291.64999985695,28.375
1325,112316.18000006676,28.375
1326,112339.0,28.375
1327,112361.94000005722,28.375
1328,112407.66000008583,28.375
1329,112549.56999993324,28.375
1330,112572.66000008583,28.375
1331,112595.8299999237,28.375
1332,112746.09999990463,28.375
1333,112769.14999985695,28.375
1334,112792.24000000954,28.375
1335,112815.19000005722,28.375
1336,112838.27999997139,28.375
1337,112861.80999994278,28.375
1338,112884.93000006676,28.375
1339,113011.71000003815,28.3125
1340,113055.8599998951,28.375
1341,113079.88999986649,28.375
1342,113102.86999988556,28.375
1343,113244.3299999237,28.3125
1344,113268.27999997139,28.3125
1345,113291.25,28.3125
1346,113314.30999994278,28.3125
1347,113337.79999995232,28.3125
1348,113362.87999987602,28.3125
1349,113385.61999988556,28.3125
1350,113409.59999990463,28.3125
1351,113433.50999999046,28.3125
1352,113456.68000006676,28.3125
1353,113480.33999991417,28.3125
1354,113503.79999995232,28.3125
1355,113527.45000004768,28.3125
1356,113550.69000005722,28.3125
1357,113573.49000000954,28.3125
1358,113724.5799999237,28.375
1359,113747.9200000763,28.375
1360,113771.25,28.375
1361,113795.4200000763,28.375
1362,113819.50999999046,28.375
1363,113842.94000005722,28.3125
1364,113866.11999988556,28.375
1365,113890.0799999237,28.3125
1366,113913.68000006676,28.3125
1367,113937.74000000954,28.375
1368,113960.61999988556,28.3125
1369,113984.75999999046,28.3125
1370,114008.13999986649,28.375
1371,114032.3299999237,28.375
1372,114055.44000005722,28.3125
1373,114196.34999990463,28.375
1374,114220.13999986649,28.375
1375,114242.63999986649,28.375
1376,114265.77999997139,28.375
1377,114289.55999994278,28.3125
1378,114313.59999990463,28.3125
1379,114337.11999988556,28.3125
1380,114361.01999998093,28.3125
1381,114384.73000001907,28.3125
1382,114409.14999985695,28.3125
1383,114433.38999986649,28.3125
1384,114477.41000008583,28.3125
1385,114500.63999986649,28.3125
1386,114612.54999995232,28.3125
1387,114635.11999988556,28.3125
1388,114659.47000002861,28.3125
1389,114682.5,28.3125
1390,114706.47000002861,28.3125
1391,114729.05999994278,28.3125
1392,114751.75,28.3125
1393,114775.1099998951,28.3125
1394,114797.98000001907,28.3125
1395,114867.88999986649,28.3125
1396,114891.61999988556,28.3125
1397,114915.50999999046,28.3125
1398,114939.73000001907,28.3125
1399,114962.44000005722,28.3125
1400,115131.47000002861,28.25
1401,115156.22000002861,28.3125
1402,115180.63999986649,28.3125
1403,115204.89999985695,28.25
1404,115252.77999997139,28.25
1405,115277.73000001907,28.25
1406,115301.74000000954,28.25
1407,115325.14999985695,28.25
1408,115348.12999987602,28.25
1409,115371.63999986649,28.25
1410,115395.45000004768,28.25
1411,115418.88999986649,28.25
1412,115443.30999994278,28.25
1413,115467.01999998093,28.25
1414,115489.84999990463,28.25
1415,115513.66000008583,28.25
1416,115654.84999990463,28.25
1417,115677.99000000954,28.25
1418,115700.75999999046,28.25
1419,115723.95000004768,28.25
1420,115748.20000004768,28.25
1421,115772.5799999237,28.25
1422,115795.39999985695,28.25
1423,115818.53999996185,28.1875
1424,115842.77999997139,28.25
1425,115865.8599998951,28.25
1426,115889.84999990463,28.25
1427,115913.0,28.25
1428,115936.71000003815,28.25
1429,115960.03999996185,28.1875
1430,115983.64999985695,28.25
1431,116154.77999997139,28.1875
1432,116178.49000000954,28.25
1433,116201.25,28.1875
1434,116223.87999987602,28.1875
1435,116247.89999985695,28.1875
1436,116270.76999998093,28.1875
1437,116293.27999997139,28.1875
1438,116316.48000001907,28.1875
1439,116339.44000005722,28.1875
1440,116362.1099998951,28.1875
1441,116385.54999995232,28.1875
1442,116408.76999998093,28.1875
1443,116432.01999998093,28.1875
1444,116474.64999985695,28.1875
1445,116586.23000001907,28.1875
1446,116609.0,28.125
1447,116656.8599998951,28.125
1448,116680.81999993324,28.125
1449,116704.64999985695,28.125
1450,116727.48000001907,28.125
1451,116768.26999998093,28.125
1452,116791.94000005722,28.125
1453,116816.14999985695,28.125
1454,116839.71000003815,28.125
1455,116863.27999997139,28.125
1456,116887.56999993324,28.125
1457,116912.0,28.125
1458,116935.89999985695,28.125
1459,116960.28999996185,28.125
1460,117161.1099998951,28.125
1461,117185.19000005722,28.125
1462,117208.27999997139,28.125
1463,117232.41000008583,28.0625
1464,117255.24000000954,28.125
1465,117277.99000000954,28.125
1466,117300.87999987602,28.0625
1467,117324.30999994278,28.0625
1468,117346.98000001907,28.0625
1469,117369.84999990463,28.0625
1470,117392.84999990463,28.125
1471,117416.69000005722,28.0625
1472,117439.05999994278,28.0625
1473,117462.89999985695,28.0625
1474,117573.63999986649,28.0625
1475,117596.96000003815,28.0625
1476,117621.06999993324,28.0625
1477,117645.34999990463,28.0625
1478,117669.01999998093,28.0625
1479,117692.36999988556,28.0625
1480,117716.5799999237,28.0625
1481,117739.91000008583,28.0625
1482,117763.06999993324,28.0625
1483,117785.97000002861,28.0625
1484,117808.61999988556,28.0625
1485,117832.55999994278,28.0625
1486,117855.47000002861,28.0625
1487,117995.77999997139,28.0625
1488,118019.80999994278,28.0625
1489,118043.18000006676,28.0625
1490,118067.37999987602,28.0625
1491,118090.75999999046,28.0625
1492,118113.50999999046,28.0625
1493,118136.94000005722,28.0625
1494,118161.26999998093,28.0
1495,118184.75,28.0625
1496,118207.75,28.0
1497,118230.54999995232,28.0625
1498,118253.25,28.0
1499,118277.94000005722,28.0
1500,118302.01999998093,28.0
1501,118325.1099998951,28.0
1502,118525.79999995232,28.0625
1503,118549.37999987602,28.0625
1504,118572.03999996185,28.0
1505,118595.16000008583,28.0
1506,118618.43000006676,28.0
1507,118641.12999987602,28.0
1508,118665.5,28.0
1509,118689.63999986649,28.0
1510,118712.84999990463,28.0
1511,118735.3599998951,28.0
1512,118758.48000001907,28.0
1513,118782.31999993324,28.0
1514,118805.24000000954,28.0
1515,118945.95000004768,28.0
1516,118968.83999991417,28.0
1517,118991.97000002861,28.0
1518,119015.5799999237,28.0
1519,119038.89999985695,28.0
1520,119062.0,28.0
1521,119085.06999993324,28.0
1522,119109.16000008583,28.0
1523,119131.72000002861,28.0
1524,119154.83999991417,28.0
1525,119177.68000006676,28.0
1526,119200.53999996185,28.0
1527,119223.27999997139,28.0
1528,119246.08999991417,27.9375
1529,119268.94000005722,27.9375
1530,119439.43000006676,27.9375
1531,119462.77999997139,27.9375
1532,119486.66000008583,27.9375
1533,119510.48000001907,27.9375
1534,119534.03999996185,27.9375
1535,119557.86999988556,27.9375
1536,119581.66000008583,27.9375
1537,119604.61999988556,27.9375
1538,119627.51999998093,27.9375
1539,119651.63999986649,27.9375
1540,119762.56999993324,27.9375
1541,119785.94000005722,27.9375
1542,119808.68000006676,27.9375
1543,119832.75999999046,27.9375
1544,119856.41000008583,27.875
1545,119879.41000008583,27.875
1546,119903.39999985695,27.9375
1547,119926.9200000763,27.875
1548,119950.45000004768,27.875
1549,119973.53999996185,27.875
1550,119997.3599998951,27.9375
1551,120108.49000000954,27.875
1552,120131.75999999046,27.9375
1553,120155.66000008583,27.875
1554,120178.55999994278,27.875
1555,120201.96000003815,27.875
1556,120225.53999996185,27.875
1557,120249.6700000763,27.875
1558,120272.5799999237,27.875
1559,120296.53999996185,27.875
1560,120320.00999999046,27.875
1561,120343.89999985695,27.875
1562,120367.59999990463,27.875
1563,120391.34999990463,27.8125
1564,120413.95000004768,27.875
1565,120436.75,27.875
1566,120459.66000008583,27.8125
1567,120570.44000005722,27.8125
1568,120593.75999999046,27.8125
1569,120616.78999996185,27.875
1570,120639.70000004768,27.8125
1571,120662.97000002861,27.8125
1572,120686.13999986649,27.8125
1573,120708.77999997139,27.8125
1574,120731.88999986649,27.8125
1575,120755.00999999046,27.8125
1576,120778.89999985695,27.8125
1577,120802.28999996185,27.8125
1578,120826.37999987602,27.8125
1579,121053.47000002861,27.8125
1580,121076.52999997139,27.75
1581,121099.46000003815,27.8125
1582,121123.50999999046,27.8125
1583,121146.95000004768,27.75
1584,121169.8599998951,27.75
1585,121192.70000004768,27.8125
1586,121216.78999996185,27.75
1587,121239.58999991417,27.75
1588,121262.66000008583,27.8125
1589,121285.41000008583,27.75
1590,121309.76999998093,27.75
1591,121334.03999996185,27.75
1592,121357.5,27.75
1593,121380.00999999046,27.75
1594,121403.20000004768,27.75
1595,121426.91000008583,27.75
1596,121537.44000005722,27.75
1597,121561.68000006676,27.75
1598,121584.79999995232,27.75
1599,121608.5,27.75
1600,121632.04999995232,27.75
1601,121655.02999997139,27.75
1602,121679.19000005722,27.75
1603,121703.19000005722,27.75
1604,121726.04999995232,27.6875
1605,121749.26999998093,27.75
1606,121773.0799999237,27.75
1607,121796.25999999046,27.75
1608,121820.81999993324,27.6875
1609,121843.80999994278,27.6875
1610,121977.71000003815,27.6875
1611,122000.56999993324,27.6875
1612,122024.64999985695,27.6875
1613,122048.5799999237,27.6875
1614,122072.13999986649,27.6875
1615,122096.50999999046,27.6875
1616,122119.14999985695,27.6875
1617,122141.87999987602,27.6875
1618,122165.81999993324,27.6875
1619,122188.47000002861,27.6875
1620,122212.33999991417,27.6875
1621,122236.53999996185,27.6875
1622,122260.18000006676,27.6875
1623,122284.26999998093,27.6875
1624,122307.37999987602,27.625
1625,122331.13999986649,27.6875
1626,122471.3299999237,27.6875
1627,122495.48000001907,27.6875
1628,122518.48000001907,27.625
1629,122543.71000003815,27.625
1630,122568.01999998093,27.625
1631,122591.28999996185,27.625
1632,122615.39999985695,27.625
1633,122638.27999997139,27.625
1634,122661.33999991417,27.625
1635,122684.44000005722,27.625
1636,122707.20000004768,27.625
1637,122731.45000004768,27.625
1638,122754.80999994278,27.625
1639,122778.37999987602,27.625
1640,122802.16000008583,27.625
1641,122913.61999988556,27.5625
1642,122936.81999993324,27.625
1643,122959.80999994278,27.5625
1644,122983.54999995232,27.625
1645,123031.84999990463,27.5625
1646,123055.5799999237,27.5625
1647,123079.61999988556,27.5625
1648,123102.5,27.5625
1649,123125.99000000954,27.5625
1650,123148.71000003815,27.5625
1651,123172.36999988556,27.5625
1652,123196.9200000763,27.5625
1653,123220.3599998951,27.5625
1654,123244.37999987602,27.5625
1655,123267.47000002861,27.5
1656,123291.13999986649,27.5
1657,123314.81999993324,27.5625
1658,123455.74000000954,27.5625
1659,123479.38999986649,27.5625
1660,123502.21000003815,27.5625
1661,123525.45000004768,27.5
1662,123548.66000008583,27.5625
1663,123572.53999996185,27.5
1664,123597.08999991417,27.5
1665,123621.03999996185,27.5
1666,123644.24000000954,27.5
1667,123667.49000000954,27.5
1668,123690.64999985695,27.5
1669,123714.68000006676,27.5
1670,123738.89999985695,27.5
1671,123849.96000003815,27.5625
1672,123873.75,27.5
1673,123897.1700000763,27.5
1674,123967.14999985695,27.5
1675,123991.53999996185,27.5
1676,124014.58999991417,27.5
1677,124038.19000005722,27.5
1678,124061.58999991417,27.5
1679,124084.94000005722,27.5
1680,124107.71000003815,27.4375
1681,124279.27999997139,27.5
1682,124302.11999988556,27.5
1683,124325.22000002861,27.5
1684,124395.33999991417,27.5
1685,124439.34999990463,27.5
1686,124462.14999985695,27.4375
1687,124485.6700000763,27.4375
1688,124656.37999987602,27.4375
1689,124680.53999996185,27.4375
1690,124703.29999995232,27.4375
1691,124727.11999988556,27.4375
1692,124750.20000004768,27.4375
1693,124773.86999988556,27.4375
1694,124796.91000008583,27.4375
1695,124820.38999986649,27.4375
1696,124843.05999994278,27.4375
1697,124865.58999991417,27.4375
1698,124888.88999986649,27.4375
1699,124911.97000002861,27.4375
1700,124936.01999998093,27.375
1701,124959.20000004768,27.4375
1702,124982.21000003815,27.4375
1703,125123.97000002861,27.4375
1704,125147.41000008583,27.375
1705,125171.62999987602,27.4375
1706,125194.53999996185,27.375
1707,125217.98000001907,27.375
1708,125240.69000005722,27.375
1709,125265.56999993324,27.375
1710,125289.49000000954,27.375
1711,125312.53999996185,27.375
1712,125335.34999990463,27.375
1713,125507.04999995232,27.375
1714,125530.72000002861,27.375
1715,125554.25,27.375
1716,125577.64999985695,27.375
1717,125601.44000005722,27.375
1718,125625.19000005722,27.375
1719,125648.54999995232,27.375
1720,125671.26999998093,27.375
1721,125694.1700000763,27.375
1722,125717.3599998951,27.375
1723,125741.41000008583,27.3125
1724,125764.4200000763,27.3125
1725,125788.36999988556,27.3125
1726,125812.47000002861,27.3125
1727,125836.41000008583,27.3125
1728,125860.76999998093,27.3125
1729,126031.33999991417,27.3125
1730,126055.24000000954,27.3125
1731,126079.29999995232,27.3125
1732,126103.18000006676,27.3125
1733,126126.30999994278,27.3125
1734,126149.96000003815,27.3125
1735,126175.18000006676,27.3125
1736,126198.75,27.25
1737,126222.58999991417,27.3125
1738,126246.70000004768,27.3125
1739,126269.50999999046,27.25
1740,126293.95000004768,27.25
1741,126317.11999988556,27.25
1742,126340.18000006676,27.25
1743,126452.66000008583,27.25
1744,126476.75,27.25
1745,126500.28999996185,27.25
1746,126523.33999991417,27.25
1747,126546.38999986649,27.25
1748,126569.80999994278,27.25
1749,126593.45000004768,27.25
1750,126616.6700000763,27.25
1751,126640.37999987602,27.25
1752,126663.87999987602,27.25
1753,126688.34999990463,27.25
1754,126712.80999994278,27.1875
1755,126736.3599998951,27.1875
1756,126846.96000003815,27.1875
1757,126870.50999999046,27.1875
1758,126893.97000002861,27.1875
1759,126916.55999994278,27.1875
1760,126940.8299999237,27.1875
1761,126965.1099998951,27.1875
1762,126988.27999997139,27.1875
1763,127012.29999995232,27.1875
1764,127036.23000001907,27.1875
1765,127060.39999985695,27.1875
1766,127083.75,27.1875
1767,127107.58999991417,27.1875
1768,127150.72000002861,27.125
1769,127173.8599998951,27.1875
1770,127197.08999991417,27.125
1771,127220.24000000954,27.125
1772,127243.21000003815,27.1875
1773,127266.84999990463,27.125
1774,127290.88999986649,27.125
1775,127314.28999996185,27.125
1776,127338.41000008583,27.125
1777,127361.48000001907,27.125
1778,127386.46000003815,27.125
1779,127409.63999986649,27.125
1780,127550.74000000954,27.125
1781,127573.53999996185,27.125
1782,127597.25999999046,27.125
1783,127620.99000000954,27.125
1784,127691.04999995232,27.125
1785,127715.02999997139,27.125
1786,127738.98000001907,27.125
1787,127761.98000001907,27.0625
1788,127785.20000004768,27.0625
1789,127809.76999998093,27.0625
1790,127834.33999991417,27.0625
1791,127858.00999999046,27.0625
1792,127881.13999986649,27.0625
1793,128039.36999988556,27.0625
1794,128063.96000003815,27.0625
1795,128086.94000005722,27.0625
1796,128111.43000006676,27.0625
1797,128134.97000002861,27.0625
1798,128157.56999993324,27.0
1799,128181.1700000763,27.0625
1800,128204.09999990463,27.0
1801,128227.0799999237,27.0
1802,128250.29999995232,27.0
1803,128273.6700000763,27.0
1804,128297.83999991417,27.0
1805,128408.73000001907,27.0
1806,128432.33999991417,27.0
1807,128456.99000000954,27.0
1808,128479.99000000954,27.0
1809,128502.71000003815,27.0
1810,128526.58999991417,27.0
1811,128550.23000001907,27.0
1812,128594.75,27.0
1813,128617.96000003815,27.0
1814,128689.89999985695,27.0
1815,128712.74000000954,27.0
1816,128736.04999995232,27.0
1817,128939.94000005722,27.0
1818,128962.72000002861,27.0
1819,128985.9200000763,27.0
1820,129009.00999999046,27.0
1821,129031.6700000763,27.0
1822,129055.53999996185,27.0
1823,129079.23000001907,27.0
1824,129102.20000004768,27.0
1825,129126.28999996185,27.0
1826,129149.64999985695,27.0
1827,129173.83999991417,27.0
1828,129197.25999999046,27.0
1829,129220.41000008583,27.0
1830,129243.47000002861,27.0
1831,129384.36999988556,27.0625
1832,129407.30999994278,27.0625
1833,129430.9200000763,27.0
1834,129454.8599998951,27.0
1835,129478.01999998093,27.0625
1836,129501.68000006676,27.0625
1837,129525.16000008583,27.0
1838,129550.24000000954,27.0
1839,129574.31999993324,27.0
1840,129645.08999991417,27.0625
1841,129667.54999995232,27.0625
1842,129692.04999995232,27.0
1843,129715.29999995232,27.0625
1844,129738.23000001907,27.0
1845,129974.18000006676,27.0625
1846,129997.53999996185,27.0625
1847,130021.29999995232,27.0625
1848,130045.86999988556,27.0625
1849,130069.63999986649,27.0625
1850,130092.84999990463,27.0625
1851,130116.84999990463,27.0625
1852,130140.0799999237,27.0625
1853,130280.49000000954,27.0625
1854,130304.19000005722,27.0625
1855,130373.76999998093,27.0625
1856,130396.5799999237,27.0625
1857,130420.51999998093,27.0625
1858,130444.38999986649,27.0625
1859,130467.86999988556,27.0625
1860,130513.75999999046,27.0625
1861,130537.55999994278,27.0625
1862,130560.52999997139,27.0625
1863,130584.58999991417,27.0625
1864,130726.43000006676,27.0625
1865,130749.21000003815,27.0625
1866,130772.14999985695,27.0625
1867,130794.95000004768,27.0625
1868,130817.9200000763,27.0625
1869,130840.98000001907,27.0625
1870,130864.54999995232,27.0625
1871,130888.62999987602,27.0625
1872,130912.29999995232,27.0625
1873,130936.53999996185,27.0625
1874,130960.55999994278,27.0625
1875,130983.88999986649,27.0625
1876,131007.77999997139,27.0625
1877,131031.22000002861,27.0625
1878,131055.5,27.0625
1879,131195.64999985695,27.0625
1880,131219.30999994278,27.0625
1881,131243.28999996185,27.0625
1882,131268.24000000954,27.0625
1883,131291.6700000763,27.0625
1884,131315.55999994278,27.0625
1885,131338.71000003815,27.0625
1886,131361.4700000286,27.0625
1887,131384.3599998951,27.0625
1888,131408.1399998665,27.0625
1889,131431.96000003815,27.0625
1890,131456.06999993324,27.0625
1891,131480.7799999714,27.0625
1892,131591.19000005722,27.0625
1893,131614.69000005722,27.0625
1894,131638.03999996185,27.0625
1895,131662.1700000763,27.0625
1896,131685.74000000954,27.0625
1897,131708.94000005722,27.0625
1898,131732.7200000286,27.0625
1899,131756.37999987602,27.0625
1900,131780.1099998951,27.0625
1901,131804.44000005722,27.0625
1902,131827.53999996185,27.0625
1903,131850.29999995232,27.0625
1904,131874.16000008583,27.0625
1905,131897.46000003815,27.0625
1906,131921.51999998093,27.0625
1907,131944.86999988556,27.0625
1908,131968.3599998951,27.0625
1909,132169.50999999046,27.125
1910,132192.98000001907,27.125
1911,132216.75999999046,27.0625
1912,132239.5,27.125
1913,132263.46000003815,27.125
1914,132287.49000000954,27.125
1915,132311.30999994278,27.125
1916,132334.87999987602,27.0625
1917,132358.51999998093,27.0625
1918,132382.55999994278,27.0625
1919,132406.45000004768,27.0625
1920,132430.81999993324,27.0625
1921,132454.87999987602,27.0625
1922,132478.44000005722,27.0625
1923,132501.6099998951,27.0625
1924,132525.43000006676,27.0625
1925,132549.3299999237,27.0625
1926,132720.11999988556,27.0625
1927,132744.84999990463,27.0625
1928,132768.7799999714,27.0625
1929,132793.06999993324,27.0625
1930,132817.28999996185,27.0625
1931,132840.33999991417,27.0625
1932,132864.03999996185,27.0625
1933,132887.06999993324,27.0625
1934,132910.9200000763,27.0625
1935,132934.1399998665,27.0625
1936,132957.25999999046,27.125
1937,132981.56999993324,27.0625
1938,133004.25,27.0625
1939,133027.76999998093,27.0625
1940,133051.49000000954,27.0625
1941,133074.39999985695,27.0625
1942,133245.6099998951,27.0625
1943,133268.34999990463,27.125
1944,133291.4700000286,27.125
1945,133314.53999996185,27.125
1946,133337.39999985695,27.125
1947,133360.24000000954,27.125
1948,133382.99000000954,27.0625
1949,133405.75999999046,27.0625
1950,133429.8899998665,27.0625
1951,133454.44000005722,27.0625
1952,133477.75,27.0625
1953,133501.31999993324,27.0625
1954,133525.75999999046,27.0625
1955,133550.03999996185,27.0625
1956,133574.08999991417,27.0625
1957,133599.78999996185,27.125
1958,133623.0799999237,27.0625
1959,133646.6099998951,27.0625
1960,133758.00999999046,27.0625
1961,133782.28999996185,27.0625
1962,133806.25999999046,27.0625
1963,133830.0,27.0625
1964,133853.83999991417,27.0625
1965,133877.51999998093,27.0625
1966,133900.2200000286,27.0625
1967,133923.14999985695,27.125
1968,133947.26999998093,27.0625
1969,133971.1700000763,27.0625
1970,133994.19000005722,27.0625
1971,134017.03999996185,27.0625
1972,134039.76999998093,27.125
1973,134063.56999993324,27.0625
1974,134087.74000000954,27.0625
1975,134110.96000003815,27.0625
1976,134134.05999994278,27.0625
1977,134156.8899998665,27.0625
1978,134327.6399998665,27.125
1979,134351.36999988556,27.125
1980,134375.04999995232,27.125
1981,134398.08999991417,27.125
1982,134422.1099998951,27.125
1983,134445.98000001907,27.125
1984,134469.81999993324,27.125
1985,134494.4200000763,27.0625
1986,134517.78999996185,27.0625
1987,134540.74000000954,27.0625
1988,134563.98000001907,27.0625
1989,134588.24000000954,27.125
1990,134611.29999995232,27.0625
1991,134635.59999990463,27.0625
1992,134822.95000004768,27.0625
1993,134846.26999998093,27.0625
1994,134869.94000005722,27.0625
1995,134893.93000006676,27.0625
1996,134916.96000003815,27.0625
1997,134940.1099998951,27.0625
1998,134963.81999993324,27.125
1999,134987.7799999714,27.125
2000,135010.79999995232,27.0625
2001,135034.3899998665,27.0625
2002,135058.0,27.0625
2003,135082.03999996185,27.0625
2004,135105.4200000763,27.125
2005,135216.59999990463,27.125
2006,135239.89999985695,27.125
2007,135265.51999998093,27.125
2008,135289.69000005722,27.0625
2009,135313.46000003815,27.125
2010,135338.04999995232,27.125
2011,135362.25999999046,27.125
2012,135385.23000001907,27.125
2013,135408.79999995232,27.125
2014,135432.04999995232,27.0625
2015,135455.98000001907,27.125
2016,135479.86999988556,27.125
2017,135503.43000006676,27.0625
2018,135527.39999985695,27.0625
2019,135668.64999985695,27.125
2020,135692.80999994278,27.125
2021,135715.99000000954,27.125
2022,135739.09999990463,27.125
2023,135763.49000000954,27.0625
2024,135786.81999993324,27.0625
2025,135809.7799999714,27.125
2026,135833.26999998093,27.125
2027,135857.44000005722,27.0625
2028,135881.1099998951,27.125
2029,135904.29999995232,27.125
2030,135928.3599998951,27.0625
2031,135951.56999993324,27.125
2032,135974.6399998665,27.125
2033,135998.16000008583,27.125
2034,136021.1700000763,27.0625
2035,136043.81999993324,27.0625
2036,136154.99000000954,27.125
2037,136178.6099998951,27.125
2038,136202.3599998951,27.125
2039,136226.3599998951,27.125
2040,136250.34999990463,27.125
2041,136275.29999995232,27.125
2042,136300.3599998951,27.125
2043,136323.4200000763,27.0625
2044,136346.8899998665,27.125
2045,136370.41000008583,27.0625
2046,136394.03999996185,27.125
2047,136565.49000000954,27.0625
2048,136590.1399998665,27.125
2049,136613.4700000286,27.0625
2050,136637.46000003815,27.0625
2051,136660.33999991417,27.0625
2052,136683.28999996185,27.125
2053,136706.79999995232,27.125
2054,136730.21000003815,27.125
2055,136754.36999988556,27.0625
2056,136778.3899998665,27.0625
2057,136801.44000005722,27.0625
2058,136825.2200000286,27.0625
2059,136848.1099998951,27.0625
2060,136871.25999999046,27.0625
2061,136895.29999995232,27.0625
2062,136919.37999987602,27.125
2063,136942.1399998665,27.0625
2064,136965.96000003815,27.0625
2065,136989.20000004768,27.125
2066,137012.48000001907,27.125
2067,137036.1399998665,27.125
2068,137059.86999988556,27.125
2069,137083.43000006676,27.0625
2070,137107.03999996185,27.125
2071,137130.73000001907,27.125
2072,137153.94000005722,27.0625
2073,137177.91000008583,27.0625
2074,137202.24000000954,27.0625
2075,137226.95000004768,27.0625
2076,137250.26999998093,27.0625
2077,137405.74000000954,27.125
2078,137429.28999996185,27.125
2079,137453.25999999046,27.0625
2080,137476.78999996185,27.125
2081,137500.58999991417,27.0625
2082,137524.53999996185,27.125
2083,137548.31999993324,27.125
2084,137571.33999991417,27.0625
2085,137594.74000000954,27.0625
2086,137617.79999995232,27.0625
2087,137640.41000008583,27.125
2088,137664.59999990463,27.125
2089,137687.20000004768,27.0625
2090,137710.2200000286,27.125
2091,137733.83999991417,27.125
2092,137757.03999996185,27.125
2093,137781.30999994278,27.125
2094,137921.71000003815,27.125
2095,137944.69000005722,27.125
2096,137992.21000003815,27.125
2097,138015.34999990463,27.125
2098,138039.48000001907,27.125
2099,138062.4700000286,27.125
2100,138085.96000003815,27.125
2101,138109.01999998093,27.0625
2102,138132.48000001907,27.0625
2103,138156.31999993324,27.0625
2104,138179.6399998665,27.0625
2105,138202.7799999714,27.125
2106,138226.0,27.125
2107,138249.8899998665,27.125
2108,138390.33999991417,27.125
2109,138414.25999999046,27.125
2110,138436.7799999714,27.0625
2111,138460.39999985695,27.0625
2112,138483.30999994278,27.0625
2113,138506.36999988556,27.0625
2114,138530.55999994278,27.125
2115,138553.99000000954,27.125
2116,138577.04999995232,27.125
2117,138625.5299999714,27.0625
2118,138649.45000004768,27.125
2119,138760.6399998665,27.0625
2120,138784.84999990463,27.125
2121,138807.55999994278,27.0625
2122,138831.8299999237,27.0625
2123,138855.36999988556,27.0625
2124,138878.44000005722,27.0625
2125,138901.6700000763,27.125
2126,138942.0799999237,27.0625
2127,138966.18000006676,27.0625
2128,138989.20000004768,27.0625
2129,139013.6099998951,27.125
2130,139037.86999988556,27.125
2131,139149.1700000763,27.125
2132,139190.48000001907,27.125
2133,139213.23000001907,27.0625
2134,139236.49000000954,27.0625
2135,139260.4700000286,27.0625
2136,139283.25,27.0625
2137,139306.76999998093,27.0625
2138,139330.16000008583,27.0625
2139,139354.08999991417,27.0625
2140,139377.24000000954,27.0625
2141,139400.91000008583,27.0625
2142,139470.74000000954,27.0625
2143,139493.55999994278,27.0625
2144,139673.0299999714,27.0625
2145,139697.11999988556,27.0625
2146,139720.98000001907,27.0625
2147,139744.06999993324,27.0625
2148,139767.03999996185,27.0625
2149,139791.1099998951,27.0625
2150,139814.53999996185,27.0625
2151,139838.71000003815,27.0625
2152,139861.26999998093,27.125
2153,139884.54999995232,27.0625
2154,139908.66000008583,27.0625
2155,139932.37999987602,27.0625
2156,139956.19000005722,27.0625
2157,140066.75,27.125
2158,140089.94000005722,27.0625
2159,140113.25,27.0625
2160,140137.14999985695,27.0625
2161,140160.2799999714,27.0625
2162,140184.51999998093,27.0625
2163,140207.1099998951,27.0625
2164,140230.45000004768,27.0625
2165,140254.93000006676,27.0625
2166,140278.45000004768,27.0625
2167,140301.70000004768,27.0625
2168,140412.51999998093,27.0625
2169,140436.30999994278,27.0625
2170,140459.53999996185,27.0625
2171,140482.94000005722,27.0625
2172,140507.16000008583,27.0625
2173,140530.95000004768,27.0625
2174,140554.44000005722,27.0625
2175,140577.8899998665,27.0625
2176,140601.9700000286,27.0625
2177,140625.01999998093,27.0625
2178,140648.23000001907,27.0625
2179,140671.7200000286,27.0625
2180,140695.51999998093,27.0625
2181,140718.18000006676,27.0625
2182,140741.89999985695,27.0625
2183,140852.6099998951,27.0625
2184,140875.4200000763,27.0625
2185,140899.59999990463,27.0625
2186,140922.70000004768,27.0625
2187,140992.28999996185,27.0625
2188,141015.59999990463,27.0625
2189,141063.6099998951,27.0625
2190,141087.36999988556,27.0625
2191,141111.06999993324,27.0625
2192,141134.33999991417,27.0625
2193,141158.05999994278,27.0625
2194,141268.34999990463,27.125
2195,141293.1399998665,27.0625
2196,141316.7200000286,27.0625
2197,141339.44000005722,27.125
2198,141363.11999988556,27.0625
2199,141386.26999998093,27.0625
2200,141409.20000004768,27.125
2201,141433.2200000286,27.0625
2202,141457.6399998665,27.125
2203,141481.78999996185,27.0625
2204,141505.80999994278,27.0625
2205,141723.49000000954,27.125
2206,141747.51999998093,27.125
2207,141770.8599998951,27.0625
2208,141795.1700000763,27.0625
2209,141818.05999994278,27.0625
2210,141841.39999985695,27.0625
2211,141864.30999994278,27.0625
2212,141887.46000003815,27.0625
2213,141911.05999994278,27.0625
2214,141935.09999990463,27.0625
2215,141958.8299999237,27.0625
2216,141981.95000004768,27.0625
2217,142005.7799999714,27.0625
2218,142029.62999987602,27.0625
2219,142054.00999999046,27.0625
2220,142077.26999998093,27.0625
2221,142255.30999994278,27.0625
2222,142279.4200000763,27.0625
2223,142302.46000003815,27.0625
2224,142326.6700000763,27.0625
2225,142349.51999998093,27.0625
2226,142372.54999995232,27.0625
2227,142395.45000004768,27.0625
2228,142419.44000005722,27.0625
2229,142443.3599998951,27.0625
2230,142467.1399998665,27.0625
2231,142511.4200000763,27.0625
2232,142535.06999993324,27.0625
2233,142676.6099998951,27.0625
2234,142699.58999991417,27.0625
2235,142722.56999993324,27.0625
2236,142746.74000000954,27.0625
2237,142769.6099998951,27.0625
2238,142793.5799999237,27.0625
2239,142817.11999988556,27.0625
2240,142840.99000000954,27.0625
2241,142864.8899998665,27.0625
2242,142889.45000004768,27.0625
2243,142912.8899998665,27.0625
2244,142935.5299999714,27.0625
2245,142959.12999987602,27.0625
2246,142982.41000008583,27.0625
2247,143006.4700000286,27.0625
2248,143029.19000005722,27.0625
2249,143169.80999994278,27.0625
2250,143193.33999991417,27.0625
2251,143217.33999991417,27.0625
2252,143240.31999993324,27.0625
2253,143263.71000003815,27.0625
2254,143286.29999995232,27.0625
2255,143309.59999990463,27.0625
2256,143332.84999990463,27.0625
2257,143374.87999987602,27.0625
2258,143398.89999985695,27.0625
2259,143424.30999994278,27.0625
2260,143448.59999990463,27.0625
2261,143472.7200000286,27.0625
2262,143496.18000006676,27.0625
2263,143519.75,27.0625
2264,143661.64999985695,27.0625
2265,143686.06999993324,27.0625
2266,143709.20000004768,27.0625
2267,143733.39999985695,27.0625
2268,143757.1399998665,27.0625
2269,143780.83999991417,27.0625
2270,143804.37999987602,27.0625
2271,143827.56999993324,27.0625
2272,143851.6700000763,27.0625
2273,143875.4200000763,27.0625
2274,143899.6700000763,27.0625
2275,143923.87999987602,27.0625
2276,143946.79999995232,27.0625
2277,144058.29999995232,27.0625
2278,144081.03999996185,27.0625
2279,144103.5799999237,27.0625
2280,144150.19000005722,27.0625
2281,144173.44000005722,27.0625
2282,144197.84999990463,27.0625
2283,144221.11999988556,27.0625
2284,144244.6700000763,27.0625
2285,144268.0,27.0625
2286,144291.31999993324,27.0625
2287,144314.55999994278,27.0625
2288,144338.51999998093,27.0625
2289,144361.18000006676,27.0625
2290,144384.73000001907,27.0625
2291,144526.6399998665,27.0625
2292,144550.4700000286,27.0625
2293,144574.34999990463,27.0625
2294,144620.5799999237,27.0625
2295,144643.29999995232,27.0625
2296,144712.31999993324,27.0625
2297,144736.0299999714,27.0625
2298,144758.96000003815,27.0
2299,144783.66000008583,27.0625
2300,144808.0,27.0625
2301,144832.1099998951,27.0625
2302,144942.43000006676,27.0625
2303,144966.1099998951,27.0625
2304,144989.74000000954,27.0625
2305,145013.6099998951,27.0625
2306,145036.20000004768,27.0625
2307,145060.2799999714,27.0625
2308,145083.36999988556,27.0625
2309,145154.91000008583,27.0625
2310,145178.4200000763,27.0625
2311,145203.09999990463,27.0625
2312,145452.84999990463,27.0625
2313,145475.5799999237,27.0625
2314,145499.14999985695,27.0625
2315,145522.34999990463,27.0625
2316,145546.50999999046,27.0625
2317,145570.44000005722,27.0625
2318,145594.2799999714,27.0625
2319,145617.36999988556,27.0625
2320,145640.54999995232,27.0625
2321,145663.6399998665,27.0625
2322,145687.14999985695,27.0625
2323,145711.75999999046,27.0625
2324,145758.70000004768,27.0625
2325,145782.3899998665,27.0625
2326,145805.56999993324,27.0625
2327,145947.25,27.0625
2328,145971.14999985695,27.0625
2329,145994.53999996185,27.0625
2330,146018.6399998665,27.0625
2331,146041.80999994278,27.0625
2332,146064.6700000763,27.0625
2333,146087.87999987602,27.0625
2334,146111.6099998951,27.0625
2335,146134.46000003815,27.0625
2336,146160.93000006676,27.0625
2337,146184.0799999237,27.0625
2338,146206.83999991417,27.0625
2339,146230.96000003815,27.0625
2340,146253.5799999237,27.0625
2341,146278.0299999714,27.0625
2342,146448.8899998665,27.0625
2343,146472.39999985695,27.0625
2344,146495.3899998665,27.0625
2345,146519.48000001907,27.0625
2346,146543.45000004768,27.0625
2347,146567.28999996185,27.0625
2348,146589.79999995232,27.0625
2349,146613.75,27.0625
2350,146637.45000004768,27.0625
2351,146661.83999991417,27.0625
2352,146684.70000004768,27.0625
2353,146707.74000000954,27.0625
2354,146730.73000001907,27.0625
2355,146753.4700000286,27.0625
2356,146777.37999987602,27.0625
2357,146801.55999994278,27.0625
2358,146935.36999988556,27.0625
2359,146959.5799999237,27.0625
2360,146983.3899998665,27.0625
2361,147006.64999985695,27.0625
2362,147030.3599998951,27.0625
2363,147055.05999994278,27.0625
2364,147079.26999998093,27.0625
2365,147102.1099998951,27.0625
2366,147126.26999998093,27.0625
2367,147150.49000000954,27.0625
2368,147174.68000006676,27.0625
2369,147197.41000008583,27.0625
2370,147220.37999987602,27.0625
2371,147243.68000006676,27.0625
2372,147267.1399998665,27.0625
2373,147409.01999998093,27.0625
2374,147432.11999988556,27.0625
2375,147456.51999998093,27.0625
2376,147480.79999995232,27.0625
2377,147504.08999991417,27.0
2378,147527.8899998665,27.0625
2379,147552.18000006676,27.0
2380,147575.44000005722,27.0625
2381,147598.68000006676,27.0625
2382,147621.69000005722,27.0625
2383,147644.6399998665,27.0625
2384,147667.54999995232,27.0625
2385,147691.3599998951,27.0625
2386,147715.6399998665,27.0625
2387,147738.20000004768,27.0625
2388,147761.86999988556,27.0625
2389,147786.03999996185,27.0625
2390,147956.36999988556,27.0625
2391,147979.1700000763,27.0625
2392,148003.49000000954,27.0625
2393,148026.69000005722,27.0625
2394,148051.25999999046,27.0625
2395,148074.6399998665,27.0625
2396,148099.75,27.0625
2397,148124.3599998951,27.0625
2398,148147.45000004768,27.0625
2399,148170.83999991417,27.0625
2400,148194.74000000954,27.0
2401,148218.70000004768,27.0625
2402,148242.69000005722,27.0625
2403,148266.76999998093,27.0625
2404,148289.74000000954,27.0625
2405,148312.8599998951,27.0
2406,148335.94000005722,27.0625
2407,148446.56999993324,27.0625
2408,148515.55999994278,27.0
2409,148538.54999995232,27.0625
2410,148561.51999998093,27.0625
2411,148585.5299999714,27.0625
2412,148608.7799999714,27.0625
2413,148631.96000003815,27.0625
2414,148656.09999990463,27.0625
2415,148680.24000000954,27.0
2416,148704.25999999046,27.0625
2417,148726.96000003815,27.0
2418,148838.8599998951,27.0625
2419,148863.16000008583,27.0625
2420,148886.04999995232,27.0625
2421,148909.44000005722,27.0625
2422,148932.2799999714,27.0625
2423,148955.37999987602,27.0
2424,148979.09999990463,27.0
2425,149003.56999993324,27.0
2426,149026.2200000286,27.0
2427,149049.33999991417,27.0
2428,149072.4200000763,27.0625
2429,149095.4700000286,27.0625
2430,149119.61999988556,27.0625
2431,149143.48000001907,27.0625
2432,149167.31999993324,27.0625
2433,149190.4200000763,27.0625
2434,149361.09999990463,27.0625
2435,149385.1399998665,27.0625
2436,149409.3899998665,27.0625
2437,149433.37999987602,27.0625
2438,149456.50999999046,27.0625
2439,149480.45000004768,27.0625
2440,149503.11999988556,27.0625
2441,149526.34999990463,27.0625
2442,149550.33999991417,27.0
2443,149573.39999985695,27.0625
2444,149596.75999999046,27.0625
2445,149620.46000003815,27.0625
2446,149643.11999988556,27.0625
2447,149813.89999985695,27.0625
2448,149837.25,27.0625
2449,149860.6399998665,27.0625
2450,149884.44000005722,27.0
2451,149926.8899998665,27.0625
2452,149949.94000005722,27.0625
2453,149974.1399998665,27.0
2454,149998.12999987602,27.0625
2455,150022.19000005722,27.0625
2456,150045.51999998093,27.0
2457,150069.74000000954,27.0625
2458,150092.45000004768,27.0625
2459,150115.93000006676,27.0625
2460,150138.95000004768,27.0625
2461,150310.11999988556,27.0625
2462,150333.24000000954,27.0625
2463,150355.8899998665,27.0625
2464,150378.61999988556,27.0625
2465,150402.14999985695,27.0625
2466,150425.3299999237,27.0625
2467,150448.25999999046,27.0625
2468,150470.8599998951,27.0625
2469,150493.9200000763,27.0625
2470,150518.20000004768,27.0
2471,150541.11999988556,27.0625
2472,150564.33999991417,27.0625
2473,150588.33999991417,27.0625
2474,150611.4200000763,27.0625
2475,150635.46000003815,27.0625
2476,150660.28999996185,27.0625
2477,150770.8899998665,27.0625
2478,150794.7799999714,27.0625
2479,150817.94000005722,27.0625
2480,150840.87999987602,27.0625
2481,150864.56999993324,27.0625
2482,150887.2799999714,27.0625
2483,150911.3299999237,27.0625
2484,150934.48000001907,27.0625
2485,150957.5799999237,27.0625
2486,150981.37999987602,27.0
2487,151005.30999994278,27.0625
2488,151029.20000004768,27.0625
2489,151053.1700000763,27.0625
2490,151076.37999987602,27.0625
2491,151100.55999994278,27.0625
2492,151123.69000005722,27.0625
2493,151147.56999993324,27.0625
2494,151171.8599998951,27.0625
2495,151402.89999985695,27.0625
2496,151426.06999993324,27.0625
2497,151450.01999998093,27.0625
2498,151472.7799999714,27.0625
2499,151495.83999991417,27.0625
2500,151518.9700000286,27.0
2501,151542.2200000286,27.0625
2502,151565.76999998093,27.0625
2503,151589.48000001907,27.0625
2504,151613.19000005722,27.0625
2505,151637.1399998665,27.0625
2506,151660.99000000954,27.0625
2507,151684.58999991417,27.0625
2508,151885.71000003815,27.0625
2509,151908.39999985695,27.0625
2510,151932.84999990463,27.0
2511,151955.78999996185,27.0625
2512,151978.8899998665,27.0625
2513,152001.55999994278,27.0625
2514,152025.61999988556,27.0
2515,152049.8299999237,27.0625
2516,152073.73000001907,27.0
2517,152097.58999991417,27.0
2518,152121.56999993324,27.0
2519,152144.54999995232,27.0
2520,152168.58999991417,27.0
2521,152192.1399998665,27.0
2522,152396.09999990463,26.9375
2523,152419.87999987602,26.9375
2524,152443.8599998951,26.9375
2525,152466.4700000286,26.9375
2526,152489.54999995232,26.9375
2527,152513.8899998665,26.9375
2528,152561.5299999714,26.9375
2529,152584.49000000954,26.9375
2530,152608.03999996185,26.9375
2531,152631.2200000286,26.9375
2532,152653.73000001907,26.875
2533,152676.81999993324,26.9375
2534,152699.87999987602,26.9375
2535,152723.8899998665,26.9375
2536,152864.89999985695,26.9375
2537,152887.98000001907,26.875
2538,152912.4700000286,26.9375
2539,152936.5,26.875
2540,152960.03999996185,26.875
2541,152983.09999990463,26.875
2542,153007.1399998665,26.875
2543,153031.24000000954,26.875
2544,153054.24000000954,26.875
2545,153077.37999987602,26.875
2546,153100.04999995232,26.875
2547,153124.05999994278,26.875
2548,153146.64999985695,26.875
2549,153170.46000003815,26.875
2550,153194.2799999714,26.875
2551,153218.1399998665,26.875
2552,153241.98000001907,26.875
2553,153383.5,26.875
2554,153408.1399998665,26.875
2555,153431.79999995232,26.875
2556,153454.6700000763,26.875
2557,153478.33999991417,26.875
2558,153502.1399998665,26.875
2559,153525.7200000286,26.875
2560,153548.94000005722,26.875
2561,153571.50999999046,26.875
2562,153594.75999999046,26.875
2563,153617.9700000286,26.875
2564,153641.1399998665,26.875
2565,153665.11999988556,26.875
2566,153689.1099998951,26.875
2567,153712.05999994278,26.875
2568,153735.11999988556,26.8125
2569,153935.44000005722,26.875
2570,153959.04999995232,26.875
2571,153982.03999996185,26.8125
2572,154005.62999987602,26.875
2573,154029.18000006676,26.8125
2574,154052.2200000286,26.8125
2575,154076.59999990463,26.8125
2576,154100.98000001907,26.8125
2577,154125.25,26.8125
2578,154147.8299999237,26.8125
2579,154171.75,26.8125
2580,154195.05999994278,26.8125
2581,154218.87999987602,26.8125
2582,154242.94000005722,26.8125
2583,154266.18000006676,26.8125
2584,154289.1099998951,26.8125
2585,154312.84999990463,26.8125
2586,154424.03999996185,26.8125
2587,154446.6099998951,26.8125
2588,154470.41000008583,26.8125
2589,154493.37999987602,26.8125
2590,154516.23000001907,26.8125
2591,154539.06999993324,26.8125
2592,154562.1399998665,26.8125
2593,154585.96000003815,26.8125
2594,154608.89999985695,26.8125
2595,154633.0299999714,26.8125
2596,154656.18000006676,26.8125
2597,154679.50999999046,26.8125
2598,154702.33999991417,26.8125
2599,154725.6099998951,26.8125
2600,154749.51999998093,26.8125
2601,154772.33999991417,26.8125
2602,154982.5,26.8125
2603,155006.14999985695,26.8125
2604,155030.04999995232,26.8125
2605,155054.6399998665,26.8125
2606,155077.33999991417,26.8125
2607,155102.25,26.8125
2608,155125.64999985695,26.8125
2609,155149.3899998665,26.8125
2610,155172.9200000763,26.8125
2611,155196.45000004768,26.8125
2612,155219.6099998951,26.8125
2613,155243.56999993324,26.75
2614,155266.4200000763,26.75
2615,155290.18000006676,26.75
2616,155313.01999998093,26.75
2617,155336.34999990463,26.75
2618,155359.24000000954,26.75
2619,155382.81999993324,26.75
2620,155523.39999985695,26.75
2621,155547.01999998093,26.75
2622,155570.96000003815,26.8125
2623,155593.45000004768,26.75
2624,155616.45000004768,26.75
2625,155639.39999985695,26.75
2626,155662.11999988556,26.75
2627,155684.71000003815,26.75
2628,155708.43000006676,26.75
2629,155731.25999999046,26.75
2630,155755.16000008583,26.75
2631,155777.80999994278,26.75
2632,155800.59999990463,26.75
2633,155823.66000008583,26.75
2634,155847.25999999046,26.75
2635,155958.33999991417,26.75
2636,155981.61999988556,26.75
2637,156004.86999988556,26.75
2638,156028.0799999237,26.75
2639,156052.18000006676,26.75
2640,156075.8899998665,26.75
2641,156099.39999985695,26.75
2642,156123.09999990463,26.75
2643,156146.61999988556,26.75
2644,156193.6700000763,26.75
2645,156216.37999987602,26.75
2646,156241.20000004768,26.75
2647,156263.83999991417,26.75
2648,156287.33999991417,26.75
2649,156311.24000000954,26.75
2650,156422.37999987602,26.75
2651,156445.18000006676,26.75
2652,156469.86999988556,26.75
2653,156492.75999999046,26.75
2654,156516.68000006676,26.75
2655,156539.93000006676,26.75
2656,156563.78999996185,26.75
2657,156587.58999991417,26.75
2658,156610.55999994278,26.75
2659,156633.55999994278,26.75
2660,156657.3899998665,26.75
2661,156680.49000000954,26.75
2662,156704.3899998665,26.6875
2663,156905.36999988556,26.75
2664,156928.75,26.75
2665,156953.11999988556,26.75
2666,156976.33999991417,26.75
2667,156999.74000000954,26.6875
2668,157041.75999999046,26.75
2669,157064.8299999237,26.75
2670,157089.24000000954,26.75
2671,157159.4700000286,26.75
2672,157183.44000005722,26.75
2673,157207.69000005722,26.75
2674,157230.98000001907,26.75
2675,157432.29999995232,26.75
2676,157455.84999990463,26.75
2677,157479.70000004768,26.75
2678,157504.08999991417,26.75
2679,157527.44000005722,26.75
2680,157550.3599998951,26.75
2681,157573.9700000286,26.75
2682,157597.9200000763,26.75
2683,157621.58999991417,26.6875
2684,157644.74000000954,26.75
2685,157667.26999998093,26.75
2686,157690.93000006676,26.75
2687,157714.29999995232,26.75
2688,157738.29999995232,26.6875
2689,157762.09999990463,26.75
2690,157785.28999996185,26.75
2691,157895.81999993324,26.75
2692,157918.70000004768,26.75
2693,157942.6700000763,26.75
2694,157966.37999987602,26.75
2695,157989.2799999714,26.75
2696,158013.1700000763,26.75
2697,158037.61999988556,26.75
2698,158060.41000008583,26.6875
2699,158084.55999994278,26.75
2700,158109.0,26.75
2701,158132.0799999237,26.75
2702,158155.00999999046,26.75
2703,158178.16000008583,26.75
2704,158202.20000004768,26.75
2705,158225.7799999714,26.75
2706,158248.8599998951,26.75
2707,158272.62999987602,26.75
2708,158295.9200000763,26.75
2709,158407.1399998665,26.75
2710,158452.0,26.75
2711,158475.44000005722,26.75
2712,158499.03999996185,26.75
2713,158523.41000008583,26.75
2714,158546.95000004768,26.75
2715,158571.01999998093,26.75
2716,158594.1399998665,26.75
2717,158617.2799999714,26.75
2718,158641.55999994278,26.75
2719,158665.64999985695,26.75
2720,158688.58999991417,26.75
2721,158711.6700000763,26.75
2722,158734.4200000763,26.75
2723,158757.74000000954,26.75
2724,158780.51999998093,26.75
2725,158984.1399998665,26.75
2726,159007.1099998951,26.75
2727,159030.96000003815,26.75
2728,159055.3899998665,26.75
2729,159079.06999993324,26.75
2730,159102.5,26.75
2731,159126.96000003815,26.75
2732,159149.91000008583,26.75
2733,159173.70000004768,26.75
2734,159197.66000008583,26.75
2735,159220.34999990463,26.75
2736,159243.01999998093,26.75
2737,159267.05999994278,26.75
2738,159290.6399998665,26.75
2739,159314.14999985695,26.75
2740,159338.3599998951,26.75
2741,159449.99000000954,26.75
2742,159473.0,26.75
2743,159497.1399998665,26.75
2744,159519.93000006676,26.75
2745,159543.75999999046,26.75
2746,159567.49000000954,26.75
2747,159590.59999990463,26.75
2748,159614.68000006676,26.75
2749,159638.14999985695,26.75
2750,159661.30999994278,26.75
2751,159684.06999993324,26.75
2752,159707.71000003815,26.75
2753,159730.34999990463,26.75
2754,159754.93000006676,26.75
2755,159866.3899998665,26.75
2756,159889.94000005722,26.75
2757,159912.94000005722,26.75
2758,159936.86999988556,26.75
2759,159959.98000001907,26.75
2760,159983.95000004768,26.75
2761,160006.59999990463,26.75
2762,160029.74000000954,26.75
2763,160054.03999996185,26.75
2764,160077.16000008583,26.75
2765,160099.70000004768,26.75
2766,160123.4200000763,26.75
2767,160170.3299999237,26.75
2768,160194.51999998093,26.75
2769,160336.2799999714,26.75
2770,160378.49000000954,26.75
2771,160402.08999991417,26.75
2772,160425.93000006676,26.75
2773,160448.8899998665,26.75
2774,160472.95000004768,26.8125
2775,160496.25999999046,26.8125
2776,160519.20000004768,26.8125
2777,160541.91000008583,26.8125
2778,160564.5299999714,26.8125
2779,160588.03999996185,26.8125
2780,160698.94000005722,26.8125
2781,160722.6700000763,26.8125
2782,160746.6099998951,26.8125
2783,160770.69000005722,26.75
2784,160794.9700000286,26.8125
2785,160819.09999990463,26.8125
2786,160841.98000001907,26.8125
2787,160865.99000000954,26.8125
2788,160889.3899998665,26.8125
2789,160912.14999985695,26.8125
2790,160936.30999994278,26.8125
2791,160960.3899998665,26.8125
2792,160984.06999993324,26.8125
2793,161214.86999988556,26.8125
2794,161238.75,26.8125
2795,161262.24000000954,26.8125
2796,161285.54999995232,26.8125
2797,161333.01999998093,26.8125
2798,161357.11999988556,26.8125
2799,161379.78999996185,26.8125
2800,161403.8599998951,26.8125
2801,161427.01999998093,26.8125
2802,161450.64999985695,26.8125
2803,161473.64999985695,26.8125
2804,161497.0799999237,26.8125
2805,161520.5799999237,26.8125
2806,161544.87999987602,26.8125
2807,161568.48000001907,26.8125
2808,161593.03999996185,26.8125
2809,161616.30999994278,26.8125
2810,161727.31999993324,26.8125
2811,161750.6399998665,26.8125
2812,161774.37999987602,26.8125
2813,161798.45000004768,26.8125
2814,161823.05999994278,26.875
2815,161847.3599998951,26.8125
2816,161871.12999987602,26.8125
2817,161895.1099998951,26.8125
2818,161918.30999994278,26.8125
2819,161941.51999998093,26.8125
2820,161965.39999985695,26.8125
2821,161989.0,26.8125
2822,162012.96000003815,26.8125
2823,162035.96000003815,26.8125
2824,162058.79999995232,26.875
2825,162083.06999993324,26.8125
2826,162107.06999993324,26.8125
2827,162248.0,26.875
2828,162272.0,26.875
2829,162295.56999993324,26.875
2830,162319.33999991417,26.875
2831,162342.58999991417,26.875
2832,162365.34999990463,26.875
2833,162390.00999999046,26.875
2834,162413.3299999237,26.875
2835,162436.5799999237,26.875
2836,162460.00999999046,26.875
2837,162483.74000000954,26.875
2838,162506.8599998951,26.875
2839,162529.34999990463,26.875
2840,162552.03999996185,26.875
2841,162576.03999996185,26.875
2842,162599.79999995232,26.875
2843,162622.53999996185,26.875
2844,162792.91000008583,26.875
2845,162815.80999994278,26.875
2846,162839.81999993324,26.875
2847,162863.25999999046,26.875
2848,162886.87999987602,26.875
2849,162909.5,26.875
2850,162932.81999993324,26.875
2851,162957.34999990463,26.9375
2852,162980.6700000763,26.875
2853,163004.64999985695,26.9375
2854,163028.03999996185,26.875
2855,163051.6099998951,26.875
2856,163074.64999985695,26.875
2857,163098.64999985695,26.875
2858,163121.21000003815,26.875
2859,163145.7799999714,26.875
2860,163365.87999987602,26.9375
2861,163388.89999985695,26.9375
2862,163412.26999998093,26.9375
2863,163435.3899998665,26.9375
2864,163460.00999999046,26.9375
2865,163482.95000004768,26.9375
2866,163506.76999998093,26.9375
2867,163531.2799999714,26.9375
2868,163554.94000005722,26.9375
2869,163577.6399998665,26.9375
2870,163601.36999988556,26.9375
2871,163625.20000004768,26.9375
2872,163649.21000003815,26.9375
2873,163672.37999987602,26.9375
2874,163696.26999998093,26.9375
2875,163719.49000000954,26.9375
2876,163950.30999994278,26.9375
2877,163974.18000006676,26.9375
2878,163997.86999988556,26.9375
2879,164021.94000005722,26.9375
2880,164044.64999985695,26.9375
2881,164068.6700000763,26.9375
2882,164092.3599998951,26.9375
2883,164115.29999995232,26.9375
2884,164138.41000008583,26.9375
2885,164161.96000003815,26.9375
2886,164185.62999987602,26.9375
2887,164209.69000005722,26.9375
2888,164257.12999987602,26.9375
2889,164280.25,26.9375
2890,164302.99000000954,26.9375
2891,164444.3599998951,27.0
2892,164467.6700000763,27.0
2893,164491.75999999046,27.0
2894,164514.61999988556,27.0
2895,164537.8899998665,27.0
2896,164561.2799999714,27.0
2897,164585.76999998093,27.0
2898,164608.89999985695,27.0
2899,164632.9200000763,27.0
2900,164657.0,27.0
2901,164798.31999993324,27.0
2902,164821.56999993324,27.0
2903,164845.3599998951,27.0
2904,164867.96000003815,27.0
2905,164890.74000000954,27.0
2906,164913.74000000954,27.0
2907,164937.75,27.0
2908,164960.8599998951,27.0
2909,164984.94000005722,27.0
2910,165008.78999996185,27.0
2911,165031.79999995232,27.0
2912,165055.4700000286,27.0
2913,165078.78999996185,27.0
2914,165101.84999990463,27.0
2915,165125.19000005722,27.0
2916,165148.64999985695,27.0
2917,165172.3299999237,27.0
2918,165312.89999985695,27.0625
2919,165336.98000001907,27.0625
2920,165360.71000003815,27.0625
2921,165383.9700000286,27.0
2922,165407.16000008583,27.0625
2923,165477.08999991417,27.0
2924,165500.5799999237,27.0625
2925,165525.30999994278,27.0625
2926,165549.33999991417,27.0625
2927,165573.11999988556,27.0625
2928,165597.18000006676,27.0625
2929,165621.3599998951,27.0625
2930,165645.51999998093,27.0625
2931,165817.1099998951,27.0625
2932,165840.43000006676,27.0625
2933,165864.7200000286,27.0625
2934,165888.7200000286,27.0625
2935,165912.0,27.0625
2936,165936.28999996185,27.0625
2937,165960.2799999714,27.0625
2938,165984.4200000763,27.0625
2939,166007.8599998951,27.0625
2940,166030.74000000954,27.0625
2941,166054.08999991417,27.0625
2942,166077.74000000954,27.0625
2943,166218.69000005722,27.125
2944,166241.53999996185,27.0625
2945,166264.39999985695,27.0625
2946,166289.04999995232,27.0625
2947,166312.59999990463,27.0625
2948,166335.74000000954,27.125
2949,166359.7200000286,27.125
2950,166382.3899998665,27.125
2951,166405.05999994278,27.125
2952,166429.24000000954,27.125
2953,166453.21000003815,27.125
2954,166476.79999995232,27.125
2955,166588.2799999714,27.125
2956,166611.28999996185,27.0625
2957,166634.95000004768,27.125
2958,166659.0799999237,27.125
2959,166681.83999991417,27.125
2960,166704.7200000286,27.125
2961,166728.01999998093,27.125
2962,166752.20000004768,27.125
2963,166775.39999985695,27.125
2964,166901.54999995232,27.125
2965,166924.71000003815,27.125
2966,166948.50999999046,27.125
2967,166972.5,27.125
2968,166995.64999985695,27.125
2969,167019.70000004768,27.125
2970,167130.98000001907,27.125
2971,167154.41000008583,27.125
2972,167177.48000001907,27.125
2973,167200.41000008583,27.125
2974,167223.5799999237,27.1875
2975,167246.70000004768,27.125
2976,167270.74000000954,27.1875
2977,167295.39999985695,27.1875
2978,167318.04999995232,27.1875
2979,167341.99000000954,27.1875
2980,167364.83999991417,27.125
2981,167388.01999998093,27.125
2982,167411.98000001907,27.125
2983,167435.5,27.125
2984,167606.95000004768,27.1875
2985,167631.11999988556,27.1875
2986,167654.46000003815,27.1875
2987,167700.8899998665,27.1875
2988,167724.7799999714,27.1875
2989,167749.21000003815,27.1875
2990,167772.18000006676,27.1875
2991,167795.83999991417,27.1875
2992,167819.25999999046,27.1875
2993,167843.46000003815,27.1875
2994,167868.43000006676,27.1875
2995,167891.14999985695,27.1875
2996,167930.74000000954,27.1875
2997,168042.75,27.1875
2998,168065.75999999046,27.1875
2999,168088.79999995232,27.1875
3000,168111.69000005722,27.1875
3001,168135.2200000286,27.1875
3002,168158.6399998665,27.1875
3003,168182.78999996185,27.1875
3004,168206.2200000286,27.25
3005,168229.19000005722,27.1875
3006,168253.04999995232,27.1875
3007,168276.31999993324,27.25
3008,168299.81999993324,27.1875
3009,168323.83999991417,27.1875
3010,168346.89999985695,27.1875
3011,168458.01999998093,27.25
3012,168481.19000005722,27.25
3013,168504.37999987602,27.1875
3014,168528.05999994278,27.25
3015,168550.94000005722,27.25
3016,168574.78999996185,27.25
3017,168597.5,27.25
3018,168620.39999985695,27.25
3019,168644.33999991417,27.25
3020,168668.41000008583,27.25
3021,168690.9200000763,27.25
3022,168714.80999994278,27.25
3023,168738.87999987602,27.25
3024,168762.05999994278,27.25
3025,168785.0,27.25
3026,168956.83999991417,27.25
3027,168979.76999998093,27.3125
3028,169002.84999990463,27.25
3029,169027.06999993324,27.25
3030,169050.83999991417,27.25
3031,169074.8599998951,27.25
3032,169098.0799999237,27.25
3033,169121.18000006676,27.25
3034,169144.99000000954,27.25
3035,169169.6399998665,27.25
3036,169192.46000003815,27.25
3037,169333.37999987602,27.25
3038,169356.39999985695,27.3125
3039,169380.54999995232,27.3125
3040,169403.4200000763,27.3125
3041,169427.29999995232,27.3125
3042,169450.28999996185,27.3125
3043,169473.87999987602,27.3125
3044,169498.75999999046,27.3125
3045,169522.39999985695,27.3125
3046,169546.87999987602,27.3125
3047,169570.83999991417,27.3125
3048,169593.95000004768,27.3125
3049,169616.6399998665,27.3125
3050,169639.62999987602,27.3125
3051,169663.45000004768,27.3125
3052,169688.58999991417,27.3125
3053,169711.09999990463,27.3125
3054,169736.06999993324,27.3125
3055,169878.62999987602,27.3125
3056,169901.2799999714,27.3125
3057,169925.34999990463,27.3125
3058,169947.9700000286,27.3125
3059,169971.31999993324,27.375
3060,169994.66000008583,27.3125
3061,170018.37999987602,27.3125
3062,170041.24000000954,27.3125
3063,170064.33999991417,27.3125
3064,170087.9700000286,27.375
3065,170111.2799999714,27.375
3066,170134.41000008583,27.3125
3067,170203.59999990463,27.3125
3068,170227.5299999714,27.3125
3069,170250.45000004768,27.375
3070,170273.75,27.3125
3071,170445.18000006676,27.375
3072,170468.80999994278,27.375
3073,170492.69000005722,27.375
3074,170516.01999998093,27.375
3075,170538.71000003815,27.375
3076,170561.76999998093,27.375
3077,170584.7200000286,27.375
3078,170607.71000003815,27.375
3079,170630.79999995232,27.375
3080,170653.53999996185,27.375
3081,170676.6700000763,27.375
3082,170699.96000003815,27.375
3083,170723.79999995232,27.375
3084,170747.50999999046,27.375
3085,170771.7200000286,27.4375
3086,170794.46000003815,27.375
3087,170819.04999995232,27.375
3088,170960.4700000286,27.4375
3089,170983.39999985695,27.4375
3090,171006.0799999237,27.4375
3091,171029.41000008583,27.4375
3092,171053.39999985695,27.4375
3093,171076.37999987602,27.4375
3094,171100.29999995232,27.4375
3095,171123.29999995232,27.4375
3096,171146.46000003815,27.4375
3097,171171.50999999046,27.4375
3098,171194.18000006676,27.4375
3099,171262.91000008583,27.4375
3100,171286.83999991417,27.4375
3101,171310.1099998951,27.4375
3102,171334.04999995232,27.4375
3103,171357.01999998093,27.5
3104,171468.56999993324,27.5
3105,171492.5799999237,27.4375
3106,171515.56999993324,27.5
3107,171539.48000001907,27.5
3108,171566.31999993324,27.5
3109,171589.6700000763,27.5
3110,171613.30999994278,27.5
3111,171638.21000003815,27.5
3112,171662.6700000763,27.5
3113,171685.39999985695,27.5
3114,171709.62999987602,27.5
3115,171733.30999994278,27.5
3116,171757.5,27.5
3117,171780.6700000763,27.5
3118,171803.91000008583,27.5
3119,171826.6399998665,27.5
3120,171850.4200000763,27.5
3121,171961.8599998951,27.5
3122,171985.05999994278,27.5625
3123,172008.37999987602,27.5
3124,172032.26999998093,27.5
3125,172056.37999987602,27.5
3126,172079.39999985695,27.5625
3127,172103.6700000763,27.5
3128,172127.33999991417,27.5625
3129,172151.03999996185,27.5625
3130,172173.6700000763,27.5625
3131,172197.75999999046,27.5625
3132,172220.5799999237,27.5625
3133,172392.19000005722,27.5625
3134,172416.48000001907,27.5625
3135,172439.5799999237,27.5625
3136,172462.9700000286,27.5625
3137,172486.09999990463,27.5625
3138,172509.4700000286,27.5625
3139,172532.09999990463,27.5625
3140,172556.91000008583,27.5625
3141,172580.1399998665,27.5625
3142,172603.61999988556,27.5625
3143,172628.37999987602,27.5625
3144,172652.4700000286,27.5625
3145,172805.03999996185,27.625
3146,172828.93000006676,27.625
3147,172852.0799999237,27.625
3148,172876.19000005722,27.625
3149,172900.09999990463,27.625
3150,172924.04999995232,27.625
3151,172947.19000005722,27.625
3152,172971.39999985695,27.625
3153,172994.36999988556,27.625
3154,173017.49000000954,27.625
3155,173040.53999996185,27.625
3156,173064.26999998093,27.625
3157,173088.3899998665,27.625
3158,173111.20000004768,27.625
3159,173135.05999994278,27.625
3160,173307.36999988556,27.6875
3161,173330.39999985695,27.6875
3162,173353.75999999046,27.6875
3163,173378.25,27.6875
3164,173401.44000005722,27.6875
3165,173425.41000008583,27.6875
3166,173449.79999995232,27.6875
3167,173473.20000004768,27.6875
3168,173497.3899998665,27.6875
3169,173521.43000006676,27.6875
3170,173544.16000008583,27.625
3171,173568.0799999237,27.6875
3172,173592.1099998951,27.6875
3173,173615.6700000763,27.6875
3174,173786.68000006676,27.6875
3175,173811.34999990463,27.6875
3176,173834.75999999046,27.6875
3177,173857.39999985695,27.75
3178,173880.2200000286,27.6875
3179,173903.2200000286,27.6875
3180,173926.01999998093,27.6875
3181,173950.48000001907,27.6875
3182,173973.00999999046,27.6875
3183,173996.03999996185,27.6875
3184,174018.86999988556,27.75
3185,174042.74000000954,27.6875
3186,174066.24000000954,27.75
3187,174089.75999999046,27.75
3188,174113.41000008583,27.75
3189,174136.7799999714,27.75
3190,174161.00999999046,27.75
3191,174184.75999999046,27.75
3192,174356.3599998951,27.75
3193,174426.87999987602,27.75
3194,174450.03999996185,27.75
3195,174473.59999990463,27.75
3196,174544.44000005722,27.75
3197,174567.5799999237,27.75
3198,174591.91000008583,27.8125
3199,174616.5799999237,27.75
3200,174639.29999995232,27.75
3201,174662.95000004768,27.8125
3202,174685.96000003815,27.8125
3203,174709.94000005722,27.8125
3204,174851.8899998665,27.8125
3205,174875.1099998951,27.8125
3206,174897.86999988556,27.8125
3207,174920.95000004768,27.8125
3208,174944.16000008583,27.8125
3209,174967.9200000763,27.8125
3210,174990.64999985695,27.8125
3211,175014.19000005722,27.8125
3212,175037.8899998665,27.8125
3213,175060.58999991417,27.875
3214,175084.53999996185,27.8125
3215,175108.6399998665,27.8125
3216,175132.83999991417,27.8125
3217,175156.9200000763,27.8125
3218,175180.9200000763,27.8125
3219,175204.53999996185,27.8125
3220,175345.8299999237,27.875
3221,175369.80999994278,27.8125
3222,175393.83999991417,27.875
3223,175417.9700000286,27.875
3224,175440.7200000286,27.875
3225,175463.54999995232,27.875
3226,175487.66000008583,27.875
3227,175511.18000006676,27.875
3228,175534.76999998093,27.875
3229,175559.00999999046,27.875
3230,175582.48000001907,27.875
3231,175605.7799999714,27.875
3232,175629.59999990463,27.875
3233,175861.74000000954,27.875
3234,175884.2200000286,27.875
3235,175907.05999994278,27.9375
3236,175931.70000004768,27.875
3237,175954.86999988556,27.875
3238,175978.8299999237,27.9375
3239,176003.34999990463,27.875
3240,176026.30999994278,27.9375
3241,176049.34999990463,27.9375
3242,176073.19000005722,27.9375
3243,176096.54999995232,27.9375
3244,176120.44000005722,27.9375
3245,176143.21000003815,27.9375
3246,176166.75999999046,27.9375
3247,176190.14999985695,27.9375
3248,176213.8599998951,27.9375
3249,176237.45000004768,27.9375
3250,176261.33999991417,27.9375
3251,176285.36999988556,27.9375
3252,176308.41000008583,27.9375
3253,176331.49000000954,27.9375
3254,176354.9200000763,27.9375
3255,176377.79999995232,27.9375
3256,176400.8299999237,27.9375
3257,176423.8599998951,27.9375
3258,176448.30999994278,27.9375
3259,176471.96000003815,27.9375
3260,176496.4700000286,27.9375
3261,176521.25999999046,27.9375
3262,176546.1099998951,27.9375
3263,176569.75999999046,27.9375
3264,176741.58999991417,27.9375
3265,176764.5799999237,27.9375
3266,176809.9200000763,28.0
3267,176833.64999985695,28.0
3268,176857.2799999714,28.0
3269,176880.34999990463,27.9375
3270,176904.20000004768,28.0
3271,176927.0,28.0
3272,176951.45000004768,28.0
3273,176975.0299999714,28.0
3274,176998.96000003815,28.0
3275,177022.11999988556,28.0
3276,177046.50999999046,28.0
3277,177070.0,28.0
3278,177094.24000000954,28.0
3279,177117.4200000763,28.0
3280,177288.8299999237,28.0
3281,177311.81999993324,28.0
3282,177336.31999993324,28.0
3283,177359.53999996185,28.0
3284,177382.39999985695,28.0
3285,177405.5299999714,28.0625
3286,177428.78999996185,28.0
3287,177452.59999990463,28.0
3288,177476.59999990463,28.0
3289,177500.4200000763,28.0625
3290,177522.9200000763,28.0625
3291,177546.84999990463,28.0625
3292,177570.6399998665,28.0
3293,177682.24000000954,28.0
3294,177705.44000005722,28.0625
3295,177728.99000000954,28.0
3296,177753.7200000286,28.0625
3297,177776.36999988556,28.0625
3298,177800.69000005722,28.0625
3299,177824.59999990463,28.0625
3300,177848.45000004768,28.0625
3301,177871.9700000286,28.0625
3302,177895.46000003815,28.0625
3303,177920.54999995232,28.0625
3304,177944.44000005722,28.0625
3305,177967.98000001907,28.0625
3306,177992.00999999046,28.0625
3307,178015.56999993324,28.0625
3308,178157.16000008583,28.125
3309,178181.25,28.0625
3310,178203.79999995232,28.0625
3311,178226.98000001907,28.0625
3312,178250.83999991417,28.0625
3313,178274.76999998093,28.0625
3314,178298.6099998951,28.0625
3315,178321.83999991417,28.0625
3316,178344.80999994278,28.0625
3317,178368.89999985695,28.125
3318,178392.49000000954,28.0625
3319,178415.12999987602,28.0625
3320,178438.19000005722,28.125
3321,178462.7200000286,28.0625
3322,178486.08999991417,28.0625
3323,178510.1700000763,28.0625
3324,178651.26999998093,28.125
3325,178674.26999998093,28.125
3326,178699.25,28.125
3327,178721.83999991417,28.125
3328,178745.78999996185,28.125
3329,178770.1700000763,28.125
3330,178793.66000008583,28.125
3331,178816.31999993324,28.125
3332,178840.19000005722,28.125
3333,178864.20000004768,28.125
3334,178888.23000001907,28.125
3335,178911.53999996185,28.125
3336,178935.71000003815,28.125
3337,178959.44000005722,28.125
3338,178982.33999991417,28.125
3339,179005.18000006676,28.125
3340,179029.05999994278,28.125
3341,179140.3899998665,28.125
3342,179164.3899998665,28.1875
3343,179187.96000003815,28.1875
3344,179211.34999990463,28.1875
3345,179234.51999998093,28.125
3346,179258.45000004768,28.1875
3347,179281.20000004768,28.1875
3348,179304.4700000286,28.125
3349,179328.28999996185,28.125
3350,179351.86999988556,28.125
3351,179376.0,28.1875
3352,179399.59999990463,28.1875
3353,179423.8599998951,28.1875
3354,179446.37999987602,28.1875
3355,179469.70000004768,28.1875
3356,179493.5799999237,28.125
3357,179517.25,28.125
3358,179540.91000008583,28.1875
3359,179563.5799999237,28.1875
3360,179588.03999996185,28.1875
3361,179611.39999985695,28.1875
3362,179636.0,28.1875
3363,179659.89999985695,28.1875
3364,179682.99000000954,28.1875
3365,179707.6399998665,28.1875
3366,179732.4200000763,28.1875
3367,179755.98000001907,28.1875
3368,179779.1700000763,28.1875
3369,179802.73000001907,28.1875
3370,179827.04999995232,28.1875
3371,179850.78999996185,28.1875
3372,179985.36999988556,28.1875
3373,180008.6399998665,28.1875
3374,180032.89999985695,28.1875
3375,180056.08999991417,28.1875
3376,180079.76999998093,28.1875
3377,180103.03999996185,28.1875
3378,180125.64999985695,28.1875
3379,180149.64999985695,28.1875
3380,180173.04999995232,28.1875
3381,180197.4200000763,28.1875
3382,180221.24000000954,28.1875
3383,180244.4700000286,28.1875
3384,180267.1700000763,28.1875
3385,180290.19000005722,28.1875
3386,180430.6099998951,28.1875
3387,180454.5799999237,28.25
3388,180477.20000004768,28.1875
3389,180500.8599998951,28.25
3390,180524.89999985695,28.25
3391,180547.7799999714,28.25
3392,180571.6399998665,28.1875
3393,180594.89999985695,28.25
3394,180617.9200000763,28.25
3395,180642.11999988556,28.25
3396,180666.8599998951,28.25
3397,180689.51999998093,28.25
3398,180713.09999990463,28.25
3399,180735.99000000954,28.25
3400,180783.7799999714,28.25
3401,180807.03999996185,28.25
3402,180831.12999987602,28.25
3403,180855.29999995232,28.25
3404,180878.00999999046,28.25
3405,181019.5299999714,28.25
3406,181043.4700000286,28.25
3407,181066.6700000763,28.25
3408,181090.9700000286,28.25
3409,181114.43000006676,28.25
3410,181137.31999993324,28.25
3411,181160.54999995232,28.25
3412,181184.66000008583,28.25
3413,181207.91000008583,28.25
3414,181230.81999993324,28.25
3415,181255.2200000286,28.25
3416,181280.11999988556,28.25
3417,181304.09999990463,28.3125
3418,181327.54999995232,28.25
3419,181350.59999990463,28.3125
3420,181462.06999993324,28.25
3421,181486.71000003815,28.25
3422,181510.5,28.3125
3423,181533.53999996185,28.25
3424,181558.30999994278,28.3125
3425,181582.09999990463,28.25
3426,181605.53999996185,28.3125
3427,181628.37999987602,28.25
3428,181651.31999993324,28.3125
3429,181675.08999991417,28.25
3430,181698.29999995232,28.3125
3431,181721.11999988556,28.3125
3432,181744.25999999046,28.3125
3433,181768.99000000954,28.3125
3434,181793.2200000286,28.3125
3435,181816.96000003815,28.3125
3436,181840.3599998951,28.3125
3437,181951.84999990463,28.3125
3438,181975.23000001907,28.3125
3439,181999.59999990463,28.3125
3440,182023.6700000763,28.3125
3441,182048.2200000286,28.3125
3442,182071.3899998665,28.3125
3443,182094.41000008583,28.3125
3444,182117.0799999237,28.3125
3445,182141.1099998951,28.3125
3446,182165.11999988556,28.3125
3447,182188.39999985695,28.3125
3448,182211.80999994278,28.3125
3449,182234.78999996185,28.3125
3450,182259.00999999046,28.3125
3451,182282.94000005722,28.3125
3452,182393.44000005722,28.3125
3453,182416.53999996185,28.3125
3454,182440.51999998093,28.3125
3455,182464.03999996185,28.3125
3456,182487.14999985695,28.3125
3457,182511.18000006676,28.3125
3458,182534.7799999714,28.3125
3459,182605.71000003815,28.3125
3460,182628.73000001907,28.3125
3461,182653.49000000954,28.3125
3462,182676.8899998665,28.3125
3463,182700.23000001907,28.3125
3464,182722.94000005722,28.3125
3465,182893.8899998665,28.375
3466,182916.91000008583,28.375
3467,182940.8899998665,28.3125
3468,182964.53999996185,28.3125
3469,182987.51999998093,28.375
3470,183011.39999985695,28.375
3471,183035.54999995232,28.375
3472,183059.06999993324,28.375
3473,183081.94000005722,28.375
3474,183105.06999993324,28.375
3475,183128.7200000286,28.375
3476,183152.71000003815,28.375
3477,183175.7200000286,28.375
3478,183199.5799999237,28.3125
3479,183340.61999988556,28.375
3480,183364.26999998093,28.375
3481,183388.6099998951,28.375
3482,183411.1399998665,28.375
3483,183434.04999995232,28.375
3484,183457.2200000286,28.375
3485,183480.04999995232,28.375
3486,183521.01999998093,28.375
3487,183544.0799999237,28.375
3488,183567.24000000954,28.375
3489,183590.86999988556,28.375
3490,183614.69000005722,28.375
3491,183638.75,28.375
3492,183662.41000008583,28.375
3493,183686.4700000286,28.375
3494,183798.3599998951,28.375
3495,183823.25,28.375
3496,183846.6399998665,28.375
3497,183870.1700000763,28.375
3498,183893.98000001907,28.375
3499,183918.51999998093,28.375
3500,183941.50999999046,28.375
3501,183964.43000006676,28.375
3502,183988.19000005722,28.375
3503,184012.01999998093,28.375
3504,184036.64999985695,28.375
3505,184060.83999991417,28.375
3506,184084.18000006676,28.375
3507,184106.7799999714,28.375
3508,184130.91000008583,28.375
3509,184154.75999999046,28.375
3510,184266.0799999237,28.375
3511,184289.54999995232,28.375
3512,184313.30999994278,28.4375
3513,184336.03999996185,28.375
3514,184359.6399998665,28.375
3515,184383.20000004768,28.375
3516,184406.21000003815,28.375
3517,184429.14999985695,28.375
3518,184452.99000000954,28.375
3519,184476.54999995232,28.375
3520,184500.73000001907,28.4375
3521,184524.80999994278,28.375
3522,184547.80999994278,28.375
3523,184570.8599998951,28.375
3524,184682.3899998665,28.4375
3525,184705.86999988556,28.4375
3526,184730.18000006676,28.375
3527,184753.3599998951,28.4375
3528,184777.08999991417,28.4375
3529,184800.56999993324,28.4375
3530,184824.62999987602,28.4375
3531,184849.34999990463,28.4375
3532,184872.58999991417,28.4375
3533,184896.74000000954,28.4375
3534,184919.6399998665,28.4375
3535,185091.1099998951,28.4375
3536,185113.86999988556,28.4375
3537,185138.1399998665,28.4375
3538,185162.21000003815,28.375
3539,185186.19000005722,28.4375
3540,185210.20000004768,28.4375
3541,185233.71000003815,28.4375
3542,185257.41000008583,28.4375
3543,185280.11999988556,28.4375
3544,185304.3599998951,28.4375
3545,185327.54999995232,28.4375
3546,185351.55999994278,28.4375
3547,185375.3599998951,28.4375
3548,185398.71000003815,28.4375
3549,185422.41000008583,28.4375
3550,185445.83999991417,28.4375
3551,185469.25,28.4375
3552,185580.78999996185,28.4375
3553,185604.76999998093,28.4375
3554,185628.76999998093,28.4375
3555,185651.84999990463,28.4375
3556,185675.7799999714,28.4375
3557,185699.66000008583,28.4375
3558,185723.37999987602,28.4375
3559,185747.39999985695,28.4375
3560,185770.41000008583,28.4375
3561,185794.49000000954,28.4375
3562,185818.28999996185,28.4375
3563,185841.7799999714,28.4375
3564,185865.21000003815,28.4375
3565,185888.2799999714,28.4375
3566,185911.48000001907,28.4375
3567,185934.6099998951,28.4375
3568,186046.44000005722,28.4375
3569,186069.80999994278,28.4375
3570,186117.08999991417,28.4375
3571,186140.9700000286,28.4375
3572,186165.20000004768,28.4375
3573,186188.33999991417,28.4375
3574,186212.19000005722,28.4375
3575,186234.94000005722,28.4375
3576,186258.09999990463,28.4375
3577,186282.0799999237,28.4375
3578,186306.45000004768,28.4375
3579,186330.39999985695,28.4375
3580,186353.83999991417,28.4375
3581,186377.73000001907,28.4375
3582,186400.5799999237,28.4375
3583,186510.89999985695,28.4375
3584,186559.09999990463,28.4375
3585,186583.19000005722,28.4375
3586,186630.74000000954,28.4375
3587,186654.16000008583,28.4375
3588,186677.59999990463,28.4375
3589,186700.53999996185,28.4375
3590,186724.12999987602,28.4375
3591,186747.45000004768,28.4375
3592,186771.37999987602,28.5
3593,186794.73000001907,28.5
3594,186819.61999988556,28.4375
3595,186842.98000001907,28.5
3596,186891.1399998665,28.4375
3597,186914.33999991417,28.4375
3598,186937.09999990463,28.4375
3599,187052.00999999046,28.5
3600,187075.01999998093,28.5
3601,187098.43000006676,28.4375
3602,187121.58999991417,28.5
3603,187144.75,28.4375
3604,187167.73000001907,28.4375
3605,187191.70000004768,28.4375
3606,187215.24000000954,28.4375
3607,187238.71000003815,28.4375
3608,187261.6399998665,28.4375
3609,187285.6399998665,28.5
3610,187309.26999998093,28.5
3611,187332.08999991417,28.5
3612,187355.83999991417,28.5
3613,187378.98000001907,28.4375
3614,187402.7799999714,28.5
3615,187425.44000005722,28.4375
3616,187536.21000003815,28.5
3617,187559.68000006676,28.5
3618,187583.76999998093,28.5
3619,187607.80999994278,28.5
3620,187630.44000005722,28.5
3621,187654.00999999046,28.4375
3622,187678.30999994278,28.5
3623,187745.1700000763,28.5
3624,187769.24000000954,28.5
3625,187909.99000000954,28.5
3626,187934.21000003815,28.5
3627,187958.1399998665,28.5
3628,187981.86999988556,28.5
3629,188005.98000001907,28.5
3630,188029.25,28.5
3631,188053.3899998665,28.5
3632,188076.36999988556,28.5
3633,188101.25999999046,28.5
3634,188125.21000003815,28.5
3635,188149.16000008583,28.5
3636,188172.5799999237,28.5
3637,188195.8299999237,28.5
3638,188219.79999995232,28.5
3639,188243.04999995232,28.5
3640,188267.5799999237,28.5
3641,188379.14999985695,28.5
3642,188402.31999993324,28.5
3643,188425.76999998093,28.5
3644,188450.33999991417,28.5
3645,188473.50999999046,28.5
3646,188497.61999988556,28.5
3647,188521.53999996185,28.5
3648,188544.62999987602,28.5
3649,188567.54999995232,28.5
3650,188590.53999996185,28.5
3651,188613.4200000763,28.5
3652,188637.80999994278,28.5
3653,188661.78999996185,28.5
3654,188686.08999991417,28.5
3655,188710.09999990463,28.5
3656,188734.55999994278,28.5
3657,188875.89999985695,28.5
3658,188899.96000003815,28.5
3659,188922.86999988556,28.5
3660,188946.49000000954,28.5
3661,188970.6099998951,28.5
3662,188993.3299999237,28.5
3663,189016.94000005722,28.5
3664,189040.69000005722,28.5
3665,189063.74000000954,28.5
3666,189087.09999990463,28.5
3667,189111.2200000286,28.5
3668,189133.96000003815,28.5
3669,189158.54999995232,28.5
3670,189182.91000008583,28.5
3671,189206.50999999046,28.5
3672,189229.11999988556,28.5
3673,189370.73000001907,28.5
3674,189394.56999993324,28.5
3675,189417.81999993324,28.5
3676,189441.00999999046,28.5
3677,189464.24000000954,28.5
3678,189488.05999994278,28.5
3679,189511.6399998665,28.5
3680,189535.4700000286,28.5
3681,189558.68000006676,28.5
3682,189581.4700000286,28.5
3683,189606.11999988556,28.5
3684,189629.53999996185,28.5
3685,189652.68000006676,28.5
3686,189675.3899998665,28.5
3687,189789.2200000286,28.5
3688,189813.48000001907,28.5
3689,189836.4200000763,28.5
3690,189860.44000005722,28.5625
3691,189883.24000000954,28.5
3692,189906.25999999046,28.5
3693,189929.01999998093,28.5
3694,189953.4700000286,28.5
3695,189998.7200000286,28.5
3696,190022.14999985695,28.5
3697,190045.83999991417,28.5625
3698,190216.56999993324,28.5625
3699,190239.4200000763,28.5
3700,190262.1399998665,28.5
3701,190285.36999988556,28.5
3702,190309.55999994278,28.5
3703,190333.03999996185,28.5625
3704,190355.87999987602,28.5
3705,190379.06999993324,28.5
3706,190402.25999999046,28.5
3707,190426.4200000763,28.5
3708,190449.34999990463,28.5
3709,190473.71000003815,28.5
3710,190497.89999985695,28.5
3711,190520.91000008583,28.5625
3712,190544.87999987602,28.5
3713,190568.78999996185,28.5
3714,190770.45000004768,28.5
3715,190794.14999985695,28.5625
3716,190817.4700000286,28.5
3717,190841.49000000954,28.5625
3718,190865.4200000763,28.5625
3719,190889.46000003815,28.5625
3720,190913.19000005722,28.5625
3721,190936.96000003815,28.5
3722,190960.20000004768,28.5625
3723,190983.03999996185,28.5625
3724,191006.75999999046,28.5625
3725,191029.58999991417,28.5625
3726,191052.23000001907,28.5625
3727,191224.08999991417,28.5625
3728,191247.55999994278,28.5
3729,191270.74000000954,28.5625
3730,191295.0,28.5625
3731,191319.21000003815,28.5
3732,191342.34999990463,28.5625
3733,191365.5,28.5625
3734,191388.43000006676,28.5625
3735,191412.39999985695,28.5
3736,191436.98000001907,28.5
3737,191460.20000004768,28.5625
3738,191484.11999988556,28.5
3739,191507.84999990463,28.5625
3740,191530.46000003815,28.5
3741,191701.14999985695,28.5625
3742,191724.95000004768,28.5625
3743,191748.08999991417,28.5625
3744,191770.94000005722,28.5625
3745,191795.66000008583,28.5625
3746,191818.83999991417,28.5625
3747,191843.44000005722,28.5625
3748,191866.55999994278,28.5625
3749,191889.79999995232,28.5625
3750,191912.98000001907,28.5625
3751,191936.6099998951,28.5625
3752,191960.61999988556,28.5625
3753,191983.01999998093,28.5625
3754,192006.29999995232,28.5625
3755,192030.2200000286,28.5625
3756,192201.99000000954,28.5625
3757,192225.21000003815,28.5625
3758,192249.18000006676,28.5625
3759,192272.75,28.5625
3760,192295.6399998665,28.5625
3761,192319.5,28.5625
3762,192343.4700000286,28.5625
3763,192366.8599998951,28.5625
3764,192390.25999999046,28.5625
3765,192414.18000006676,28.5625
3766,192438.6399998665,28.5625
3767,192461.95000004768,28.5625
3768,192484.7200000286,28.5625
3769,192507.54999995232,28.5625
3770,192530.55999994278,28.5625
3771,192553.69000005722,28.5625
3772,192577.14999985695,28.5625
3773,192600.37999987602,28.5625
3774,192712.45000004768,28.5625
3775,192735.79999995232,28.5625
3776,192760.0,28.5625
3777,192783.91000008583,28.5625
3778,192807.0799999237,28.5625
3779,192830.8599998951,28.5625
3780,192853.73000001907,28.5625
3781,192877.3599998951,28.5625
3782,192900.03999996185,28.5625
3783,192923.28999996185,28.5625
3784,192946.5299999714,28.5625
3785,193057.09999990463,28.5625
3786,193080.44000005722,28.5625
3787,193103.68000006676,28.5625
3788,193127.24000000954,28.5625
3789,193149.81999993324,28.5625
3790,193174.00999999046,28.5625
3791,193221.14999985695,28.5625
3792,193243.86999988556,28.5625
3793,193267.68000006676,28.5625
3794,193292.28999996185,28.5625
3795,193315.4200000763,28.5625
3796,193338.6700000763,28.5625
3797,193362.76999998093,28.5625
3798,193386.03999996185,28.5625
3799,193409.9700000286,28.5625
3800,193432.75,28.5625
3801,193573.12999987602,28.5625
3802,193596.11999988556,28.5625
3803,193620.36999988556,28.5625
3804,193643.4200000763,28.5625
3805,193667.46000003815,28.5625
3806,193691.16000008583,28.5625
3807,193714.70000004768,28.5625
3808,193737.58999991417,28.5625
3809,193761.1399998665,28.5625
3810,193785.24000000954,28.5625
3811,193810.3599998951,28.5625
3812,193833.19000005722,28.5625
3813,193857.37999987602,28.5625
3814,193880.49000000954,28.5625
3815,193904.24000000954,28.5625
3816,193928.26999998093,28.5625
3817,193951.71000003815,28.5625
3818,194093.19000005722,28.5625
3819,194115.7200000286,28.5625
3820,194138.4700000286,28.5625
3821,194161.46000003815,28.5625
3822,194184.79999995232,28.5625
3823,194207.8599998951,28.5625
3824,194231.83999991417,28.5
3825,194257.66000008583,28.5625
3826,194281.03999996185,28.5625
3827,194303.75,28.5625
3828,194327.03999996185,28.5625
3829,194350.18000006676,28.5625
3830,194373.75,28.5625
3831,194396.68000006676,28.5625
3832,194538.55999994278,28.5625
3833,194561.49000000954,28.5625
3834,194585.3599998951,28.5625
3835,194609.6399998665,28.5625
3836,194633.80999994278,28.5625
3837,194657.99000000954,28.5625
3838,194681.8599998951,28.5625
3839,194705.54999995232,28.5625
3840,194728.28999996185,28.5625
3841,194751.71000003815,28.5625
3842,194775.50999999046,28.5625
3843,194799.16000008583,28.5625
3844,194822.69000005722,28.5625
3845,194933.44000005722,28.5625
3846,194956.80999994278,28.5625
3847,194980.14999985695,28.5625
3848,195003.94000005722,28.5625
3849,195026.51999998093,28.5625
3850,195050.45000004768,28.5625
3851,195073.18000006676,28.5625
3852,195096.26999998093,28.5625
3853,195119.74000000954,28.5
3854,195142.58999991417,28.5625
3855,195167.66000008583,28.5625
3856,195191.48000001907,28.5625
3857,195214.1399998665,28.5625
3858,195385.6099998951,28.5625
3859,195409.75999999046,28.5625
3860,195432.9200000763,28.5625
3861,195457.2799999714,28.5625
3862,195480.30999994278,28.5625
3863,195504.31999993324,28.5625
3864,195527.9700000286,28.5625
3865,195551.5,28.5625
3866,195575.25999999046,28.5625
3867,195599.2799999714,28.5625
3868,195623.24000000954,28.5625
3869,195645.99000000954,28.5625
3870,195668.9200000763,28.5625
3871,195692.14999985695,28.5625
3872,195832.50999999046,28.5625
3873,195856.7200000286,28.5625
3874,195880.74000000954,28.5625
3875,195903.94000005722,28.5625
3876,195928.24000000954,28.5625
3877,195952.21000003815,28.5625
3878,195975.18000006676,28.5625
3879,195998.61999988556,28.5625
3880,196022.30999994278,28.5625
3881,196045.70000004768,28.5625
3882,196069.0299999714,28.5625
3883,196091.79999995232,28.5625
3884,196115.26999998093,28.5625
3885,196138.81999993324,28.5625
3886,196161.99000000954,28.5625
3887,196304.16000008583,28.5625
3888,196327.66000008583,28.5625
3889,196350.86999988556,28.5625
3890,196374.09999990463,28.5625
3891,196397.58999991417,28.5625
3892,196421.25,28.5625
3893,196444.31999993324,28.5625
3894,196467.6399998665,28.5625
3895,196490.3899998665,28.5625
3896,196513.4700000286,28.5625
3897,196537.29999995232,28.5625
3898,196560.55999994278,28.5625
3899,196583.61999988556,28.5625
3900,196725.1099998951,28.5625
3901,196748.75999999046,28.5625
3902,196772.76999998093,28.5625
3903,196795.99000000954,28.5625
3904,196818.89999985695,28.5625
3905,196841.48000001907,28.5625
3906,196864.3899998665,28.5625
3907,196887.26999998093,28.5625
3908,196910.36999988556,28.5625
3909,196934.59999990463,28.5625
3910,196957.1399998665,28.5625
3911,196981.0799999237,28.5625
3912,197005.55999994278,28.5625
3913,197029.1099998951,28.5625
3914,197053.1099998951,28.5625
3915,197075.9200000763,28.5625
3916,197306.6099998951,28.5625
3917,197329.73000001907,28.5625
3918,197354.53999996185,28.5625
3919,197377.84999990463,28.5625
3920,197401.43000006676,28.5625
3921,197425.29999995232,28.5625
3922,197448.03999996185,28.5625
3923,197471.70000004768,28.5625
3924,197495.79999995232,28.5625
3925,197519.01999998093,28.5625
3926,197542.41000008583,28.5625
3927,197565.68000006676,28.5625
3928,197588.59999990463,28.5625
3929,197612.83999991417,28.5625
3930,197637.39999985695,28.5625
3931,197778.87999987602,28.5625
3932,197801.80999994278,28.5625
3933,197825.44000005722,28.5625
3934,197848.64999985695,28.5625
3935,197872.68000006676,28.5625
3936,197901.16000008583,28.5625
3937,197924.24000000954,28.5625
3938,197947.83999991417,28.5625
3939,197971.91000008583,28.5625
3940,197995.3599998951,28.5625
3941,198018.41000008583,28.5625
3942,198041.3599998951,28.5625
3943,198064.20000004768,28.5625
3944,198087.1700000763,28.5625
3945,198289.45000004768,28.5625
3946,198313.11999988556,28.5625
3947,198337.33999991417,28.5625
3948,198360.12999987602,28.5625
3949,198383.0,28.5625
3950,198406.48000001907,28.5625
3951,198429.94000005722,28.5625
3952,198452.73000001907,28.5625
3953,198476.81999993324,28.5625
3954,198500.83999991417,28.5625
3955,198525.31999993324,28.5625
3956,198666.78999996185,28.5625
3957,198691.0,28.5625
3958,198735.98000001907,28.5625
3959,198759.25,28.5625
3960,198783.53999996185,28.5625
3961,198806.6399998665,28.5625
3962,198829.81999993324,28.5625
3963,198852.54999995232,28.5625
3964,198876.44000005722,28.5625
3965,198899.95000004768,28.5625
3966,198923.76999998093,28.5625
3967,198970.58999991417,28.5625
3968,198993.6099998951,28.5625
3969,199194.49000000954,28.5625
3970,199218.55999994278,28.5625
3971,199242.54999995232,28.5625
3972,199266.25,28.5625
3973,199288.9700000286,28.5625
3974,199312.75,28.5625
3975,199336.31999993324,28.5625
3976,199359.05999994278,28.5625
3977,199383.05999994278,28.5625
3978,199406.14999985695,28.5625
3979,199430.08999991417,28.5625
3980,199453.43000006676,28.5625
3981,199478.0299999714,28.5625
3982,199502.08999991417,28.5625
3983,199526.24000000954,28.5625
3984,199549.4200000763,28.5625
3985,199572.51999998093,28.5625
3986,199727.8299999237,28.5625
3987,199751.4200000763,28.5625
3988,199774.69000005722,28.5625
3989,199798.25,28.5625
3990,199821.44000005722,28.5625
3991,199844.86999988556,28.5625
3992,199869.0,28.5625
3993,199892.78999996185,28.5625
3994,199916.89999985695,28.5625
3995,199940.39999985695,28.5625
3996,199963.8899998665,28.5625
3997,199988.0299999714,28.5625
3998,200011.87999987602,28.5625
3999,200058.68000006676,28.5625
4000,200081.76999998093,28.5625
4001,200104.5299999714,28.5625
4002,200128.37999987602,28.5625
4003,200151.81999993324,28.5625
4004,200412.44000005722,28.5625
4005,200435.33999991417,28.5625
4006,200458.3599998951,28.5625
4007,200481.51999998093,28.5625
4008,200505.14999985695,28.5625
4009,200528.0,28.5625
4010,200551.16000008583,28.5625
4011,200575.06999993324,28.5625
4012,200598.06999993324,28.5625
4013,200622.2200000286,28.5625
4014,200645.91000008583,28.5625
4015,200670.09999990463,28.5625
4016,200693.8599998951,28.5625
4017,200717.62999987602,28.5625
4018,200919.6099998951,28.5625
4019,200942.95000004768,28.5625
4020,200965.84999990463,28.5625
4021,200989.1700000763,28.5625
4022,201012.96000003815,28.5625
4023,201036.29999995232,28.5625
4024,201060.03999996185,28.5625
4025,201083.03999996185,28.5625
4026,201107.09999990463,28.5625
4027,201131.14999985695,28.5625
4028,201154.14999985695,28.5625
4029,201178.24000000954,28.5625
4030,201202.8299999237,28.5625
4031,201225.84999990463,28.5625
4032,201250.12999987602,28.5625
4033,201273.29999995232,28.5625
4034,201414.1099998951,28.5625
4035,201437.14999985695,28.5625
4036,201460.69000005722,28.5625
4037,201483.87999987602,28.5625
4038,201506.74000000954,28.5625
4039,201530.83999991417,28.5625
4040,201553.59999990463,28.5625
4041,201576.87999987602,28.5625
4042,201599.69000005722,28.5625
4043,201624.18000006676,28.5625
4044,201647.41000008583,28.5625
4045,201670.9200000763,28.5
4046,201693.94000005722,28.5
4047,201717.41000008583,28.5625
4048,201740.1399998665,28.5
4049,201763.2799999714,28.5625
4050,201787.1099998951,28.5
4051,201929.26999998093,28.5625
4052,201952.4200000763,28.5
4053,201976.16000008583,28.5625
4054,201998.87999987602,28.5625
4055,202021.53999996185,28.5625
4056,202044.2799999714,28.5625
4057,202066.8899998665,28.5625
4058,202090.53999996185,28.5
4059,202133.8599998951,28.5
4060,202158.1399998665,28.5
4061,202181.11999988556,28.5625
4062,202204.94000005722,28.5
4063,202228.78999996185,28.5625
4064,202252.19000005722,28.5625
4065,202275.64999985695,28.5625
4066,202299.74000000954,28.5625
4067,202410.6700000763,28.5625
4068,202436.74000000954,28.5625
4069,202460.53999996185,28.5
4070,202484.37999987602,28.5625
4071,202508.41000008583,28.5625
4072,202533.14999985695,28.5
4073,202557.31999993324,28.5
4074,202581.24000000954,28.5
4075,202604.74000000954,28.5
4076,202628.75999999046,28.5
4077,202651.83999991417,28.5625
4078,202674.50999999046,28.5625
4079,202698.8599998951,28.5
4080,202722.83999991417,28.5
4081,202746.6700000763,28.5
4082,202769.55999994278,28.5
4083,202793.36999988556,28.5625
4084,202963.69000005722,28.5625
4085,202986.94000005722,28.5
4086,203010.76999998093,28.5625
4087,203034.04999995232,28.5
4088,203057.48000001907,28.5
4089,203081.54999995232,28.5
4090,203105.48000001907,28.5
4091,203129.09999990463,28.5625
4092,203151.86999988556,28.5625
4093,203175.01999998093,28.5
4094,203199.7200000286,28.5
4095,203222.74000000954,28.5
4096,203246.7200000286,28.5
4097,203269.34999990463,28.5
4098,203293.54999995232,28.5
4099,203316.3899998665,28.5
4100,203427.98000001907,28.5
4101,203451.87999987602,28.5
4102,203474.5799999237,28.5
4103,203499.09999990463,28.5
4104,203521.6399998665,28.5
4105,203545.8599998951,28.5625
4106,203569.37999987602,28.5
4107,203639.50999999046,28.5
4108,203662.14999985695,28.5
4109,203685.76999998093,28.5
4110,203708.93000006676,28.5
4111,203732.04999995232,28.5
4112,203872.3899998665,28.5
4113,203895.3299999237,28.5
4114,203918.2200000286,28.5
4115,203941.0799999237,28.5
4116,203965.26999998093,28.5
4117,203988.39999985695,28.5
4118,204011.51999998093,28.5625
4119,204035.53999996185,28.5
4120,204058.31999993324,28.5
4121,204081.8599998951,28.5
4122,204104.6399998665,28.5
4123,204129.11999988556,28.5
4124,204361.34999990463,28.5625
4125,204384.45000004768,28.5625
4126,204408.20000004768,28.5
4127,204432.84999990463,28.5
4128,204457.36999988556,28.5
4129,204481.08999991417,28.5
4130,204503.78999996185,28.5
4131,204526.75,28.5
4132,204550.51999998093,28.5
4133,204574.8599998951,28.5
4134,204598.6099998951,28.5
4135,204622.91000008583,28.5
4136,204646.08999991417,28.5
4137,204757.4700000286,28.5
4138,204781.19000005722,28.5
4139,204805.7799999714,28.5
4140,204829.50999999046,28.5
4141,204853.41000008583,28.5
4142,204876.44000005722,28.5
4143,204899.34999990463,28.5
4144,204922.25999999046,28.5
4145,204945.75,28.5
4146,204969.3899998665,28.5
4147,204993.75,28.5
4148,205016.46000003815,28.5
4149,205040.23000001907,28.5
4150,205063.89999985695,28.5
4151,205086.55999994278,28.5
4152,205199.1700000763,28.5
4153,205223.2799999714,28.5
4154,205247.05999994278,28.5
4155,205270.34999990463,28.5
4156,205293.31999993324,28.5
4157,205316.95000004768,28.5
4158,205339.74000000954,28.5
4159,205362.8899998665,28.4375
4160,205386.1700000763,28.5
4161,205542.8599998951,28.5
4162,205567.41000008583,28.5
4163,205590.75999999046,28.5
4164,205613.95000004768,28.5
4165,205637.39999985695,28.5
4166,205660.6700000763,28.5
4167,205684.2200000286,28.5
4168,205707.58999991417,28.5
4169,205731.75999999046,28.5
4170,205755.16000008583,28.5
4171,205779.53999996185,28.5
4172,205802.75999999046,28.5
4173,205826.49000000954,28.4375
4174,205850.0,28.4375
4175,205990.29999995232,28.5
4176,206013.1399998665,28.5
4177,206036.4700000286,28.5
4178,206060.44000005722,28.5
4179,206084.1399998665,28.5
4180,206107.79999995232,28.5
4181,206130.6399998665,28.5
4182,206154.74000000954,28.5
4183,206177.95000004768,28.5
4184,206200.83999991417,28.5
4185,206223.98000001907,28.5
4186,206247.23000001907,28.4375
4187,206270.70000004768,28.5
4188,206472.5,28.5
4189,206495.71000003815,28.5
4190,206519.1399998665,28.5
4191,206542.0,28.5
4192,206566.14999985695,28.5
4193,206589.39999985695,28.5
4194,206613.66000008583,28.4375
4195,206637.6700000763,28.5
4196,206660.91000008583,28.4375
4197,206684.9200000763,28.4375
4198,206707.9700000286,28.4375
4199,206731.51999998093,28.4375
4200,206754.66000008583,28.4375
4201,206778.29999995232,28.4375
4202,206801.18000006676,28.4375
4203,206824.24000000954,28.4375
4204,206848.9700000286,28.4375
4205,206872.5299999714,28.4375
4206,206982.6700000763,28.4375
4207,207006.95000004768,28.4375
4208,207030.0799999237,28.4375
4209,207053.37999987602,28.5
4210,207076.75,28.4375
4211,207101.44000005722,28.4375
4212,207124.66000008583,28.4375
4213,207147.8899998665,28.4375
4214,207172.14999985695,28.4375
4215,207195.91000008583,28.4375
4216,207218.69000005722,28.4375
4217,207242.80999994278,28.4375
4218,207265.56999993324,28.4375
4219,207289.26999998093,28.4375
4220,207400.04999995232,28.4375
4221,207423.41000008583,28.4375
4222,207446.96000003815,28.4375
4223,207493.91000008583,28.4375
4224,207517.6700000763,28.4375
4225,207541.45000004768,28.4375
4226,207564.26999998093,28.4375
4227,207588.1700000763,28.4375
4228,207633.89999985695,28.4375
4229,207657.98000001907,28.4375
4230,207681.0,28.4375
4231,207704.1399998665,28.4375
4232,207815.14999985695,28.4375
4233,207838.31999993324,28.4375
4234,207860.98000001907,28.4375
4235,207884.51999998093,28.4375
4236,208009.41000008583,28.4375
4237,208033.51999998093,28.4375
4238,208056.16000008583,28.4375
4239,208079.25999999046,28.375
4240,208102.0299999714,28.4375
4241,208126.05999994278,28.4375
4242,208148.61999988556,28.4375
4243,208290.4700000286,28.4375
4244,208313.5299999714,28.4375
4245,208336.24000000954,28.4375
4246,208359.2200000286,28.4375
4247,208382.7799999714,28.4375
4248,208405.58999991417,28.4375
4249,208428.55999994278,28.4375
4250,208452.48000001907,28.4375
4251,208475.99000000954,28.4375
4252,208499.66000008583,28.4375
4253,208523.49000000954,28.4375
4254,208547.4200000763,28.4375
4255,208570.28999996185,28.4375
4256,208594.41000008583,28.4375
4257,208618.31999993324,28.4375
4258,208641.33999991417,28.4375
4259,208664.3299999237,28.4375
4260,208687.70000004768,28.4375
4261,208710.87999987602,28.4375
4262,208914.00999999046,28.4375
4263,208937.8599998951,28.4375
4264,208960.96000003815,28.4375
4265,208984.48000001907,28.4375
4266,209007.1399998665,28.4375
4267,209030.75999999046,28.4375
4268,209054.75,28.4375
4269,209078.7799999714,28.4375
4270,209102.5799999237,28.4375
4271,209125.48000001907,28.4375
4272,209148.73000001907,28.4375
4273,209172.24000000954,28.4375
4274,209195.50999999046,28.4375
4275,209219.4200000763,28.4375
4276,209243.26999998093,28.4375
4277,209354.8599998951,28.4375
4278,209378.86999988556,28.4375
4279,209402.95000004768,28.4375
4280,209426.14999985695,28.4375
4281,209448.76999998093,28.4375
4282,209471.9700000286,28.4375
4283,209495.14999985695,28.4375
4284,209539.19000005722,28.4375
4285,209562.19000005722,28.4375
4286,209603.64999985695,28.4375
4287,209626.69000005722,28.4375
4288,209650.6700000763,28.4375
4289,209673.41000008583,28.4375
4290,209784.37999987602,28.4375
4291,209807.25,28.4375
4292,209831.74000000954,28.4375
4293,209855.93000006676,28.4375
4294,209902.19000005722,28.375
4295,209925.1099998951,28.375
4296,209948.9700000286,28.4375
4297,209973.14999985695,28.375
4298,209997.3599998951,28.375
4299,210021.54999995232,28.4375
4300,210045.0799999237,28.375
4301,210067.6099998951,28.375
4302,210090.6700000763,28.375
4303,210113.44000005722,28.375
4304,210284.3599998951,28.4375
4305,210308.5799999237,28.375
4306,210332.64999985695,28.375
4307,210376.7200000286,28.375
4308,210400.71000003815,28.375
4309,210423.99000000954,28.375
4310,210447.61999988556,28.375
4311,210471.58999991417,28.375
4312,210495.26999998093,28.375
4313,210518.4200000763,28.375
4314,210541.6700000763,28.375
4315,210713.11999988556,28.375
4316,210736.70000004768,28.375
4317,210760.84999990463,28.375
4318,210783.70000004768,28.375
4319,210807.28999996185,28.375
4320,210831.25999999046,28.375
4321,210878.33999991417,28.375
4322,210902.24000000954,28.375
4323,210926.31999993324,28.375
4324,210950.3599998951,28.375
4325,210973.8299999237,28.3125
4326,210998.25999999046,28.375
4327,211021.69000005722,28.375
4328,211045.8599998951,28.375
4329,211216.4700000286,28.375
4330,211239.50999999046,28.375
4331,211262.58999991417,28.375
4332,211286.8299999237,28.375
4333,211310.1700000763,28.375
4334,211334.37999987602,28.375
4335,211357.04999995232,28.375
4336,211380.3899998665,28.375
4337,211404.3599998951,28.375
4338,211427.99000000954,28.3125
4339,211451.86999988556,28.375
4340,211475.4700000286,28.375
4341,211498.62999987602,28.3125
4342,211521.58999991417,28.375
4343,211544.3599998951,28.3125
4344,211655.2200000286,28.3125
4345,211678.99000000954,28.375
4346,211726.45000004768,28.3125
4347,211750.25999999046,28.375
4348,211774.19000005722,28.375
4349,211797.66000008583,28.375
4350,211821.93000006676,28.375
4351,211845.2799999714,28.375
4352,211869.29999995232,28.375
4353,211891.95000004768,28.375
4354,212093.6700000763,28.3125
4355,212116.58999991417,28.375
4356,212140.55999994278,28.3125
4357,212164.3599998951,28.375
4358,212189.00999999046,28.3125
4359,212212.91000008583,28.3125
4360,212259.96000003815,28.3125
4361,212282.62999987602,28.3125
4362,212306.6399998665,28.3125
4363,212329.7200000286,28.3125
4364,212353.11999988556,28.3125
4365,212376.06999993324,28.3125
4366,212398.9700000286,28.3125
4367,212422.21000003815,28.3125
4368,212445.75999999046,28.3125
4369,212468.89999985695,28.3125
4370,212492.78999996185,28.3125
4371,212723.26999998093,28.3125
4372,212747.1700000763,28.3125
4373,212771.03999996185,28.3125
4374,212794.9200000763,28.3125
4375,212817.73000001907,28.3125
4376,212864.6399998665,28.3125
4377,212888.91000008583,28.3125
4378,212912.1399998665,28.3125
4379,212936.44000005722,28.3125
4380,212959.64999985695,28.3125


==> data_p1_analysis.tex <==
timestamp,time_in_seconds,time_label,T1,T9,x,y,z,err_x,err_y,err_z,rolling_err_mean_x,rolling_err_mean_y,rolling_err_mean_z,corected_err_x,corected_err_y,corected_err_z
2024-12-18 17:28:42.220385,0.0,17:28,22.9375,21.125,-329724.50623859145,-831484.772256477,1684307.721419323,-3.830512527085375,15.604227864881977,-13.787337879650295,2.0628106091118585,8.118435451993719,-11.286400506505743,-329726.56904920057,-831492.890691929,1684319.0078198295
2024-12-18 17:33:31.480385,289.26,17:33,22.9375,21.125,-329718.20327554643,-831491.6057125076,1684297.4271414767,2.4724505179328844,8.770771834300831,-24.081615725997835,2.7376781279211477,7.585454659332754,-10.655236119113397,-329720.9409536744,-831499.1911671669,1684308.0823775958
2024-12-18 17:40:06.490385,684.27,17:40,23.0,21.1875,-329719.99958373106,-831490.3348921518,1684309.5171795732,0.6761423333082348,10.041592190158553,-11.99157762946561,2.2151010919881697,7.428792336149714,-10.797103225432624,-329722.21468482306,-831497.7636844879,1684320.3142827987
2024-12-18 17:44:44.840385,962.62,17:44,23.0625,21.1875,-329720.0572136605,-831499.9209137289,1684303.9061000855,0.6185124038602225,0.45557061303406954,-17.60265711718239,2.0434168930265253,7.500358718289395,-10.584734979784116,-329722.10063055356,-831507.4212724472,1684314.4908350653
2024-12-18 17:50:00.580385,1278.36,17:50,23.0625,21.1875,-329722.52475362766,-831491.4546453201,1684300.801285233,-1.8490275632939301,8.92183902184479,-20.707471969537437,1.873913815745618,7.325852838259501,-9.607547848857939,-329724.3986674434,-831498.7804981583,1684310.408833082
2024-12-18 17:59:04.990385,1822.77,17:59,23.125,21.1875,-329716.27896004746,-831487.6510008192,1684319.7196047783,4.396766016900074,12.725483522750437,-1.7891524243168533,1.784468607580493,6.865257364428544,-9.468541822017869,-329718.06342865503,-831494.5162581836,1684329.1881466003
2024-12-18 18:04:45.660385,2163.44,18:04,23.125,21.25,-329712.1750063639,-831491.588578674,1684316.3875853117,8.500719700474292,8.78790566790849,-5.121171890990809,1.6277422357884728,6.556967210462865,-9.370991851340102,-329713.8027485997,-831498.1455458845,1684325.758577163
2024-12-18 18:09:11.200385,2428.98,18:09,23.125,21.25,-329720.1344527147,-831494.9860547812,1684313.2938657876,0.5412733496632427,5.390429560677148,-8.214891415089369,1.5750819583513982,6.819783075770829,-8.628161130460082,-329721.7095346731,-831501.8058378571,1684321.922026918
2024-12-18 18:14:15.040385,2732.82,18:14,23.1875,21.25,-329719.4195710285,-831496.6641352791,1684312.4061917486,1.2561550358659588,3.7123490627855062,-9.102565454086289,1.5774026125834912,6.6272063279328375,-8.483477750633794,-329720.9969736411,-831503.2913416071,1684320.8896694991
2024-12-18 18:19:05.530385,3023.31,18:19,23.1875,21.25,-329714.96622255904,-831489.4559096108,1684316.8882494632,5.709503505320754,10.920574731077068,-4.62050773948431,1.4874808354623383,6.135285242774989,-8.46382559200283,-329716.4537033945,-831495.5911948537,1684325.3520750552
2024-12-18 18:24:31.850385,3349.63,18:24,23.25,21.25,-329716.4767921371,-831496.4044384394,1684314.377300877,4.198933927284088,3.9720459025120363,-7.131456325761974,1.4436434666249192,5.884282314606632,-7.860531693080529,-329717.9204356037,-831502.288720754,1684322.23783257
2024-12-18 18:29:22.100385,3639.88,18:29,23.25,21.25,-329710.51450522954,-831498.6538184019,1684317.7963293449,10.161220834823325,1.722665940062143,-3.712427857797593,1.7389137031000463,5.316906067714583,-7.104280591210617,-329712.25341893267,-831503.9707244695,1684324.900609936
2024-12-18 18:34:00.630385,3918.41,18:34,23.3125,21.3125,-329724.7315494036,-831494.827639884,1684309.0092487014,-4.0558233392075635,5.548844457953237,-12.499508501263335,1.2702506275603636,5.235564873675772,-6.3588434074162725,-329726.0018000311,-831500.0632047576,1684315.3680921088
2024-12-18 18:39:16.890385,4234.67,18:39,23.3125,21.3125,-329720.86420375784,-831491.9457626558,1684313.6848094163,-0.18847769347485155,8.430721686105244,-7.8239477863535285,1.8436755737056956,4.569823444698981,-5.608441299248842,-329722.70787933154,-831496.5155861005,1684319.2932507156
2024-12-18 18:45:39.460385,4617.24,18:45,23.3125,21.3125,-329721.17485533055,-831495.4937138241,1684325.5818291868,-0.499129266187083,4.8827705178409815,4.073071984108537,1.7449310029734901,4.467250518805702,-4.608180327085956,-329722.9197863335,-831499.9609643429,1684330.1900095139
2024-12-18 18:50:05.110385,4882.89,18:50,23.375,21.3125,-329720.23293557926,-831500.420159085,1684314.1253057832,0.44279048510361463,-0.043674743035808206,-7.383451419416815,1.6783937238145707,4.497632525550823,-3.4375750881375833,-329721.91132930305,-831504.9177916105,1684317.5628808714
2024-12-18 18:54:30.560385,5148.34,18:54,23.375,21.375,-329721.55560577725,-831498.7521595949,1684313.6985648822,-0.8798797128838487,1.6243247470119968,-7.810192320495844,1.1076765342260755,3.8438960129528175,-3.5633849019206885,-329722.66328231146,-831502.5960556079,1684317.2619497841
2024-12-18 18:58:56.540385,5414.32,18:58,23.4375,21.3125,-329719.99586882244,-831489.0888315559,1684325.5087183272,0.6798572419211268,11.28765278600622,3.9999611245002598,0.8707534052553543,3.2745656228147535,-3.3735268269000307,-329720.8666222277,-831492.3633971787,1684328.8822451541
2024-12-18 19:03:22.720385,5680.5,19:03,23.4375,21.375,-329719.0565516756,-831497.2156594751,1684315.629580289,1.6191743887611665,3.1608248668489978,-5.8791769137606025,0.8706616939549955,2.7354957206130384,-2.813825506750228,-329719.9272133696,-831499.9511551957,1684318.4434057956
2024-12-18 19:07:48.950385,5946.73,19:07,23.4375,21.375,-329720.8967589942,-831503.5876997171,1684313.4183226246,-0.22103292983956635,-3.2112153752241284,-8.090434578014538,1.003769586799622,2.40447078885821,-2.2505376053574895,-329721.900528581,-831505.992170506,1684315.66886023
2024-12-18 19:12:26.880385,6224.66,19:12,23.5,21.4375,-329720.1088299745,-831499.5122605907,1684325.714103488,0.5668960898765363,0.8642237512394786,4.205346285365522,0.7953679720106136,1.924924911892352,-1.8809589628418464,-329720.9041979465,-831501.4371855026,1684327.595062451
2024-12-18 19:17:16.020385,6513.8,19:17,23.5,21.4375,-329718.3055636255,-831496.6871576618,1684323.6026924623,2.3701624388922937,3.6893266801489517,2.093935259617865,0.8510791458732759,1.8250212431718995,-0.8336007700279533,-329719.1566427713,-831498.512178905,1684324.4362932323
2024-12-18 19:21:41.410385,6779.19,19:21,23.5,21.4375,-329728.04520013276,-831493.3138775824,1684313.0813223363,-7.36947406840045,7.062606759485789,-8.427434866316617,0.06777987202041827,1.7822703104022712,-0.16940895913700973,-329728.1129800048,-831495.0961478929,1684313.2507312954
2024-12-18 19:30:15.870385,7293.65,19:30,23.5625,21.4375,-329707.957659862,-831504.3154621603,1684325.2756238447,12.718066202360205,-3.938977818354033,3.766866642050445,0.31889127317117527,1.4014999949306781,0.7007367571793675,-329708.2765511352,-831505.7169621552,1684324.5748870876
2024-12-18 19:34:42.070385,7559.85,19:34,23.5625,21.4375,-329722.1308496459,-831502.0749451726,1684324.911580501,-1.4551235815160908,-1.6984608307247981,3.402823298238218,0.41369914488833665,0.878578607702539,1.5667904601321512,-329722.5445487908,-831502.9535237803,1684323.3447900407
2024-12-18 19:39:08.350385,7826.13,19:39,23.625,21.4375,-329723.92203649,-831490.8166231784,1684325.383995251,-3.2463104256312363,9.559861163492315,3.875238048378378,0.40185261580682846,0.5552880208761919,1.9816032786343603,-329724.3238891058,-831491.3719111993,1684323.4023919725
2024-12-18 19:43:46.950385,8104.73,19:43,23.5625,21.4375,-329728.2640210288,-831501.3794675837,1684317.077598689,-7.588294964458328,-1.0029832418076694,-4.431158513762057,0.4358614812483124,0.26444920915777664,2.4890494994774817,-329728.69988251006,-831501.6439167929,1684314.5885491895
2024-12-18 19:49:02.540385,8420.32,19:49,23.625,21.4375,-329717.1503920723,-831503.5445168669,1684320.374604887,3.525333992089145,-3.168032524990849,-1.134152315557003,0.1063257633081992,0.356692779681734,3.0351514180656523,-329717.2567178356,-831503.9012096466,1684317.339453469
2024-12-18 19:55:46.650385,8824.43,19:55,23.625,21.5,-329720.136378652,-831506.3065227275,1684325.0475935107,0.5393474123557098,-5.930038385558873,3.5388363080564886,-0.029584261436303633,-0.31363785105557845,3.0774601888399395,-329720.1067943906,-831505.9928848764,1684321.9701333218
2024-12-18 20:00:37.690385,9115.47,20:00,23.6875,21.5,-329716.62430527876,-831503.615658846,1684324.2352376778,4.0514207856031135,-3.239174504065886,2.7264804751612246,-0.1098776105070664,-0.15258614970038512,4.136449611313375,-329716.51442766824,-831503.4630726962,1684320.0987880665
2024-12-18 20:05:15.460385,9393.24,20:05,23.6875,21.5,-329719.3426564696,-831499.5263730271,1684324.649400956,1.3330695947515778,0.8501113147940487,3.140643753344193,-0.26203688439480693,-0.053657899860159626,4.824162487295412,-329719.08061958523,-831499.4727151273,1684319.8252384686
2024-12-18 20:13:01.930385,9859.71,20:13,23.6875,21.5625,-329715.30685748596,-831498.5024154825,1684336.371822926,5.368868578399997,1.8740688593825325,14.863065723329782,-0.21051350617060616,0.03524742641353181,4.919803629285612,-329715.0963439798,-831498.5376629089,1684331.4520192966
2024-12-18 20:18:42.830385,10200.61,20:18,23.6875,21.5625,-329726.96378998045,-831499.55158799,1684331.7443573736,-6.288063916086685,0.8248963518999517,10.235600170912221,-0.1747443184666779,-0.13825315342927796,5.919448357241761,-329726.789045662,-831499.4133348366,1684325.8249090163
2024-12-18 20:23:58.870385,10516.65,20:23,23.75,21.5625,-329719.4582099794,-831502.8238165089,1684327.282308744,1.2175160849583335,-2.4473321669502184,5.773551541380584,-0.3068908796523742,-0.27395156751542044,6.587322645853939,-329719.15131909976,-831502.5498649414,1684320.6949860982
2024-12-18 20:30:27.440385,10905.22,20:30,23.75,21.5625,-329718.8732384518,-831502.9271117876,1684331.8719371783,1.8024876125855371,-2.5506274456856772,10.36317997565493,-1.0288956850778224,0.02675156662284973,6.983164376446179,-329717.8443427667,-831502.9538633543,1684324.888772802
2024-12-18 20:35:16.510385,11194.29,20:35,23.75,21.5625,-329721.42363244126,-831502.2828161474,1684334.2928983753,-0.7479063768987544,-1.906331805512309,12.784141172654927,-0.8887999966529951,-0.21590893686239032,6.887168989162005,-329720.5348324446,-831502.0669072106,1684327.4057293863
2024-12-18 20:39:54.550385,11472.33,20:39,23.8125,21.5625,-329719.518749405,-831506.527774131,1684324.781676421,1.1569766593747772,-6.151289789122529,3.2729192182887346,-0.5933368671824046,-0.7300472238344983,7.46836678753607,-329718.9254125378,-831505.7977269072,1684317.3133096334
2024-12-18 20:44:20.950385,11738.73,20:44,23.8125,21.5625,-329728.475855854,-831496.8150446139,1684325.1667051725,-7.800129789626226,3.5614397280151024,3.6579479698557407,-0.5083372204736363,-0.5006400806929118,8.39694670580017,-329727.9675186335,-831496.3144045332,1684316.7697584666
2024-12-18 20:48:46.550385,12004.33,20:48,23.8125,21.5625,-329722.8499793421,-831503.1657748014,1684326.3972025134,-2.174253277713433,-2.7892904594773427,4.888445310760289,-0.30140464169172837,-0.44137844675597515,9.328599636620353,-329722.54857470037,-831502.7243963546,1684317.0686028767
2024-12-18 20:57:03.440385,12501.22,20:57,23.8125,21.5625,-329720.7427120061,-831493.8335737466,1684337.8683581608,-0.06698594172485173,6.542910595308058,16.359600958181545,-0.3030124977868538,-0.05346996397046106,10.068548475037373,-329720.4396995083,-831493.7801037827,1684327.799809686
2024-12-18 21:01:29.080385,12766.86,21:01,23.8125,21.5625,-329724.09210374585,-831501.5102064705,1684327.8602930203,-3.4163776814821176,-1.133722128579393,6.351535817608237,-0.5942301666807561,0.3702372297799836,10.477330297353634,-329723.49787357915,-831501.8804437002,1684317.3829627228
2024-12-18 21:07:09.840385,13107.62,21:07,23.8125,21.625,-329719.0268390318,-831497.6452487389,1684327.7225674698,1.6488870325847529,2.731235602986999,6.213810267159715,-0.24229864723470418,0.10835261809240494,10.926829191944783,-329718.78454038454,-831497.753601357,1684316.795738278
2024-12-18 21:11:36.180385,13373.96,21:11,23.8125,21.5625,-329717.5544106837,-831500.3306698385,1684344.5952317494,3.121315380674787,0.04581450344994664,23.08647454669699,-0.2531457020696031,-0.05588030995291081,11.017703137537907,-329717.3012649816,-831500.2747895286,1684333.5775286118
2024-12-18 21:16:01.710385,13639.49,21:16,23.875,21.625,-329730.82027791766,-831496.1635442782,1684327.1066823972,-10.144551853300072,4.212940063676797,5.59792519453913,0.15592569793252983,-0.2119607295663584,10.949860601475285,-329730.9762036156,-831495.9515835487,1684316.1568217957
2024-12-18 21:20:27.540385,13905.32,21:20,23.875,21.625,-329723.11976077594,-831498.0006963434,1684333.5883001871,-2.4440347115742043,2.37578799854964,12.079542984487489,0.12545613701444208,-0.16657950358820103,11.585583571843538,-329723.24521691294,-831497.8341168398,1684322.0027166153
2024-12-18 21:25:05.550385,14183.33,21:25,23.875,21.625,-329719.18884018896,-831507.1708157458,1684322.895677368,1.486885875405278,-6.794331403914839,1.386920165270567,0.10488840891602672,-0.0520449750557808,11.643791472129081,-329719.29372859787,-831507.1187707707,1684311.2518858959
2024-12-18 21:29:43.740385,14461.52,21:29,23.875,21.625,-329717.7173107711,-831501.6135272048,1684337.589149017,2.9584152932511643,-1.2370428629219532,16.080391814233735,0.2830515679559626,0.05770526265925063,11.595919945709673,-329718.0003623391,-831501.6712324675,1684325.9932290711
2024-12-18 21:35:37.260385,14815.04,21:35,23.875,21.625,-329726.47902844794,-831496.5619175778,1684336.5777769724,-5.8033023835741915,3.8145667641656473,15.069019769784063,0.2709289970613706,0.3611657713883601,12.323815887217366,-329726.749957445,-831496.9230833491,1684324.253961085
2024-12-18 21:42:56.340385,15254.12,21:42,23.875,21.625,-329712.80480791786,-831502.3000225542,1684339.9393164343,7.8709181465092115,-1.9235382123151794,18.430559231666848,0.6939224805987795,0.19132795377213152,12.994281685456546,-329713.4987303985,-831502.4913505081,1684326.9450347489
2024-12-18 21:47:59.800385,15557.58,21:47,23.9375,21.625,-329720.17014363,-831498.160444589,1684340.5865191175,0.5055824343580753,2.216039752936922,19.07776191481389,0.7389407624640236,0.22355765142544573,13.255671146680557,-329720.9090843925,-831498.3840022404,1684327.3308479707
2024-12-18 21:52:25.490385,15823.27,21:52,23.9375,21.625,-329722.73987632553,-831494.7178077772,1684332.8196559465,-2.064150261168834,5.658676564693451,11.310898743802682,0.7299651841389104,-0.2973747093818106,13.25351254413614,-329723.46984150965,-831494.4204330678,1684319.5661434024
2024-12-18 21:57:40.410385,16138.19,21:57,23.9375,21.625,-329711.95209456125,-831505.0259498726,1684334.0888777424,8.723631503118668,-4.649465530645102,12.580120539758354,0.9731029466077287,-0.5320129395418224,13.480806609260894,-329712.92519750784,-831504.493936933,1684320.6080711333
2024-12-18 22:02:18.590385,16416.37,22:02,23.9375,21.625,-329715.5346456375,-831501.9513069715,1684338.2801757834,5.14108042686712,-1.5748226295690984,16.771418580785394,0.7830028695586536,-0.6524490310001143,14.19712251932582,-329716.3176485071,-831501.2988579405,1684324.083053264
2024-12-18 22:06:56.630385,16694.41,22:06,23.9375,21.6875,-329718.3732905804,-831502.8292768019,1684330.3196641163,2.3024354839581065,-2.4527924599824473,8.810906913597137,0.671023335208052,-0.7970741491520866,13.581536325914342,-329719.0443139156,-831502.0322026528,1684316.7381277904
2024-12-18 22:11:33.970385,16971.75,22:11,23.9375,21.6875,-329720.0980707587,-831501.8708107633,1684340.6324911218,0.5776553056784905,-1.494326421408914,19.123733919113874,1.127490468051595,-1.1798709301344519,14.155819682626142,-329721.2255612267,-831500.6909398332,1684326.4766714391
2024-12-18 22:15:59.830385,17237.61,22:15,23.9375,21.6875,-329719.30516074185,-831500.5218866884,1684333.0943030843,1.3705653225188144,-0.14540234650485218,11.585545881651342,1.4558173020791618,-1.2679423060534256,14.52798611461185,-329720.76097804395,-831499.2539443824,1684318.5663169697
2024-12-18 22:20:50.600385,17528.38,22:20,23.9375,21.625,-329717.6822061014,-831499.9780611554,1684333.2875963205,2.9935199629398994,0.39842318650335073,11.778839117847383,1.024549295596357,-1.2154028492902096,14.544361789622123,-329718.706755397,-831498.7626583062,1684318.7432345308
2024-12-18 22:26:31.670385,17869.45,22:26,23.9375,21.6875,-329719.7733233938,-831500.1551034477,1684340.0674911926,0.9024026705883443,0.22138089418876916,18.55873398995027,0.6099792479903304,-1.0737992577432167,14.241118496250627,-329720.38330264174,-831499.08130419,1684325.8263726963
2024-12-18 22:30:57.190385,18134.97,22:30,24.0,21.6875,-329719.5929926997,-831500.3816387838,1684339.2464869355,1.0827333646593615,-0.005154441925697029,17.737729732878506,1.3269951678701633,-1.4288669949829844,13.94066499417559,-329720.9199878676,-831498.9527717888,1684325.3058219415
2024-12-18 22:36:25.650385,18463.43,22:36,23.9375,21.6875,-329721.9045954229,-831502.4889511507,1684331.8863811991,-1.2288693585433066,-2.1124668087577447,10.377623996464536,0.8594233771575437,-1.3962721729961534,13.92768357184139,-329722.76401880005,-831501.0926789776,1684317.9586976273
2024-12-18 22:42:57.210385,18854.99,22:42,23.9375,21.6875,-329720.9311991509,-831504.7731533236,1684337.8230275074,-0.2554730865522288,-4.396668981644325,16.31427030474879,1.1761319789165143,-2.027652938500978,13.504309651209041,-329722.10733112984,-831502.7455003851,1684324.3187178562
2024-12-18 22:47:22.730385,19120.51,22:47,24.0,21.6875,-329718.986210734,-831506.4376093039,1684332.6334683879,1.689515330363065,-6.06112496193964,11.12471118522808,1.3463528882767561,-2.304606895439238,13.62151628165018,-329720.3325636223,-831504.1330024084,1684319.0119521061
2024-12-18 22:54:00.900385,19518.68,22:54,24.0,21.6875,-329723.0189406498,-831500.1744066596,1684342.7652015812,-2.3432145854458213,0.20207768236286938,21.256444378523156,0.8128298666006664,-2.023228320636831,13.513444653035895,-329723.8317705164,-831498.1511783389,1684329.2517569282
2024-12-18 22:59:42.520385,19860.3,22:59,24.0,21.6875,-329719.90598090505,-831503.3677973197,1684331.6679216877,0.7697451593121514,-2.9913129777414724,10.159164485055953,0.5860876621362487,-2.1194955550433536,13.155341940000653,-329720.4920685672,-831501.2483017646,1684318.5125797477
2024-12-18 23:05:29.730385,20207.51,23:05,24.0,21.6875,-329721.23446812795,-831504.2022766789,1684339.1666328881,-0.5587420635856688,-3.8257923369528726,17.657875685486943,0.5321092257010085,-2.135248593692224,13.554999640222551,-329721.76657735364,-831502.0670280852,1684325.611633248
2024-12-18 23:10:20.940385,20498.72,23:10,24.0,21.6875,-329716.22489726136,-831499.8501952377,1684341.4037952588,4.450828803004697,0.526289104251191,19.89503805618733,0.5202004025645909,-2.62506001963768,12.945699778241327,-329716.74509766395,-831497.225135218,1684328.4580954807
2024-12-18 23:14:46.760385,20764.54,23:14,24.0,21.6875,-329728.2454683251,-831506.0674871538,1684323.2395665431,-7.569742260733619,-5.6910028118873015,1.730809340486303,0.5998650455869556,-3.0242258806469007,13.001696077053479,-329728.8453333707,-831503.0432612732,1684310.2378704662
2024-12-18 23:19:25.290385,21043.07,23:19,24.0,21.6875,-329726.42328177084,-831498.6398517824,1684331.221039856,-5.747555706475396,1.736632559564896,9.71228265343234,0.6864628323819488,-3.0933946377176436,13.295089680102787,-329727.1097446032,-831495.5464571447,1684317.925950176
2024-12-18 23:24:27.790385,21345.57,23:24,24.0,21.6875,-329711.42169413046,-831504.0183400598,1684330.2682534289,9.254031933902297,-3.6418557178694755,8.759496226208284,0.8229172469499255,-3.2850785922824537,13.050676590363894,-329712.2446113774,-831500.7332614675,1684317.2175768386
2024-12-18 23:30:31.950385,21709.73,23:30,24.0,21.6875,-329722.6238155228,-831501.6155312925,1684339.6667065653,-1.9480894584557973,-1.239046950591728,18.15794936264865,0.7745561726402402,-3.540588163194202,12.608523829263591,-329723.3983716955,-831498.0749431293,1684327.058182736
2024-12-18 23:34:57.570385,21975.35,23:34,24.0,21.6875,-329713.51926299307,-831511.4194406646,1684331.6956667842,7.156463071296457,-11.042956322664395,10.186909581534564,0.8701359538217297,-3.77418493611982,12.629553525686442,-329714.3893989469,-831507.6452557285,1684319.0661132585
2024-12-18 23:39:59.840385,22277.62,23:39,24.0,21.6875,-329719.16523722897,-831500.5338408729,1684335.2809951857,1.5104888353962451,-0.15735653101000935,13.772237983066589,0.9750974883292136,-3.6243125890614465,12.372924006133829,-329720.1403347173,-831496.9095282839,1684322.9080711796
2024-12-18 23:44:37.860385,22555.64,23:44,24.0,21.6875,-329723.15607801644,-831499.1169998017,1684331.8193735415,-2.480351952079218,1.2594845402054489,10.310616338858381,0.79702594328583,-3.384749703425249,12.23281644265877,-329723.95310395974,-831495.7322500983,1684319.586557099
2024-12-18 23:50:06.330385,22884.11,23:50,24.0,21.6875,-329720.29623193125,-831503.972918894,1684330.7600188097,0.3794941331143491,-3.596434552106075,9.251261607045308,1.02688312259159,-3.907608615317648,11.43535505788445,-329721.3231150538,-831500.0653102787,1684319.3246637518
2024-12-18 23:55:10.140385,23187.92,23:55,24.0,21.6875,-329719.50683774555,-831503.1600906135,1684338.712475821,1.1688883188180625,-2.7836062716087326,17.20371861825697,1.2779849472045455,-4.435774456687449,11.123311062786906,-329720.78482269275,-831498.7243161568,1684327.589164758
2024-12-19 00:00:01.220385,23479.0,00:00,24.0,21.6875,-329720.34815604455,-831512.1568507082,1684327.8371940202,0.32757001981372014,-11.780366366263479,6.328436817508191,1.4935599744951884,-4.461983441924011,10.938836051117894,-329721.84171601903,-831507.6948672662,1684316.898357969
2024-12-19 00:06:18.790385,23856.57,00:06,24.0,21.75,-329717.6322032384,-831508.9043697696,1684334.2702253594,3.0435228259884752,-8.527885427698493,12.761468156706542,1.2051043662414442,-4.658038272827287,10.0113989109883,-329718.8373076046,-831504.2463314967,1684324.2588264483
2024-12-19 00:12:00.050385,24197.83,00:12,23.9375,21.6875,-329715.86365257873,-831501.4306050539,1684339.4488619845,4.812073485634755,-1.0541207119822502,17.940104781882837,1.55873158253685,-4.508723092365211,10.412573252549572,-329717.42238416127,-831496.9218819615,1684329.036288732
2024-12-19 00:18:31.240385,24589.02,00:18,23.9375,21.6875,-329716.90778068785,-831504.1804664936,1684334.934816308,3.767945376515854,-3.803982151672244,13.426059105433524,2.2629448169055175,-5.045655702961431,10.132877112665613,-329719.17072550475,-831499.1348107907,1684324.8019391955
2024-12-19 00:23:55.080385,24912.86,00:23,23.9375,21.6875,-329720.6085752602,-831505.747339773,1684329.9612789524,0.06715080415597185,-5.370855431072414,8.452521749772131,1.8577016826214579,-4.869501940495822,9.869648109966269,-329722.4662769428,-831500.8778378326,1684320.0916308425
2024-12-19 00:28:44.220385,25202.0,00:28,23.9375,21.6875,-329719.8974200181,-831507.3944833821,1684332.328004824,0.7783060462679714,-7.017999040195718,10.819247621344402,2.1591129665445936,-5.1261807614105885,9.432857418898493,-329722.05653298466,-831502.2683026207,1684322.895147405
2024-12-19 00:33:09.970385,25467.75,00:33,23.9375,21.625,-329718.72700692626,-831501.6258340353,1684332.4338075968,1.9487191381049342,-1.2493496934184805,10.92505039414391,1.760642904610861,-4.7332083213120875,9.37166213992584,-329720.4876498309,-831496.8926257141,1684323.062145457
2024-12-19 00:37:35.530385,25733.31,00:37,23.9375,21.625,-329722.7257131799,-831501.4067887055,1684329.691209555,-2.0499871155479923,-1.0303043635794893,8.182452352251858,1.860201590669541,-4.8712757724071185,8.908433366489286,-329724.5859147706,-831496.535512933,1684320.7827761883
2024-12-19 00:42:02.550385,26000.33,00:42,23.9375,21.625,-329718.1919398844,-831511.1544438093,1684326.018512501,2.483786179975141,-10.777959467377514,4.509755298262462,2.048332978644231,-4.923901805681886,8.54667335029115,-329720.240272863,-831506.2305420036,1684317.4718391506
2024-12-19 00:46:54.690385,26292.47,00:46,23.9375,21.625,-329714.6328425882,-831514.4592799884,1684325.1149977907,6.042883476184215,-14.082795646507293,3.606240588007495,2.1463914915359403,-5.075431008030483,8.196298164060517,-329716.7792340797,-831509.3838489804,1684316.9186996266
2024-12-19 00:51:33.800385,26571.58,00:51,23.9375,21.625,-329716.70739255485,-831504.7526653688,1684335.292657643,3.9683335095178336,-4.376181026920676,13.78390044043772,2.144562243087594,-5.0460926541182705,8.025114093064552,-329718.8519547979,-831499.7065727147,1684327.26754355
2024-12-19 00:55:59.300385,26837.08,00:55,23.9375,21.625,-329722.2824650347,-831503.9673466866,1684321.9276153161,-1.6067389703239314,-3.590862344717607,0.4188581134658307,2.2222388842187466,-4.291382700631705,7.819435104561437,-329724.5047039189,-831499.675963986,1684314.1081802116
2024-12-19 01:00:49.610385,27127.39,01:00,23.875,21.625,-329720.8192967829,-831502.9318683641,1684331.664227716,-0.14357071853009984,-2.5553840221837163,10.15547051327303,1.9451513506078517,-3.8792392556622093,7.448282990782034,-329722.76444813353,-831499.0526291084,1684324.215944725
2024-12-19 01:05:15.210385,27392.99,01:05,23.875,21.625,-329711.6348038491,-831509.9154366049,1684325.3474209185,9.040922215266619,-9.538952262955718,3.8386637158691883,1.7188850096371469,-4.253189224184358,6.527903918897556,-329713.35368885874,-831505.6622473807,1684318.8195169996
2024-12-19 01:11:06.660385,27744.44,01:11,23.875,21.625,-329719.9317999504,-831500.319111048,1684324.7404443722,0.7439261139370501,0.05737329390831292,3.231687169522047,1.4242154187467393,-4.199820432296422,6.465114540442647,-329721.3560153692,-831496.1192906157,1684318.2753298318
2024-12-19 01:16:09.740385,28047.52,01:16,23.875,21.5625,-329716.29417856043,-831507.0057865317,1684330.4941020529,4.381547503930051,-6.62930218980182,8.985344850225374,1.2840378258066873,-4.0861231333443095,5.8808150648449855,-329717.57821638626,-831502.9196633984,1684324.613286988
2024-12-19 01:20:35.270385,28313.05,01:20,23.875,21.5625,-329721.8871342937,-831503.1670194225,1684330.4105659258,-1.2114082293119282,-2.7905350805958733,8.901808723108843,1.5137818616376968,-3.9382434826166857,5.5878547469952276,-329723.4009161553,-831499.2287759399,1684324.8227111788
2024-12-19 01:25:01.190385,28578.97,01:25,23.875,21.5625,-329717.07450482174,-831503.4332573459,1684325.5531909436,3.601221242628526,-3.056773004005663,4.044433740898967,1.3618297768740117,-4.027021531752932,5.374667336887104,-329718.43633459863,-831499.4062358142,1684320.1785236066
2024-12-19 01:29:26.910385,28844.69,01:29,23.875,21.5625,-329719.205318869,-831500.2221465005,1684324.2224132014,1.4704071953892708,0.15433784143533558,2.7136559986975044,1.5947510002934862,-4.020065529587945,4.9977677165685845,-329720.80006986926,-831496.2020809709,1684319.2246454847
2024-12-19 01:34:17.230385,29135.01,01:34,23.875,21.5625,-329718.2370031605,-831507.1550321433,1684323.4021398989,2.438722903840244,-6.778547801426612,1.8933826962020248,1.6509970058326697,-3.3883947480769296,5.124491726780044,-329719.88800016633,-831503.7666373953,1684318.277648172
2024-12-19 01:38:43.310385,29401.09,01:38,23.8125,21.5625,-329719.54525196296,-831502.5439851814,1684335.11761033,1.1304741014027968,-2.1675008394522592,13.608853127341717,1.2230750358319797,-2.6703970746214813,5.100696956250994,-329720.7683269988,-831499.8735881067,1684330.0169133737
2024-12-19 01:43:09.460385,29667.24,01:43,23.8125,21.5,-329718.7169465808,-831496.307941685,1684323.5179352616,1.9587794835679233,4.068542656954378,2.00917805894278,1.1380389951047531,-2.412793429928743,4.7384430259089205,-329719.8549855759,-831493.895148255,1684318.7794922357
2024-12-19 01:47:34.870385,29932.65,01:47,23.8125,21.5625,-329723.4510414442,-831500.2493574253,1684326.47603097,-2.775315379840322,0.12712691666092724,4.967273767339066,1.309123386451531,-2.4810290153892267,4.717882599958795,-329724.76016483066,-831497.7683284099,1684321.75814837
2024-12-19 01:52:00.410385,30198.19,01:52,23.8125,21.5625,-329720.6152457391,-831509.2835543929,1684320.120901475,0.06048032524995506,-8.907070050947368,-1.3878557276912034,1.116699765400318,-2.400204414562766,4.452157855233444,-329721.7319455045,-831506.8833499782,1684315.6687436197
2024-12-19 01:56:26.310385,30464.09,01:56,23.8125,21.5,-329723.09584209655,-831503.059721864,1684333.6162393605,-2.4201160321827047,-2.6832375220255926,12.10748215788044,0.8960267735112991,-1.8256496663393809,4.574033567892565,-329723.99186887004,-831501.2340721976,1684329.0422057926
2024-12-19 02:00:52.260385,30730.04,02:00,23.8125,21.5,-329723.55230471195,-831503.359696495,1684317.6909899649,-2.87657864758512,-2.983212153078057,-3.817767237778753,1.2575230094482235,-2.078161980042101,4.727138849352265,-329724.8098277214,-831501.281534515,1684312.9638511154
2024-12-19 02:05:18.500385,30996.28,02:05,23.8125,21.5625,-329715.07279526565,-831504.2890107168,1684326.1758381492,5.602930798719171,-3.9125263749156147,4.667080946499482,1.1818449567820477,-1.7608275654880952,4.599328939049017,-329716.2546402224,-831502.5281831514,1684321.57650921
2024-12-19 02:09:44.290385,31262.07,02:09,23.8125,21.5625,-329721.9180007063,-831503.4901730672,1684327.9568719845,-1.242274641932454,-3.113688725279644,6.448114781873301,1.3304266944815892,-1.7108074392225328,4.354204103738691,-329723.2484274008,-831501.779365628,1684323.6026678807
2024-12-19 02:14:09.910385,31527.69,02:14,23.8125,21.5,-329717.8343674881,-831501.26071266,1684321.7763175282,2.8413585762609728,-0.884228318114765,0.26756032556295395,1.1061321624604585,-1.6527367163438438,3.8860678815482452,-329718.94049965055,-831499.6079759437,1684317.8902496467
2024-12-19 02:18:35.540385,31793.32,02:18,23.8125,21.5,-329717.01077376807,-831497.8893573976,1684328.6797167154,3.6649522962979972,2.487126944353804,7.170959512703121,0.9031944505460117,-1.9593209313627864,3.831039555415156,-329717.9139682186,-831495.9300364662,1684324.84867716
2024-12-19 02:23:00.820385,32058.6,02:23,23.8125,21.5,-329723.6192039582,-831499.3813288459,1684324.6153076096,-2.943477893830277,0.995155496057123,3.1065504068974406,1.0077263585463654,-1.6220603173243857,3.7033946312675696,-329724.62693031674,-831497.7592685285,1684320.9119129784
2024-12-19 02:27:27.130385,32324.91,02:27,23.8125,21.5,-329718.4931494101,-831499.3429888303,1684327.685325106,2.182576654246077,1.0334955116268247,6.176567903254181,1.1721872217687113,-1.7239565897200788,3.234371972447705,-329719.6653366319,-831497.6190322406,1684324.4509531334
2024-12-19 02:31:52.870385,32590.65,02:31,23.8125,21.5,-329718.6896928164,-831505.4002939813,1684321.4958463712,1.986033247958403,-5.023809639387764,-0.012910831486806273,1.3065593535014028,-1.8488366872160917,3.5407109432410273,-329719.9962521699,-831503.5514572941,1684317.9551354279
2024-12-19 02:36:32.140385,32869.92,02:36,23.75,21.5,-329724.86019282497,-831501.2345517467,1684326.0840080767,-4.184466760605574,-0.8580674048280343,4.575250874040648,1.559754006888917,-1.7491246788718162,3.469778005244388,-329726.4199468319,-831499.4854270678,1684322.6142300714
2024-12-19 02:41:22.860385,33160.64,02:41,23.75,21.5,-329716.26893667877,-831497.8497868922,1684327.9068108844,4.4067893855972216,2.526697449735366,6.398053681710735,1.7361801126251175,-1.5397958106838079,3.5657185838069942,-329718.0051167914,-831496.3099910815,1684324.3410923006
2024-12-19 02:45:48.650385,33426.43,02:45,23.75,21.5,-329712.34037899575,-831505.6218696358,1684327.9556552828,8.335347068612464,-5.245385293848813,6.4468980801757425,1.682645052383166,-1.971596772710438,2.8371574217010114,-329714.02302404813,-831503.6502728631,1684325.118497861
2024-12-19 02:50:14.420385,33692.2,02:50,23.75,21.4375,-329717.8834176664,-831500.3417638261,1684327.8100939365,2.79230839794036,0.034720515832304955,6.30133673385717,1.7377885984744699,-1.9992400816963276,2.9618227318417105,-329719.6212062649,-831498.3425237444,1684324.8482712046
2024-12-19 02:54:40.340385,33958.12,02:54,23.6875,21.5,-329718.766917802,-831502.1165967709,1684325.2629443842,1.908808262378443,-1.7401124290190637,3.7541871815919876,1.3778911516918535,-1.849331751632105,2.6832994869134077,-329720.1448089537,-831500.2672650194,1684322.5796448973
2024-12-19 02:59:07.490385,34225.27,02:59,23.75,21.5,-329721.7846899942,-831502.2137721655,1684315.7223302776,-1.1089639298152179,-1.837287823553197,-5.786426925100386,1.7631822804105468,-1.9114786043896206,2.4226345276083086,-329723.5478722746,-831500.302293561,1684313.29969575
2024-12-19 03:03:46.100385,34503.88,03:03,23.75,21.4375,-329723.4670108192,-831506.6604150159,1684323.0668183526,-2.7912847548141144,-6.283930673962459,1.5580611499026418,1.5629381447104693,-1.5244001212940064,2.381657785447758,-329725.0299489639,-831505.1360148946,1684320.685160567
2024-12-19 03:08:24.290385,34782.07,03:08,23.75,21.4375,-329716.0418330925,-831500.0725592485,1684320.7215964918,4.633892971847672,0.303925093379803,-0.7871607108972967,1.5466744244331494,-1.6007398516549507,1.9970967301965825,-329717.58850751695,-831498.4718193968,1684318.7244997616
2024-12-19 03:13:52.400385,35110.18,03:13,23.6875,21.4375,-329716.0915738353,-831504.6838069017,1684325.2681344948,4.58415222907206,-4.307322559761815,3.7593772921245545,1.8047457643662623,-1.8082985249126242,1.6518472444066512,-329717.89631959965,-831502.8755083767,1684323.6162872503
2024-12-19 03:18:55.990385,35413.77,03:18,23.6875,21.4375,-329715.8951318144,-831498.9304237324,1684329.9510536483,4.780594249954447,1.446060609538108,8.442296445602551,1.8503490522769945,-2.013795278024017,1.2279233703101498,-329717.7454808667,-831496.9166284543,1684328.723130278
2024-12-19 03:23:21.550385,35679.33,03:23,23.6875,21.4375,-329718.13395372307,-831498.15540525,1684324.986439272,2.5417723412974738,2.221079091890715,3.4776820694096386,1.6009068382499252,-1.5721944757083075,1.0918717984930568,-329719.7348605613,-831496.5832107743,1684323.8945674736
2024-12-19 03:27:47.090385,35944.87,03:27,23.75,21.4375,-329716.91029751865,-831504.8876481609,1684322.1356536248,3.765428545710165,-4.511163818999194,0.6268964221235365,1.9941142649622634,-1.6129217863060712,0.764831290691204,-329718.9044117836,-831503.2747263747,1684321.3708223342
2024-12-19 03:32:25.780385,36223.56,03:32,23.6875,21.4375,-329724.2200783616,-831512.1275420665,1684318.3164549563,-3.5443522972636856,-11.751057724584825,-3.192302246345207,1.8200317982728371,-1.8177380208979317,0.20213326399347611,-329726.0401101599,-831510.3098040456,1684318.1143216924
2024-12-19 03:36:51.590385,36489.37,03:36,23.6875,21.4375,-329722.39429024403,-831503.9402059837,1684320.3089614778,-1.7185641796677373,-3.56372164178174,-1.199795724824071,1.3124268696770915,-1.8508718724007762,-0.4770924928487234,-329723.70671711373,-831502.0893341113,1684320.7860539707
2024-12-19 03:41:17.820385,36755.6,03:41,23.6875,21.4375,-329722.6306416481,-831501.1409357855,1684320.3268500057,-1.9549155837157741,-0.7644514435669407,-1.181907196994871,1.2255648968164765,-1.9489770578331358,-1.0831766019663995,-329723.8562065449,-831499.1919587277,1684321.4100266076
2024-12-19 03:45:43.920385,37021.7,03:45,23.6875,21.4375,-329713.8268870032,-831504.7952569751,1684322.4829078391,6.848839061160106,-4.418772633187473,0.97415063646622,1.2358298313670926,-1.5034686660371899,-0.965083634735839,-329715.0627168346,-831503.2917883091,1684323.4479914738
2024-12-19 03:50:09.820385,37287.6,03:50,23.6875,21.375,-329722.0394943378,-831493.132064515,1684320.9158059428,-1.3637682734406553,7.244419826893136,-0.5929512598086149,1.5149963111561235,-1.621427002684435,-1.0142864827510147,-329723.55449064897,-831491.5106375123,1684321.9300924256
2024-12-19 03:54:35.430385,37553.21,03:54,23.625,21.375,-329717.3523118939,-831499.4924917351,1684320.603934555,3.3234141704742797,0.8839926067739725,-0.9048226475715637,1.8201137472753457,-1.2782589223989773,-1.1966766838228242,-329719.17242564115,-831498.2142328128,1684321.800611239
2024-12-19 03:59:13.480385,37831.26,03:59,23.625,21.4375,-329718.1997058196,-831503.7400609843,1684317.365068408,2.4760202447650954,-3.363576642354019,-4.143688794691116,1.4681462140260486,-1.249260252397064,-1.4233414509910203,-329719.6678520336,-831502.4908007319,1684318.788409859
2024-12-19 04:03:39.070385,38096.85,04:03,23.625,21.375,-329717.535480364,-831503.6584206456,1684318.7829237499,3.1402457003714517,-3.2819363037124276,-2.725833452772349,1.0979720028616222,-1.1863565538799212,-2.0102607688556113,-329718.63345236686,-831502.4720640917,1684320.7931845188
2024-12-19 04:08:05.060385,38362.84,04:08,23.625,21.375,-329723.927979311,-831496.1266771327,1684318.638763363,-3.252253246610053,4.249807209242135,-2.8699938396457583,1.0663731258717322,-1.044996920174786,-2.51931891091434,-329724.99435243686,-831495.0816802125,1684321.158082274
2024-12-19 04:12:30.660385,38628.44,04:12,23.625,21.375,-329716.602836864,-831502.0898252693,1684319.2161574129,4.072889200353529,-1.7133409273810685,-2.2925997897982597,1.0188347399290207,-1.0362656041480867,-3.181183414633519,-329717.62167160393,-831501.0535596651,1684322.3973408274
2024-12-19 04:16:56.570385,38894.35,04:16,23.625,21.375,-329719.92466847925,-831502.1509278186,1684316.0901523237,0.7510575851192698,-1.7744434766937047,-5.418604878941551,0.911328686226625,-0.8826764676099023,-3.3917268363958493,-329720.8359971655,-831501.268251351,1684319.48187916
2024-12-19 04:21:22.120385,39159.9,04:21,23.5625,21.375,-329723.00008249626,-831506.3176805173,1684313.6919143891,-2.3243564318981953,-5.94119617540855,-7.816842813510448,1.1900366736891945,-0.529908472522428,-3.5113085401577075,-329724.19011916994,-831505.7877720448,1684317.2032229293
2024-12-19 04:26:01.030385,39438.81,04:26,23.625,21.375,-329719.7075190965,-831502.4019727202,1684315.082327645,0.9682069678674452,-2.025488378247246,-6.4264295576140285,1.0752590228193661,-0.1441071288427338,-3.610372173943601,-329720.7827781193,-831502.2578655913,1684318.6926998189
2024-12-19 04:30:26.820385,39704.6,04:30,23.625,21.3125,-329718.5513541764,-831492.7609205432,1684327.742896696,2.124371887941379,7.615563798695803,6.234139493433759,0.8650640852228251,-0.13605341075232164,-3.9966602843986556,-329719.41641826165,-831492.6248671325,1684331.7395569806
2024-12-19 04:35:05.200385,39982.98,04:35,23.5625,21.3125,-329715.9221939186,-831504.6908972351,1684314.6890704692,4.753532145754434,-4.314412893145345,-6.819686733419076,0.6516105530207001,0.19237876294313797,-4.144569850349355,-329716.57380447164,-831504.883275998,1684318.8336403195
2024-12-19 04:39:43.360385,40261.14,04:39,23.5625,21.375,-329717.0595446607,-831499.4538853299,1684319.23662413,3.616181403689552,0.9225990120321512,-2.2721330726053566,0.7324588771970455,-0.11654045704441766,-4.388047497641916,-329717.7920035379,-831499.3373448729,1684323.6246716278
2024-12-19 04:44:09.470385,40527.25,04:44,23.5625,21.3125,-329723.43315129075,-831499.4635871785,1684315.9616363812,-2.757425226387568,0.9128971634199843,-5.5471208214294165,0.5232828224099995,-0.06423740136060155,-4.893750358694454,-329723.95643411315,-831499.3993497771,1684320.8553867398
2024-12-19 04:48:58.730385,40816.51,04:48,23.5625,21.3125,-329723.86523226975,-831503.3628292328,1684312.9428288196,-3.1895062053808942,-2.986344890901819,-8.56592838303186,0.18827494270434336,0.09969822934363037,-5.429297454799304,-329724.05350721243,-831503.4625274622,1684318.3721262745
2024-12-19 04:53:24.970385,41082.75,04:53,23.5625,21.3125,-329716.5587082312,-831495.9618714246,1684319.260832665,4.117017833166756,4.4146129173459485,-2.2479245376307517,-0.08146583736552634,-0.06969470078391689,-6.29609845223881,-329716.4772423938,-831495.8921767238,1684325.5569311173
2024-12-19 04:57:51.030385,41348.81,04:57,23.5625,21.3125,-329719.13225982786,-831497.9720476135,1684311.087284694,1.5434662365005352,2.404436728451401,-10.421472508693114,-0.1781765662543919,-0.08467352961278743,-6.607851063655246,-329718.9540832616,-831497.8873740839,1684317.6951357576
2024-12-19 05:03:05.320385,41663.1,05:03,23.5625,21.375,-329719.1679246464,-831501.6622762936,1684317.7142417678,1.507801417959854,-1.2857919516973197,-3.7945154348853976,-0.38127737117299276,0.031195488891431263,-7.037924440976765,-329718.7866472752,-831501.6934717825,1684324.7521662088
2024-12-19 05:07:30.820385,41928.6,05:07,23.5,21.3125,-329718.3672106249,-831504.7194141697,1684315.8052391773,2.308515439450275,-4.3429298277478665,-5.703518025344238,-0.517486226553696,0.3009022567088583,-7.191644690698013,-329717.84972439834,-831505.0203164264,1684322.996883868
2024-12-19 05:12:46.940385,42244.72,05:12,23.5,21.3125,-329724.8046209123,-831495.8383777664,1684318.2286251683,-4.128894847934134,4.538106575491838,-3.280132034327835,-0.2833008291366111,0.32836922999870566,-7.676941547753467,-329724.5213200832,-831496.1667469965,1684325.905566716
2024-12-19 05:17:24.210385,42521.99,05:17,23.5,21.25,-329727.0447353376,-831500.9718077056,1684312.214799686,-6.369009273243137,-0.5953233636682853,-9.293957516551018,-0.21170636796991207,0.3520972223930238,-7.714809118714627,-329726.83302896965,-831501.3239049279,1684319.9296088049
2024-12-19 05:22:13.900385,42811.68,05:22,23.5,21.3125,-329718.30941117945,-831497.8981813275,1684319.3768069542,2.3663148849154823,2.478303014417179,-2.1319502484984696,-0.5129647809995471,0.011402994266799873,-8.474140139939706,-329717.7964463984,-831497.9095843218,1684327.8509470941
2024-12-19 05:27:28.860385,43126.64,05:27,23.5,21.3125,-329720.3416795301,-831499.6193681348,1684315.8027753497,0.33404653426259756,0.7571162071544677,-5.705981852952391,-0.89208129395376,0.6321239175740629,-8.550970530991131,-329719.4495982361,-831500.2514920523,1684324.3537458808
2024-12-19 05:31:54.530385,43392.31,05:31,23.5,21.25,-329721.7450090444,-831498.3941275658,1684309.984174473,-1.0692829800536856,1.982356776134111,-11.524582729674876,-1.1130630159029915,0.3729376798506737,-9.341190264061359,-329720.6319460285,-831498.7670652457,1684319.325364737
2024-12-19 05:38:13.100385,43770.88,05:38,23.5,21.3125,-329725.2348712934,-831500.2974127395,1684306.1185793898,-4.559145229053684,0.07907160243485123,-15.390177812892944,-1.2382077329176744,0.30836992336082314,-9.932867270606081,-329723.9966635605,-831500.6057826629,1684316.0514466604
2024-12-19 05:42:52.060385,44049.84,05:42,23.5,21.3125,-329723.20003674546,-831507.2156721783,1684300.5801028037,-2.5243106810958125,-6.83918783639092,-20.92865439900197,-1.301266740785823,0.40439339972189847,-10.211616836066934,-329721.8987700047,-831507.620065578,1684310.7917196397
2024-12-19 05:47:17.750385,44315.53,05:47,23.4375,21.3125,-329725.95890461764,-831496.4412325381,1684312.0919585233,-5.28317855327623,3.935251803835854,-9.416798679390922,-1.7089459196625587,0.3157367819332562,-10.588049743069513,-329724.249958698,-831496.75696932,1684322.6800082664
2024-12-19 05:51:55.560385,44593.34,05:51,23.5,21.25,-329720.8679537673,-831499.6565758807,1684310.184616489,-0.1922277029370889,0.7199084612075239,-11.32414071355015,-1.7618225484426755,0.2837924366606222,-10.77887397717374,-329719.10613121884,-831499.9403683174,1684320.9634904664
2024-12-19 05:56:22.010385,44859.79,05:56,23.4375,21.3125,-329722.78505444224,-831496.4870856944,1684312.8620270796,-2.1093283778754994,3.8893986474722624,-8.646730123087764,-2.1204635565352095,0.21381345304239185,-11.744487297410766,-329720.6645908857,-831496.7008991475,1684324.606514377
2024-12-19 06:00:47.410385,45125.19,06:00,23.4375,21.25,-329718.0821891505,-831505.7408740782,1684303.500680391,2.5935369138605893,-5.364389736321755,-18.008076811674982,-2.7673759185986238,0.3891245926830119,-12.222256348545974,-329715.31481323193,-831506.1299986709,1684315.7229367394
2024-12-19 06:06:15.550385,45453.33,06:06,23.4375,21.3125,-329718.204035412,-831501.9036848799,1684314.2871086549,2.4716906523681246,-1.5272005379665643,-7.221648547798395,-2.9659728384354995,0.19802186727368584,-12.935831590611045,-329715.23806257354,-831502.1017067472,1684327.2229402454
2024-12-19 06:10:41.130385,45718.91,06:10,23.4375,21.3125,-329724.87778085005,-831499.9154993339,1684311.7969452504,-4.202054785680957,0.4609850080450997,-9.71181195229292,-2.874031429991148,0.5706960539821357,-13.53033976999688,-329722.00374942005,-831500.4861953879,1684325.3272850204
2024-12-19 06:15:06.870385,45984.65,06:15,23.4375,21.3125,-329723.88364069065,-831491.6557578456,1684313.0756322572,-3.207914626284037,8.72072649630718,-8.433124945499003,-3.5205644419849187,0.4678664479094247,-14.273761611609231,-329720.3630762487,-831492.1236242935,1684327.3493938688
2024-12-19 06:19:58.060385,46275.84,06:19,23.4375,21.25,-329721.7001608216,-831504.8967963221,1684302.6420097356,-1.0244347572443075,-4.520311980159022,-18.86674746708013,-4.036135205666402,0.5910850941713545,-14.787910068784619,-329717.66402561596,-831505.4878814162,1684317.4299198044
2024-12-19 06:24:24.010385,46541.79,06:24,23.4375,21.25,-329726.06119034806,-831500.8195100648,1684303.5364192438,-5.38546428369591,-0.4430257228668779,-17.972337958868593,-4.025905515890502,0.6425190021538929,-14.957336135729705,-329722.0352848322,-831501.462029067,1684318.4937553795
2024-12-19 06:29:02.260385,46820.04,06:29,23.4375,21.25,-329725.189471435,-831501.3463362292,1684307.089087945,-4.513745370612014,-0.969851887319237,-14.419669257709756,-3.897048708508789,1.0277128099530404,-14.772008692246995,-329721.29242272646,-831502.3740490392,1684321.861096637
2024-12-19 06:33:28.000385,47085.78,06:33,23.4375,21.25,-329725.1199709876,-831497.8236603981,1684311.355741618,-4.444244923244696,2.5528239437844604,-10.153015584684908,-3.6864215192396106,1.2397862126263568,-14.470759597695654,-329721.43354946835,-831499.0634466108,1684325.8265012156
2024-12-19 06:37:53.760385,47351.54,06:37,23.4375,21.25,-329720.24266903225,-831498.6428788642,1684307.0799757778,0.43305703211808577,1.733605477726087,-14.42878142488189,-3.310966129348214,0.9993434878942069,-14.521727064801823,-329716.9317029029,-831499.6422223521,1684321.6017028426
2024-12-19 06:42:19.370385,47617.15,06:42,23.375,21.3125,-329726.69938581635,-831503.1318349496,1684297.4363620428,-6.0236597519833595,-2.755350607680157,-24.072395159862936,-3.3759560348477127,0.9121343593855965,-14.680206215751934,-329723.3234297815,-831504.043969309,1684312.1165682585
2024-12-19 06:47:09.210385,47906.99,06:47,23.4375,21.25,-329731.95237022825,-831501.0378802372,1684305.7720891035,-11.276644163881429,-0.6613958952948451,-15.73666809918359,-3.5868081591685215,1.0851435453653158,-15.107758214131795,-329728.36556206906,-831502.1230237826,1684320.8798473177
2024-12-19 06:51:34.620385,48172.4,06:51,23.4375,21.25,-329728.9751562289,-831499.851535,1684303.243545085,-8.299430164508522,0.5249493418959901,-18.26521211769432,-3.926390203209372,1.3792346219942417,-14.726530873471694,-329725.0487660257,-831501.230769622,1684317.9700759584
2024-12-19 06:56:13.480385,48451.26,06:56,23.4375,21.25,-329725.1139657603,-831493.1456497847,1684299.730127919,-4.438239695911761,7.230834557209164,-21.778629283653572,-4.003239296886715,1.6241942760479149,-15.036985994693602,-329721.1107264634,-831494.7698440608,1684314.7671139138
2024-12-19 07:02:28.580385,48826.36,07:02,23.375,21.25,-329731.8866044313,-831500.057603055,1684303.7649482803,-11.210878366953693,0.318881286890246,-17.743808922357857,-4.437815564091406,1.9849748783245948,-15.660656709523339,-329727.4487888672,-831502.0425779334,1684319.4256049898
2024-12-19 07:07:06.940385,49104.72,07:07,23.4375,21.1875,-329731.1686655674,-831497.0317765633,1684305.005657749,-10.492939503048547,3.3447077786549926,-16.503099453635514,-4.486384048575668,1.8911127030816195,-15.931907787597517,-329726.6822815188,-831498.9228892664,1684320.9375655367
2024-12-19 07:11:32.640385,49370.42,07:11,23.375,21.1875,-329721.5301855591,-831497.3140154982,1684306.4262270671,-0.8544594947597943,3.0624688437674195,-15.082530135521665,-4.509560756959088,1.935399369386557,-15.40913445815178,-329717.02062480216,-831499.2494148675,1684321.8353615252
2024-12-19 07:18:15.910385,49773.69,07:18,23.4375,21.25,-329722.5288783384,-831492.2083427757,1684310.010455703,-1.8531522740377113,8.168141566216946,-11.498301499756053,-4.517132419167043,2.1885528358675184,-14.926408080716751,-329718.01174591924,-831494.3968956115,1684324.9368637835
2024-12-19 07:24:09.630385,50127.41,07:24,23.375,21.25,-329718.7768657708,-831502.7621307222,1684306.9063337892,1.898860293556936,-2.3856463802512735,-14.602423413423821,-4.5222843879462395,2.472208446013697,-14.79232771895338,-329714.25458138285,-831505.2343391682,1684321.6986615083
2024-12-19 07:31:05.120385,50542.9,07:31,23.375,21.25,-329718.0743414299,-831501.4905297575,1684311.021641714,2.601384634443093,-1.1140454155392945,-10.487115488620475,-4.982780270993577,2.746115943793917,-14.723667173945744,-329713.09156115894,-831504.2366457012,1684325.745308888
2024-12-19 07:35:43.940385,50821.72,07:35,23.375,21.25,-329722.2327417828,-831501.4879675794,1684306.8565543192,-1.5570157184265554,-1.1114832374732941,-14.652202883502468,-5.026783348925944,2.9203146962958964,-14.590685154089616,-329717.20595843386,-831504.4082822757,1684321.4472394732
2024-12-19 07:40:47.610385,51125.39,07:40,23.375,21.25,-329727.212949053,-831492.8538927889,1684303.8834351136,-6.537222988612484,7.522591553046368,-17.625322089064866,-4.854146987263535,3.3668917729574743,-13.674614970394899,-329722.3588020657,-831496.2207845618,1684317.558050084
2024-12-19 07:46:16.080385,51453.86,07:46,23.375,21.25,-329725.21341207536,-831499.564961469,1684311.5064545448,-4.537686010997277,0.8115228728856891,-10.002302657812834,-4.336790792328039,3.522487668736306,-13.381103726669348,-329720.876621283,-831503.0874491378,1684324.8875582714
2024-12-19 07:50:41.910385,51719.69,07:50,23.375,21.25,-329719.8178663792,-831496.7595321448,1684307.7675511092,0.8578596851439215,3.616952197160572,-13.741206093458459,-4.023613120714712,3.7159948302266588,-13.348349941184832,-329715.7942532585,-831500.475526975,1684321.1159010504
2024-12-19 07:55:07.850385,51985.63,07:55,23.375,21.25,-329734.00388246134,-831492.3391066861,1684298.699860239,-13.328156396979466,8.03737765585538,-22.808896963717416,-4.00288179195486,3.5402528438775334,-12.926835974061396,-329730.0010006694,-831495.8793595299,1684311.626696213
2024-12-19 07:59:46.380385,52264.16,07:59,23.375,21.25,-329724.9035788648,-831493.6268635257,1684307.3793596176,-4.227852800453547,6.749620816204697,-14.129397585056722,-3.623513551165448,3.709798715297917,-12.673311082045792,-329721.2800653137,-831497.336662241,1684320.0526706995
2024-12-19 08:05:35.150385,52612.93,08:05,23.375,21.25,-329722.18687169766,-831503.9667763297,1684313.620249654,-1.5111456332961097,-3.590291987755336,-7.8885075487196445,-3.2418787760608314,3.7300815451114127,-12.46054506140192,-329718.9449929216,-831507.6968578747,1684326.0807947153
2024-12-19 08:12:05.790385,53003.57,08:12,23.375,21.3125,-329726.2201952544,-831495.5032872687,1684313.67367317,-5.544469190062955,4.873197073233314,-7.835084032732993,-3.3823152043726568,3.769352880484589,-12.306310645277229,-329722.83788005006,-831499.2726401492,1684325.9799838152
2024-12-19 08:16:44.280385,53282.06,08:16,23.4375,21.3125,-329725.29766277934,-831495.3895684162,1684309.904775542,-4.621936714975163,4.986915925750509,-11.603981660678983,-3.477887887518591,3.4944285876263166,-12.356811216872302,-329721.81977489183,-831498.8839970038,1684322.2615867588
2024-12-19 08:23:13.440385,53671.22,08:23,23.375,21.3125,-329734.7903845316,-831492.0716029448,1684312.7976130631,-14.114658467238769,8.304881397169083,-8.71114413952455,-3.8363377662569595,3.8864335854848227,-12.2071037371022,-329730.95404676534,-831495.9580365302,1684325.0047168003
2024-12-19 08:28:54.940385,54012.72,08:28,23.375,21.25,-329721.1667336688,-831494.9847050617,1684309.8725981948,-0.49100760446162894,5.391779280267656,-11.636159007903188,-4.296175080592677,4.2436106569865455,-12.329960040565181,-329716.87055858824,-831499.2283157186,1684322.2025582353
2024-12-19 08:33:33.470385,54291.25,08:33,23.375,21.3125,-329723.07402222144,-831493.7537163397,1684316.6738359004,-2.398296157072764,6.622768002212979,-4.8349213022738695,-4.5068796469131485,4.655540956560379,-12.151325975723852,-329718.5671425745,-831498.4092572962,1684328.8251618762
2024-12-19 08:40:15.950385,54693.73,08:40,23.375,21.3125,-329721.0878901346,-831497.7703664259,1684311.9358252217,-0.41216407023603097,2.6061179160606116,-9.572931980947033,-4.337684368438204,4.41662007351988,-11.695159632945433,-329716.7502057662,-831502.1869864993,1684323.6309848547
2024-12-19 08:44:54.340385,54972.12,08:44,23.375,21.25,-329722.398425125,-831495.7878846087,1684303.9313745801,-1.7226990606286563,4.588599733193405,-17.577382622519508,-4.3195024009328336,4.744356182668443,-11.849055721593851,-329718.07892272406,-831500.5322407914,1684315.7804303018


==> data_singular_values_summary.tex <==
component_index,All params,Kinematic,Compliance,Thermal,Joint
1,4.272800e+02,2.965002e+02,3.212490e+01,4.272559e+02,2.234014e+01
2,3.052167e+02,2.924360e+02,1.255040e+01,1.079308e+02,1.787436e+01
3,3.017407e+02,2.578154e+02,1.136268e+00,5.747385e+01,1.756793e+01
4,2.584413e+02,1.948826e+02,6.779704e-01,1.922041e+01,1.740103e+01
5,2.093086e+02,1.716637e+02,2.282582e-01,1.277908e+01,1.710767e+01
6,1.928633e+02,1.560481e+02,1.946137e-01,7.798509e+00,1.691531e+01
7,1.765239e+02,4.995061e+01,1.820670e-01,,1.688849e+01
8,1.078909e+02,4.522692e+01,1.096035e-01,,1.667136e+01
9,5.746305e+01,3.742055e+01,3.393678e-02,,1.643300e+01
10,5.216732e+01,3.452538e+01,,,1.641728e+01
11,4.711189e+01,3.318588e+01,,,1.624676e+01
12,3.981030e+01,2.997852e+01,,,1.610250e+01
13,3.739057e+01,2.450679e+01,,,1.590701e+01
14,3.497070e+01,2.293380e+01,,,1.578264e+01
15,3.145055e+01,2.115048e+01,,,1.575610e+01
16,2.759821e+01,2.034194e+01,,,1.551806e+01
17,2.634834e+01,1.941652e+01,,,1.542696e+01
18,2.405616e+01,1.660012e+01,,,1.536241e+01
19,2.312124e+01,1.483169e+01,,,1.526213e+01
20,2.147503e+01,1.410074e+01,,,1.517497e+01
21,1.923511e+01,1.196220e+01,,,1.514704e+01
22,1.887885e+01,1.063422e+01,,,1.506286e+01
23,1.786517e+01,9.882580e+00,,,1.496953e+01
24,1.751881e+01,8.438083e+00,,,1.485876e+01
25,1.711404e+01,7.905956e+00,,,1.480532e+01
26,1.701159e+01,6.421809e+00,,,1.478971e+01
27,1.684052e+01,6.069727e+00,,,1.476003e+01
28,1.679375e+01,4.663476e+00,,,1.473636e+01
29,1.665862e+01,3.988788e+00,,,1.465251e+01
30,1.660944e+01,3.496845e+00,,,1.462353e+01
31,1.641521e+01,1.596999e-03,,,1.445293e+01
32,1.624283e+01,7.411606e-04,,,1.444092e+01
33,1.601929e+01,2.181109e-04,,,1.437772e+01
34,1.600116e+01,1.977504e-04,,,1.435437e+01
35,1.598969e+01,9.667393e-05,,,1.423358e+01
36,1.576621e+01,2.911029e-05,,,1.418402e+01
37,1.566166e+01,,,,1.413067e+01
38,1.551632e+01,,,,1.404872e+01
39,1.537362e+01,,,,1.399764e+01
40,1.528085e+01,,,,1.395634e+01
41,1.524011e+01,,,,1.393112e+01
42,1.513913e+01,,,,1.386074e+01
43,1.508167e+01,,,,1.377421e+01
44,1.493500e+01,,,,1.376271e+01
45,1.486649e+01,,,,1.368160e+01
46,1.481495e+01,,,,1.363586e+01
47,1.479004e+01,,,,1.362581e+01
48,1.475768e+01,,,,1.355997e+01
49,1.471678e+01,,,,1.349681e+01
50,1.458923e+01,,,,1.348460e+01
51,1.452048e+01,,,,1.342646e+01
52,1.443696e+01,,,,1.339547e+01
53,1.441516e+01,,,,1.337003e+01
54,1.438896e+01,,,,1.335091e+01
55,1.431844e+01,,,,1.331527e+01
56,1.419320e+01,,,,1.328287e+01
57,1.414347e+01,,,,1.326305e+01
58,1.407167e+01,,,,1.316290e+01
59,1.402069e+01,,,,1.312122e+01
60,1.396764e+01,,,,1.307568e+01
61,1.392878e+01,,,,1.305265e+01
62,1.391536e+01,,,,1.303847e+01
63,1.380423e+01,,,,1.301852e+01
64,1.379634e+01,,,,1.299872e+01
65,1.371621e+01,,,,1.298533e+01
66,1.368889e+01,,,,1.294617e+01
67,1.363992e+01,,,,1.293221e+01
68,1.360345e+01,,,,1.288833e+01
69,1.349045e+01,,,,1.285196e+01
70,1.347154e+01,,,,1.283818e+01
71,1.343859e+01,,,,1.281132e+01
72,1.340590e+01,,,,1.279579e+01
73,1.339834e+01,,,,1.278193e+01
74,1.336653e+01,,,,1.275636e+01
75,1.332499e+01,,,,1.272134e+01
76,1.331793e+01,,,,1.267191e+01
77,1.326424e+01,,,,1.265087e+01
78,1.325297e+01,,,,1.256591e+01
79,1.324117e+01,,,,1.254542e+01
80,1.320859e+01,,,,1.251665e+01
81,1.316748e+01,,,,1.248300e+01
82,1.313154e+01,,,,1.246037e+01
83,1.303810e+01,,,,1.245297e+01
84,1.302144e+01,,,,1.241703e+01
85,1.299440e+01,,,,1.239577e+01
86,1.296838e+01,,,,1.237178e+01
87,1.295699e+01,,,,1.236247e+01
88,1.292819e+01,,,,1.232377e+01
89,1.290388e+01,,,,1.229261e+01
90,1.286116e+01,,,,1.225297e+01
91,1.281507e+01,,,,1.221746e+01
92,1.280747e+01,,,,1.220746e+01
93,1.279878e+01,,,,1.220572e+01
94,1.279093e+01,,,,1.215809e+01
95,1.275740e+01,,,,1.211532e+01
96,1.272618e+01,,,,1.209059e+01
97,1.271679e+01,,,,1.204883e+01
98,1.267514e+01,,,,1.203170e+01
99,1.264747e+01,,,,1.200141e+01
100,1.261037e+01,,,,1.197575e+01
101,1.255866e+01,,,,1.196215e+01
102,1.253544e+01,,,,1.194111e+01
103,1.249907e+01,,,,1.191634e+01
104,1.248484e+01,,,,1.188418e+01
105,1.244111e+01,,,,1.184664e+01
106,1.241838e+01,,,,1.181886e+01
107,1.241301e+01,,,,1.181376e+01
108,1.236026e+01,,,,1.178645e+01
109,1.234221e+01,,,,1.177457e+01
110,1.232990e+01,,,,1.172634e+01
111,1.227842e+01,,,,1.171386e+01
112,1.226455e+01,,,,1.168027e+01
113,1.224061e+01,,,,1.167333e+01
114,1.223532e+01,,,,1.162775e+01
115,1.221567e+01,,,,1.162154e+01
116,1.217802e+01,,,,1.160273e+01
117,1.215086e+01,,,,1.157819e+01
118,1.212298e+01,,,,1.156967e+01
119,1.205939e+01,,,,1.156171e+01
120,1.204044e+01,,,,1.154300e+01
121,1.203378e+01,,,,1.152359e+01
122,1.201729e+01,,,,1.148237e+01
123,1.199058e+01,,,,1.145784e+01
124,1.195850e+01,,,,1.142523e+01
125,1.192613e+01,,,,1.140665e+01
126,1.190551e+01,,,,1.136291e+01
127,1.187458e+01,,,,1.135614e+01
128,1.184573e+01,,,,1.132519e+01
129,1.182232e+01,,,,1.132293e+01
130,1.181647e+01,,,,1.130593e+01
131,1.178797e+01,,,,1.126671e+01
132,1.176386e+01,,,,1.124285e+01
133,1.173545e+01,,,,1.121944e+01
134,1.170558e+01,,,,1.119589e+01
135,1.170171e+01,,,,1.117654e+01
136,1.167733e+01,,,,1.114997e+01
137,1.164297e+01,,,,1.114154e+01
138,1.162453e+01,,,,1.111390e+01
139,1.159491e+01,,,,1.109377e+01
140,1.158442e+01,,,,1.107827e+01
141,1.154892e+01,,,,1.105429e+01
142,1.154024e+01,,,,1.103493e+01
143,1.152669e+01,,,,1.099032e+01
144,1.151489e+01,,,,1.096462e+01
145,1.147343e+01,,,,1.094699e+01
146,1.145279e+01,,,,1.093562e+01
147,1.141327e+01,,,,1.092546e+01
148,1.140533e+01,,,,1.089931e+01
149,1.135210e+01,,,,1.086673e+01
150,1.134295e+01,,,,1.086275e+01
151,1.132759e+01,,,,1.082268e+01
152,1.131773e+01,,,,1.080409e+01
153,1.129973e+01,,,,1.080125e+01
154,1.127853e+01,,,,1.079498e+01
155,1.124524e+01,,,,1.075478e+01
156,1.121630e+01,,,,1.073230e+01
157,1.120722e+01,,,,1.072191e+01
158,1.119375e+01,,,,1.068692e+01
159,1.116865e+01,,,,1.066611e+01
160,1.114506e+01,,,,1.065123e+01
161,1.111947e+01,,,,1.062547e+01
162,1.109454e+01,,,,1.060257e+01
163,1.107637e+01,,,,1.059914e+01
164,1.106470e+01,,,,1.057132e+01
165,1.101539e+01,,,,1.052632e+01
166,1.098185e+01,,,,1.049508e+01
167,1.097090e+01,,,,1.047846e+01
168,1.096486e+01,,,,1.046582e+01
169,1.094778e+01,,,,1.043441e+01
170,1.094248e+01,,,,1.041989e+01
171,1.089699e+01,,,,1.039844e+01
172,1.086818e+01,,,,1.039208e+01
173,1.084879e+01,,,,1.036853e+01
174,1.081343e+01,,,,1.034264e+01
175,1.080190e+01,,,,1.032226e+01
176,1.079640e+01,,,,1.030095e+01
177,1.079084e+01,,,,1.026525e+01
178,1.076593e+01,,,,1.024662e+01
179,1.072896e+01,,,,1.023059e+01
180,1.071135e+01,,,,1.022526e+01
181,1.069644e+01,,,,1.019590e+01
182,1.066511e+01,,,,1.018361e+01
183,1.063136e+01,,,,1.016389e+01
184,1.062104e+01,,,,1.015422e+01
185,1.060248e+01,,,,1.012966e+01
186,1.058104e+01,,,,1.012008e+01
187,1.056396e+01,,,,1.009931e+01
188,1.053010e+01,,,,1.008594e+01
189,1.050535e+01,,,,1.005187e+01
190,1.048808e+01,,,,1.003486e+01
191,1.044340e+01,,,,1.002015e+01
192,1.043401e+01,,,,1.000121e+01
193,1.040326e+01,,,,9.970568e+00
194,1.039516e+01,,,,9.954135e+00
195,1.039263e+01,,,,9.940547e+00
196,1.034986e+01,,,,9.926736e+00
197,1.033721e+01,,,,9.912095e+00
198,1.031038e+01,,,,9.896453e+00
199,1.028692e+01,,,,9.881300e+00
200,1.027893e+01,,,,9.866297e+00
201,1.025100e+01,,,,9.856357e+00
202,1.023289e+01,,,,9.828819e+00
203,1.022126e+01,,,,9.821471e+00
204,1.020884e+01,,,,9.798142e+00
205,1.018700e+01,,,,9.766027e+00
206,1.016650e+01,,,,9.749969e+00
207,1.014590e+01,,,,9.736910e+00
208,1.014177e+01,,,,9.729394e+00
209,1.012825e+01,,,,9.718453e+00
210,1.009613e+01,,,,9.694449e+00
211,1.007112e+01,,,,9.670572e+00
212,1.006348e+01,,,,9.667512e+00
213,1.003811e+01,,,,9.619878e+00
214,1.000919e+01,,,,9.610175e+00
215,9.994748e+00,,,,9.597567e+00
216,9.976598e+00,,,,9.563030e+00
217,9.962296e+00,,,,9.559950e+00
218,9.955960e+00,,,,9.540672e+00
219,9.928589e+00,,,,9.522544e+00
220,9.919017e+00,,,,9.512806e+00
221,9.895706e+00,,,,9.510824e+00
222,9.868723e+00,,,,9.484663e+00
223,9.863861e+00,,,,9.461594e+00
224,9.846420e+00,,,,9.431069e+00
225,9.832866e+00,,,,9.429117e+00
226,9.820368e+00,,,,9.418371e+00
227,9.802932e+00,,,,9.391508e+00
228,9.794461e+00,,,,9.370922e+00
229,9.782218e+00,,,,9.369797e+00
230,9.757506e+00,,,,9.346668e+00
231,9.734254e+00,,,,9.322290e+00
232,9.716030e+00,,,,9.318499e+00
233,9.702363e+00,,,,9.314014e+00
234,9.696669e+00,,,,9.299560e+00
235,9.670013e+00,,,,9.274325e+00
236,9.660283e+00,,,,9.249877e+00
237,9.638526e+00,,,,9.242659e+00
238,9.613121e+00,,,,9.219065e+00
239,9.605298e+00,,,,9.215575e+00
240,9.569571e+00,,,,9.178002e+00
241,9.551217e+00,,,,9.166826e+00
242,9.540727e+00,,,,9.150847e+00
243,9.532931e+00,,,,9.132470e+00
244,9.518006e+00,,,,9.092680e+00
245,9.503516e+00,,,,9.086598e+00
246,9.480161e+00,,,,9.072016e+00
247,9.466020e+00,,,,9.064115e+00
248,9.458757e+00,,,,9.023913e+00
249,9.423489e+00,,,,9.011616e+00
250,9.405278e+00,,,,8.989525e+00
251,9.392164e+00,,,,8.975539e+00
252,9.387296e+00,,,,8.955493e+00
253,9.374433e+00,,,,8.947919e+00
254,9.358912e+00,,,,8.923914e+00
255,9.331776e+00,,,,8.913513e+00
256,9.317726e+00,,,,8.896780e+00
257,9.312456e+00,,,,8.884128e+00
258,9.297100e+00,,,,8.875629e+00
259,9.266525e+00,,,,8.868836e+00
260,9.257985e+00,,,,8.841972e+00
261,9.246095e+00,,,,8.834258e+00
262,9.229268e+00,,,,8.820910e+00
263,9.226069e+00,,,,8.818480e+00
264,9.179047e+00,,,,8.791645e+00
265,9.168658e+00,,,,8.776365e+00
266,9.157359e+00,,,,8.770512e+00
267,9.133021e+00,,,,8.755777e+00
268,9.105697e+00,,,,8.733874e+00
269,9.081042e+00,,,,8.724204e+00
270,9.071904e+00,,,,8.689051e+00
271,9.063965e+00,,,,8.663642e+00
272,9.034837e+00,,,,8.656335e+00
273,9.012898e+00,,,,8.647736e+00
274,9.008300e+00,,,,8.630820e+00
275,8.991425e+00,,,,8.621407e+00
276,8.975391e+00,,,,8.606088e+00
277,8.954122e+00,,,,8.594055e+00
278,8.936042e+00,,,,8.577805e+00
279,8.930083e+00,,,,8.565630e+00
280,8.920375e+00,,,,8.556228e+00
281,8.896107e+00,,,,8.531659e+00
282,8.879962e+00,,,,8.511227e+00
283,8.869179e+00,,,,8.506936e+00
284,8.864701e+00,,,,8.503208e+00
285,8.852337e+00,,,,8.464476e+00
286,8.839247e+00,,,,8.456885e+00
287,8.805384e+00,,,,8.420272e+00
288,8.799970e+00,,,,8.414038e+00
289,8.782417e+00,,,,8.399015e+00
290,8.770868e+00,,,,8.390790e+00
291,8.765401e+00,,,,8.381610e+00
292,8.731120e+00,,,,8.360075e+00
293,8.711869e+00,,,,8.349146e+00
294,8.702672e+00,,,,8.344545e+00
295,8.693803e+00,,,,8.331433e+00
296,8.667713e+00,,,,8.318187e+00
297,8.647078e+00,,,,8.303139e+00
298,8.636909e+00,,,,8.284420e+00
299,8.633557e+00,,,,8.279657e+00
300,8.623952e+00,,,,8.269073e+00
301,8.599590e+00,,,,8.252648e+00
302,8.580134e+00,,,,8.250951e+00
303,8.566770e+00,,,,8.240238e+00
304,8.560700e+00,,,,8.213269e+00
305,8.541567e+00,,,,8.193253e+00
306,8.523673e+00,,,,8.173570e+00
307,8.512577e+00,,,,8.149492e+00
308,8.508136e+00,,,,8.125375e+00
309,8.483935e+00,,,,8.117454e+00
310,8.459820e+00,,,,8.108736e+00
311,8.452837e+00,,,,8.078928e+00
312,8.422942e+00,,,,8.070206e+00
313,8.407240e+00,,,,8.041270e+00
314,8.393974e+00,,,,8.031778e+00
315,8.382778e+00,,,,8.022216e+00
316,8.373231e+00,,,,8.020504e+00
317,8.353563e+00,,,,8.006677e+00
318,8.344611e+00,,,,7.993893e+00
319,8.334498e+00,,,,7.964707e+00
320,8.321596e+00,,,,7.941915e+00
321,8.302646e+00,,,,7.931821e+00
322,8.292333e+00,,,,7.921013e+00
323,8.285758e+00,,,,7.899412e+00
324,8.266163e+00,,,,7.879129e+00
325,8.256951e+00,,,,7.871254e+00
326,8.251480e+00,,,,7.860939e+00
327,8.226047e+00,,,,7.853370e+00
328,8.212459e+00,,,,7.842734e+00
329,8.196579e+00,,,,7.831376e+00
330,8.181909e+00,,,,7.814834e+00
331,8.161530e+00,,,,7.791136e+00
332,8.140601e+00,,,,7.771240e+00
333,8.122332e+00,,,,7.761300e+00
334,8.109004e+00,,,,7.753641e+00
335,8.098994e+00,,,,7.734972e+00
336,8.081664e+00,,,,7.720343e+00
337,8.065800e+00,,,,7.713673e+00
338,8.046559e+00,,,,7.696070e+00
339,8.029006e+00,,,,7.673218e+00
340,8.016999e+00,,,,7.661539e+00
341,8.011766e+00,,,,7.648404e+00
342,7.992982e+00,,,,7.628699e+00
343,7.970103e+00,,,,7.627385e+00
344,7.955234e+00,,,,7.609169e+00
345,7.937343e+00,,,,7.580152e+00
346,7.926221e+00,,,,7.567646e+00
347,7.904114e+00,,,,7.542422e+00
348,7.899649e+00,,,,7.538195e+00
349,7.888867e+00,,,,7.532633e+00
350,7.862206e+00,,,,7.512630e+00
351,7.851981e+00,,,,7.494346e+00
352,7.833642e+00,,,,7.474873e+00
353,7.821745e+00,,,,7.464170e+00
354,7.812408e+00,,,,7.457931e+00
355,7.801909e+00,,,,7.423072e+00
356,7.794068e+00,,,,7.403733e+00
357,7.787185e+00,,,,7.392000e+00
358,7.775829e+00,,,,7.387635e+00
359,7.752439e+00,,,,7.376626e+00
360,7.737184e+00,,,,7.352013e+00
361,7.731160e+00,,,,7.346781e+00
362,7.718953e+00,,,,7.319024e+00
363,7.700726e+00,,,,7.307601e+00
364,7.681719e+00,,,,7.304577e+00
365,7.670212e+00,,,,7.293174e+00
366,7.655575e+00,,,,7.282295e+00
367,7.636577e+00,,,,7.267516e+00
368,7.621416e+00,,,,7.248200e+00
369,7.615727e+00,,,,7.230264e+00
370,7.600103e+00,,,,7.203265e+00
371,7.582137e+00,,,,7.197381e+00
372,7.570511e+00,,,,7.184003e+00
373,7.554799e+00,,,,7.162568e+00
374,7.531857e+00,,,,7.143298e+00
375,7.529391e+00,,,,7.119763e+00
376,7.524735e+00,,,,7.100338e+00
377,7.504318e+00,,,,7.085293e+00
378,7.489305e+00,,,,7.082319e+00
379,7.459957e+00,,,,7.063994e+00
380,7.451544e+00,,,,7.051940e+00
381,7.444525e+00,,,,7.043900e+00
382,7.416827e+00,,,,7.026418e+00
383,7.408547e+00,,,,7.019941e+00
384,7.397216e+00,,,,7.010251e+00
385,7.385189e+00,,,,7.007514e+00
386,7.377245e+00,,,,6.991382e+00
387,7.365875e+00,,,,6.982293e+00
388,7.350174e+00,,,,6.976495e+00
389,7.341149e+00,,,,6.955885e+00
390,7.320095e+00,,,,6.948549e+00
391,7.302748e+00,,,,6.928513e+00
392,7.297610e+00,,,,6.917791e+00
393,7.279277e+00,,,,6.890893e+00
394,7.256166e+00,,,,6.886579e+00
395,7.239481e+00,,,,6.865520e+00
396,7.209669e+00,,,,6.851589e+00
397,7.191603e+00,,,,6.828895e+00
398,7.174029e+00,,,,6.803999e+00
399,7.172383e+00,,,,6.797502e+00
400,7.160914e+00,,,,6.787493e+00
401,7.132410e+00,,,,6.770573e+00
402,7.112141e+00,,,,6.762520e+00
403,7.105392e+00,,,,6.727318e+00
404,7.089280e+00,,,,6.722930e+00
405,7.081562e+00,,,,6.690362e+00
406,7.073878e+00,,,,6.684023e+00
407,7.057152e+00,,,,6.672259e+00
408,7.048916e+00,,,,6.659536e+00
409,7.037539e+00,,,,6.646244e+00
410,7.023627e+00,,,,6.616382e+00
411,7.010669e+00,,,,6.608585e+00
412,6.998119e+00,,,,6.594481e+00
413,6.986301e+00,,,,6.590170e+00
414,6.975324e+00,,,,6.579334e+00
415,6.972986e+00,,,,6.567958e+00
416,6.944740e+00,,,,6.562266e+00
417,6.937694e+00,,,,6.526289e+00
418,6.927340e+00,,,,6.507803e+00
419,6.909735e+00,,,,6.490225e+00
420,6.884242e+00,,,,6.460318e+00
421,6.879864e+00,,,,6.448585e+00
422,6.869785e+00,,,,6.437424e+00
423,6.847130e+00,,,,6.414904e+00
424,6.831745e+00,,,,6.405088e+00
425,6.817710e+00,,,,6.378168e+00
426,6.803325e+00,,,,6.367050e+00
427,6.792032e+00,,,,6.360058e+00
428,6.766033e+00,,,,6.355715e+00
429,6.744491e+00,,,,6.338208e+00
430,6.730079e+00,,,,6.325862e+00
431,6.707076e+00,,,,6.318503e+00
432,6.696280e+00,,,,6.314971e+00
433,6.693657e+00,,,,6.283460e+00
434,6.682269e+00,,,,6.269231e+00
435,6.660853e+00,,,,6.252139e+00
436,6.643974e+00,,,,6.250942e+00
437,6.622039e+00,,,,6.217977e+00
438,6.610934e+00,,,,6.196727e+00
439,6.599511e+00,,,,6.180903e+00
440,6.592755e+00,,,,6.157048e+00
441,6.587326e+00,,,,6.144816e+00
442,6.566523e+00,,,,6.119993e+00
443,6.563585e+00,,,,6.103873e+00
444,6.530863e+00,,,,6.077773e+00
445,6.526665e+00,,,,6.047486e+00
446,6.493920e+00,,,,6.022262e+00
447,6.482489e+00,,,,5.998731e+00
448,6.451623e+00,,,,5.981325e+00
449,6.435725e+00,,,,5.968510e+00
450,6.433712e+00,,,,5.954213e+00
451,6.404803e+00,,,,5.941234e+00
452,6.398604e+00,,,,5.935741e+00
453,6.371738e+00,,,,5.899243e+00
454,6.362397e+00,,,,5.887316e+00
455,6.353161e+00,,,,5.873111e+00
456,6.347122e+00,,,,5.867459e+00
457,6.335512e+00,,,,5.852585e+00
458,6.318814e+00,,,,5.837129e+00
459,6.310276e+00,,,,5.791989e+00
460,6.293142e+00,,,,5.770997e+00
461,6.267227e+00,,,,5.748431e+00
462,6.263432e+00,,,,5.734515e+00
463,6.242576e+00,,,,5.730488e+00
464,6.216838e+00,,,,5.697045e+00
465,6.190681e+00,,,,5.677742e+00
466,6.184139e+00,,,,5.662618e+00
467,6.155576e+00,,,,5.635368e+00
468,6.140034e+00,,,,5.601478e+00
469,6.117556e+00,,,,5.580748e+00
470,6.098114e+00,,,,5.564333e+00
471,6.076655e+00,,,,5.550173e+00
472,6.043596e+00,,,,5.539827e+00
473,6.004699e+00,,,,5.534564e+00
474,5.992542e+00,,,,5.506862e+00
475,5.982522e+00,,,,5.488899e+00
476,5.972642e+00,,,,5.468933e+00
477,5.956110e+00,,,,5.440283e+00
478,5.944833e+00,,,,5.437884e+00
479,5.933794e+00,,,,5.435814e+00
480,5.898226e+00,,,,5.418453e+00
481,5.884009e+00,,,,5.401108e+00
482,5.871552e+00,,,,5.394213e+00
483,5.866047e+00,,,,5.380237e+00
484,5.845531e+00,,,,5.363725e+00
485,5.839232e+00,,,,5.346403e+00
486,5.793465e+00,,,,5.327777e+00
487,5.772694e+00,,,,5.325731e+00
488,5.750310e+00,,,,5.303308e+00
489,5.742234e+00,,,,5.297214e+00
490,5.730839e+00,,,,5.271663e+00
491,5.691947e+00,,,,5.261399e+00
492,5.675825e+00,,,,5.240140e+00
493,5.654062e+00,,,,5.210737e+00
494,5.633777e+00,,,,5.189148e+00
495,5.600800e+00,,,,5.182610e+00
496,5.580835e+00,,,,5.166039e+00
497,5.556946e+00,,,,5.153555e+00
498,5.551062e+00,,,,5.138651e+00
499,5.536581e+00,,,,5.130801e+00
500,5.525706e+00,,,,5.122006e+00
501,5.510950e+00,,,,5.119152e+00
502,5.489750e+00,,,,5.085607e+00
503,5.467663e+00,,,,5.063826e+00
504,5.450808e+00,,,,5.044166e+00
505,5.438741e+00,,,,5.012146e+00
506,5.429247e+00,,,,4.974765e+00
507,5.423031e+00,,,,4.963113e+00
508,5.404173e+00,,,,4.946198e+00
509,5.392432e+00,,,,4.911753e+00
510,5.385745e+00,,,,4.896518e+00
511,5.365602e+00,,,,4.879585e+00
512,5.351680e+00,,,,4.814899e+00
513,5.339879e+00,,,,4.723289e+00
514,5.312716e+00,,,,4.696918e+00
515,5.302382e+00,,,,4.691788e+00
516,5.292767e+00,,,,4.670979e+00
517,5.273195e+00,,,,4.657345e+00
518,5.256241e+00,,,,4.636238e+00
519,5.241894e+00,,,,4.599538e+00
520,5.217836e+00,,,,4.536665e+00
521,5.204060e+00,,,,4.507669e+00
522,5.196436e+00,,,,4.502907e+00
523,5.174628e+00,,,,4.483987e+00
524,5.156808e+00,,,,4.463673e+00
525,5.148118e+00,,,,4.411370e+00
526,5.142212e+00,,,,4.383461e+00
527,5.124529e+00,,,,4.369078e+00
528,5.118757e+00,,,,4.332847e+00
529,5.100734e+00,,,,4.329713e+00
530,5.074741e+00,,,,4.307206e+00
531,5.045131e+00,,,,4.292009e+00
532,5.003142e+00,,,,4.268451e+00
533,4.968325e+00,,,,4.224709e+00
534,4.959687e+00,,,,4.165172e+00
535,4.923853e+00,,,,4.114462e+00
536,4.897303e+00,,,,4.094723e+00
537,4.885650e+00,,,,4.086969e+00
538,4.837588e+00,,,,4.062596e+00
539,4.805629e+00,,,,4.012472e+00
540,4.721791e+00,,,,3.959939e+00
541,4.697286e+00,,,,3.869212e+00
542,4.693642e+00,,,,3.855843e+00
543,4.669282e+00,,,,3.843879e+00
544,4.650317e+00,,,,3.832036e+00
545,4.634233e+00,,,,3.777621e+00
546,4.627722e+00,,,,3.764268e+00
547,4.570174e+00,,,,3.741637e+00
548,4.533457e+00,,,,3.697690e+00
549,4.503706e+00,,,,3.683449e+00
550,4.501249e+00,,,,3.630841e+00
551,4.483776e+00,,,,3.615802e+00
552,4.463631e+00,,,,3.566151e+00
553,4.390931e+00,,,,3.558232e+00
554,4.377570e+00,,,,3.547821e+00
555,4.337813e+00,,,,3.447296e+00
556,4.330181e+00,,,,3.398014e+00
557,4.322816e+00,,,,3.350248e+00
558,4.310627e+00,,,,3.118216e+00
559,4.285591e+00,,,,3.112344e+00
560,4.269753e+00,,,,3.055488e+00
561,4.251194e+00,,,,3.012116e+00
562,4.198323e+00,,,,2.935493e+00
563,4.168764e+00,,,,2.934305e+00
564,4.130698e+00,,,,2.843307e+00
565,4.092309e+00,,,,2.839635e+00
566,4.080862e+00,,,,2.671742e+00
567,4.069696e+00,,,,2.632168e+00
568,4.012450e+00,,,,2.586833e+00
569,4.003855e+00,,,,2.404675e+00
570,3.852154e+00,,,,
571,3.844339e+00,,,,
572,3.833502e+00,,,,
573,3.790652e+00,,,,
574,3.774267e+00,,,,
575,3.760967e+00,,,,
576,3.695540e+00,,,,
577,3.669493e+00,,,,
578,3.625099e+00,,,,
579,3.614467e+00,,,,
580,3.577176e+00,,,,
581,3.563352e+00,,,,
582,3.555661e+00,,,,
583,3.398602e+00,,,,
584,3.368613e+00,,,,
585,3.337630e+00,,,,
586,3.138774e+00,,,,
587,3.105010e+00,,,,
588,3.083020e+00,,,,
589,3.004801e+00,,,,
590,2.945529e+00,,,,
591,2.934746e+00,,,,
592,2.843826e+00,,,,
593,2.839161e+00,,,,
594,2.680509e+00,,,,
595,2.635962e+00,,,,
596,2.587169e+00,,,,
597,2.413752e+00,,,,
598,2.386336e+00,,,,
599,1.842911e+00,,,,
600,1.432751e+00,,,,
601,3.478526e-01,,,,
602,8.805941e-02,,,,
603,5.505450e-02,,,,
604,4.133471e-02,,,,
605,2.841477e-02,,,,
606,2.244756e-02,,,,
607,1.457868e-02,,,,
608,4.376022e-04,,,,
609,2.863317e-04,,,,
610,1.977963e-04,,,,
611,9.939765e-05,,,,
612,5.581134e-05,,,,
613,4.627895e-05,,,,
614,3.194565e-05,,,,
615,2.964567e-05,,,,
616,1.025116e-05,,,,
617,2.949355e-06,,,,
618,6.897364e-07,,,,
619,3.327876e-07,,,,
620,2.673327e-07,,,,
621,7.661240e-09,,,,
622,5.913288e-12,,,,
623,2.349087e-13,,,,
624,1.181403e-13,,,,
625,8.825186e-14,,,,
626,4.542375e-14,,,,
627,1.160349e-14,,,,
628,9.248200e-16,,,,
629,6.271216e-16,,,,
630,3.990581e-16,,,,
631,2.141535e-16,,,,
632,1.197107e-16,,,,
633,4.178159e-17,,,,
634,9.801744e-30,,,,
635,4.349561e-33,,,,

